Uncovering and Exploiting Hidden APIs in Mobile Super Apps

Mobile applications, particularly those from social media platforms such as WeChat and TikTok, are evolving into "super apps" that offer a wide range of services such as instant messaging and media sharing, e-commerce, e-learning, and e-government. These super apps often provide APIs for developers to create "miniapps" that run within the super app. These APIs should have been thoroughly scrutinized for security. Unfortunately, we find that many of them are undocumented and unsecured, potentially allowing miniapps to bypass restrictions and gain higher privileged access. To systematically identify these hidden APIs before they are exploited by attackers, we developed a tool APIScope with both static analysis and dynamic analysis, where static analysis is used to recognize hidden undocumented APIs, and dynamic analysis is used to confirm whether the identified APIs can be invoked by an unprivileged 3rdparty miniapps. We have applied APIScope to five popular super apps (i.e., WeChat, WeCom, Baidu, QQ, and Tiktok) and found that all of them contain hidden APIs, many of which can be exploited due to missing security checks. We have also quantified the hidden APIs that may have security implications by verifying if they have access to resources protected by Android permissions. Furthermore, we demonstrate the potential security hazards by presenting various attack scenarios, including unauthorized access to any web pages, downloading and installing malicious software, and stealing sensitive information. We have reported our findings to the relevant vendors, some of whom have patched the vulnerabilities and rewarded us with bug bounties.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}

==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> images/histograms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotstableread[col sep=comma,header=true]{images/1-normal.csv}\normal
\pgfplotstableread[col sep=comma,header=true]{images/2-wallhack.csv}\wallhack
\pgfplotstableread[col sep=comma,header=true]{images/3-aimbot.csv}\aimbot
\pgfplotstableread[col sep=comma,header=true]{images/4-triggerbot.csv}\triggerbot
\pgfplotstableread[col sep=comma,header=true]{images/5-artificial.csv}\artificial
\pgfplotstableread[col sep=comma,header=true]{images/6-speedhack.csv}\speedhack

\begin{figure*}[t]
\centering
\captionsetup{margin=0.2cm}
\scalebox{1.0}{

 \begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
          \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
              xmin = 0, xmax = 70, xlabel={(a)}, xlabel style = {font=\Large}, 
              legend style={font=\Large},
              xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\LARGE}
              ]
              \addplot[color=blue,
                solid,
                mark=*,
                mark options={solid},
                smooth] table[x expr=\thisrowno{0}, y index={1}]{\normal};
              \legend{No Cheats}
            \end{axis}
          \end{tikzpicture}      	
        }
        %\caption{(a)}
        \label{fig:normal}
     
\end{minipage}%

 \begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
         \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
               legend style={font=\Large},
              xmin = 0, xmax = 70, xlabel={(b)}, xlabel style = {font=\Large}, 
               xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\Large}
              ]
				\addplot[color=red,
                solid,
                mark=*,
                mark options={solid},
                smooth] table[x expr=\thisrowno{0}, y index={1}, color=red]{\wallhack};
              \legend{Wall-hack}
            \end{axis}
          \end{tikzpicture}
      
            	
        }
       %\caption{(b)}
        \label{fig:wallhack}
     
\end{minipage}%

 \begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
         \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
               legend style={font=\Large},
              xmin = 0, xmax = 70, xlabel={(c)}, xlabel style = {font=\Large}, 
               xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\Large}
              ]
				\addplot[color=red,
                solid,
                mark=*,
                mark options={solid},
                smooth] table[x expr=\thisrowno{0}, y index={1}]{\aimbot};
              \legend{Aim-bot}
            \end{axis}
          \end{tikzpicture}
      
            	
        }
       %\caption{Distribution of average data buffer sizes sent using wallhack cheat for groups of 400 send API calls}
        \label{fig:aimbot}
     
\end{minipage}%

	\begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
         \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
               legend style={font=\Large},
              xmin = 0, xmax = 70, xlabel={(d)}, xlabel style = {font=\Large}, 
               xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\Large}
              ]
				\addplot[color=red,
                solid,
                mark=*,
                mark options={solid},
                smooth] table[x expr=\thisrowno{0}, y index={1}]{\triggerbot};
              \legend{Trigger-bot}
            \end{axis}
          \end{tikzpicture}   	
        }
       %\caption{Distribution of average data buffer sizes sent using wallhack cheat for groups of 400 send API calls}
        \label{fig:triggerbot}
     
\end{minipage}%
 
}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}[t]
\centering
\captionsetup{margin=0.2cm}
\scalebox{1.0}{

 \begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
          \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
               legend style={font=\Large},
              xmin = 0, xmax = 70, xlabel={(e)}, xlabel style = {font=\Large}, 
               xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\Large}
              ]
              \addplot[color=red,
                solid,
                mark=*,
                mark options={solid},
                smooth] table[x expr=\thisrowno{0}, y index={1}]{\artificial};
              \legend{Artificial Lag}
            \end{axis}
          \end{tikzpicture}

            	
        }
        %\caption{Distribution of average data buffer sizes sent during normal game play for groups of 400 send API calls}
        \label{fig:artificial}
     
\end{minipage}%

 \begin{minipage}{0.23\linewidth}
      \centering
      \resizebox{0.90\linewidth}{!}{
      
         \begin{tikzpicture}
            \begin{axis}[
              legend pos = north east,
               legend style={font=\Large},
              xmin = 0, xmax = 70, xlabel={(f)}, xlabel style = {font=\Large}, 
               xticklabel style = {font=\Large},
              yticklabel style = {font=\Large},
              ymin = 0, ymax = 120, ylabel={Average frequency}, ylabel style = {font=\Large}
              ]
				\addplot[color=red,
                solid, mark=*, mark options={solid}, smooth] table[x expr=\thisrowno{0}, y index={1}]{\speedhack};
              \legend{Speed hack}
            \end{axis}
          \end{tikzpicture}
      
            	
        }
       %\caption{Distribution of average data buffer sizes sent using wallhack cheat for groups of 400 send API calls}
        \label{fig:speedhack}
 \end{minipage}%
 
  
  \begin{minipage}{0.25\linewidth}
      \centering
      \resizebox{0.95\linewidth}{!}{
      
      \begin{tikzpicture}
      \begin{axis}[ 
      xbar, xmin=0, xmax = 25,
      xlabel={(g) Average time (sec) per 400 API calls},
      symbolic y coords={%
          {Without Cheat},
          {Wall-hack},
          {Aim-bot},
          {Trigger-bot},
          {Artificial lag},
          Speed-hack},
      ytick=data,
      nodes near coords, 
      xticklabel style = {font=\Large},
      yticklabel style = {font=\Large},
      xlabel style = {font=\Large},
      ylabel style = {font=\Large},
      nodes near coords align={horizontal},
      ytick=data
      ]
      \addplot coordinates {
          (10.29,{Without Cheat}) 
          (13.14,{Wall-hack}) 
          (10.94,{Aim-bot}) 
          (15.81,{Trigger-bot})
          (18.52,{Artificial lag})
          (4.06,Speed-hack)};
      \end{axis}
      \end{tikzpicture} %width=6cm,height=7.59cm  	
        }
       %\caption{Distribution of average data buffer sizes sent using wallhack cheat for groups of 400 send API calls}
        \label{fig:call-time}
 \end{minipage}%
  
   }
 \caption{Average frequency distribution of data buffer sizes (x-axis) sent from client to server during game play (a) without cheats and with (b) \textit{wall-hack}, (c) \textit{aim-bot} (d) \textit{trigger-bot} (e) \textit{artificial lag} and (f) \textit{speed-hack} installed. Results are calculated over groups of 400 network \texttt{sendto()} API calls. Figure-(g) shows the average time taken to run them.}
\label{fig:distribution}
\end{figure*}


==> images/policy.tex <==
\definecolor{gray}{rgb}{0.4,0.4,0.4}
\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
\definecolor{cyan}{rgb}{0.0,0.6,0.6}

\lstset{
  basicstyle=\ttfamily\footnotesize,
  columns=fullflexible,
  showstringspaces=false,
  commentstyle=\color{gray}\upshape
}

\lstdefinelanguage{XML}
{
  morestring=[b]",
  morestring=[s]{>}{<},
  morecomment=[s]{<?}{?>},
  stringstyle=\color{black},
  identifierstyle=\color{darkblue},
  keywordstyle=\color{cyan},
  morekeywords={xmlns,version,type}% list your attributes here
}

\begin{lstlisting}[float, 
					language=XML, 
                    caption={A simplified policy for detecting \textit{unlimited health} and \textit{unlimited ammunition} cheats. In run-time integrity check, \texttt{read\_time\_limit} value is assigned to \texttt{MAX\_TIMEOUT} used in \autoref{lst:tsx-listing}.},
                    label = {lst:xml-listing},
                    captionpos=b]
<policy-health-check>
	<max_value> 0 </max_value>
    <min_value> 100 </min_value>
    <update_order> DESC </update_order>
    <memory_region> 
    	<addr_offsets> [val1] <addr_offsets>
    	<size> [val2] </size>
        <read_time_limit> [val3] </read_time_limit>
    </memory_region>
<\policy-health-check>
<policy-ammo-check>
	<primary-ammo> 
    	<max_round> 7 </max_round>
        <max_bullets> 140 </max_bullets>
        <update_order> DESC </update_order>
        <memory_region> 
        	<addr_offsets> [val4] <addr_offsets>
            <size> [val5] </size>
            <read_time_limit> [val6] </read_time_limit>
        </memory_region>
    </primary-ammo>
    </secondary-ammo> 
    	.
    </secondary-ammo> 
</policy-ammo-check>
\end{lstlisting}



==> images/tsx-listing.tex <==
\lstset{
    frame=tb, % draw a frame at the top and bottom of the code block
    tabsize=4, % tab space width
    showstringspaces=false, % don't mark spaces in strings
    %numbers=left, % display line numbers on the left
    commentstyle=\color{brown}, % comment color
    keywordstyle=\color{blue}, % keyword color
    stringstyle=\color{red} % string color
}

\begin{lstlisting}[float, 
					language=C++, 
                    caption={A simplified TSX-based function for reading arbitrary game memory regions. It returns the reading time using a secure reference clock detailed in~\cite{Chen:2017:DPS}.},
                    label = {lst:tsx-listing},
                    captionpos=b]
// placeholder for game memory data                  
int game_data[MAX_VAL]; 
// function to read arbitrary game memory
int read_region(int * address, int size){
	int start_time, end_time, time_elapsed;
    // read time from a secure reference clock
    start_time = get_current_time();
	while(1){
    	// begin RTM transaction
    	if (_xbegin() == _XBEGIN_STARTED) {
          for(int i = 0; i < size; i++){
          	game_data[i] = *(address + i);
          }
          // commit and end transaction
          _xend();
		} else {
        	// code when transaction aborts
        	time_elapsed = get_current_time() - start_time;
        	if( time_elapsed > MAX_TIMEOUT){
                break;
            }
		}
	}
    end_time = get_current_time();
    return (end_time - start_time);
}

\end{lstlisting}




==> images/tsx-sample.tex <==
\lstset{
    frame=tb, % draw a frame at the top and bottom of the code block
    tabsize=4, % tab space width
    showstringspaces=false, % don't mark spaces in strings
    %numbers=left, % display line numbers on the left
    commentstyle=\color{brown}, % comment color
    keywordstyle=\color{blue}, % keyword color
    stringstyle=\color{red}, % string color
    basicstyle=\footnotesize\ttfamily,
    breaklines=true,
    stepnumber=1,
    numbers=left,
    xleftmargin=2em
    %frame=single,
    %framexleftmargin=1.5em
}

\begin{lstlisting}[float, 
					language=C++, 
                    caption={An example snippet for TSX transaction.},
                    label = {tsx-sample},
                    captionpos=b]
// begin transaction
if ((status = _xbegin()) == _XBEGIN_STARTED) {
	// transaction code
    [statement-1, statement-2, ..., statement-n]
	// commit and end transaction
	_xend();
} else {
	[fall-back code during abort]
}
\end{lstlisting}



==> paper/00_abs_backup.tex <==
\begin{abstract}
   Recently, a novel miniapp paradigm, called miniapp, has brought significant convenience to our daily life, where small programs host into the super apps (e.g., \wechat, \textsf{Tiktok}), and enrich functionalities (e.g. e-commerce, e-learning, e-government) of those super apps. These miniapps can be developed by 1st party (i.e., the one who also programmed the super apps) or by the 3rd party developers.  While intuitively, for a specific super app platform,  both the 1st-part miniapps and the 3rd-party miniapps should have used the same set of the APIs, since they are all built on top of the same platform. In this work, we surprisingly found that the 1st party miniapps may additionally use some APIs that are not publicly documented at their API documentation (much like backdoors). These undocumented APIs can achieve high privileged functionalities (e.g., APK downloading, arbitrary web view accessing, sensitive information querying), which are restricted to be used by 3rd party miniapps. However, due to the lack of security checks, we found that the undocumented APIs can be invoked by the 3rd party miniapps as well, resulting in undocumented API abuse issues, which powers multiple attacks (e.g., SQL injection, information stealing, arbitrary file overwritten and malware installation). To qualify the issues, we designed a tool \sysname with two novel techniques developed (i.e., static API recognition to identify the undocumented APIs,  and dynamic API classification to further confirm whether the identified API are exploitable), and scanned five leading miniapps providers (e.g., \wechat, \textsf{WeCom} \textsf{Baidu}, \textsf{QQ} and \textsf{Tiktok}). Our results are worrisome: all of them have undocumented APIs, and are subject to API abuse.  We have reported our findings to all the vendors, and some of them ranked the issues as the high severity vulnerability and rewarded us with bug bounty. We also learned that some of them have already fixed the issues. \looseness=-1         
%The past few years have witnessed a rapid increase in the popularity of miniapp paradigm
 %in which a mobile super app (e.g., \wechat~\cite{totalrevenue}, \textsf{Snapchat}~\cite{snapmini}) provides a seamless runtime environment for a miniapp, a web-app alike small application, for enhanced user experience (e.g., install-less) and stickiness with the super app (e.g., a user can access almost all the daily services without leaving it).


\end{abstract}




==> paper/04_enum.tex <==

In this section,
    we introduce the methods that we used to crawl WeChat open documents and enumerate MiniProgram interfaces and APIs in WeChat Android app.

\subsection{Crawling Official Documents}

A well-written API document is essential to developers.
From the view of the developers,
    these APIs are provided officially that developers may use to fulfill their requirements.
However,
    from the view of a malicious attacker,
    the API documents is the entrypoint of compromising the WeChat framework,
    even the whole system.

Generally speaking,
    the APIs which are well-written in open documents should be tracked and maintained by WeChat.
Thus,
    in this paper,
    we assume that the open APIs are fully controlled and well-maintained by WeChat and a malicious attacker may not leverage those APIs to compromising MiniProgram framework or system.

\noindent
\textbf{Analysing WeChat Open Documents}

An active API described in WeChat open documents generally contains the following parts.

\begin{enumerate}[i]
    \item \textbf{Category} The category (and subcategory) of the API.
            WeChat defined multiple categories of a API,
            including Network, Location, File and Devices etc,
            which each one may contain more subcategories.

    \item \textbf{Definition} The detailed definition of the API,
            which contains API name,
            type of return value,
            parameters and type of parameters.

    \item \textbf{Hints} The other information that developers may notice,
            including deprecated API and fallback compatibility.

    \item \textbf{Examples} the example usage of the API.
            A good example usage may guide developers to use them correctly and securely.
\end{enumerate}

Almost all of the API documents of vendors have structured layouts,
    as well as WeChat open documents.
Therefor,
    we may analyze each part of the API document by utilizing HTML DOM tree analysis.

\sysname will be given an initial document URL and then send request to the specified URL.
When the initial response is successfully received,
    \sysname will build the DOM tree from the original response texts,
    analyze all of the APIs by a side placement of the indexes and push them into a request queue.

After that,
    \sysname iterate the queue,
    send the request of the target API documents asynchronously and finally fetch the response.

Whenever \sysname obtain the response,
    \sysname build the HTML DOM tree from the plain response texts.
Though the DOM tree,
    \sysname is able to analyze each part of the documents,
    and gather them into a simple JSON-based database for further analysis.

\CW{need to put a figure here...}

% Maybe there should have some NLP work 
% (maybe?) to processing the detail message
% of the documents

\noindent
\textbf{Document Analysis}

\CW{I don't know what further analysis is needed here,
    but I just think there should have more processing required to tell our story.}


% present why no static analysis

\subsection{Enumerating Local Interfaces}

Differ from the official open documents,
    the implementation of those APIs are highly bounded with platforms.
For WeChat,
    there are three common platforms that are widely used by users: 1) Android, 2) iOS and 3) Windows.
During our investigation,
    we noticed that Android and Windows platforms are using \code{V8} to implement their MiniProgram runtime,
    and iOS are using JSCore to do that.
After that,
    we assessed these three platforms,
    and developed the enumerating local interfaces part of \sysname targeting Android platform.

\noindent
\textbf{Dynamic Analysis}

In Android platform,
    WeChat implemented a series of native libraries upon \code{V8} engine.
These libraries are designed in multiple purposes,
    such as native \code{V8} features access,
    performance optimization and communication bridge with framework layer.

In this paper,
    we mainly focus on the access control and isolation of the MiniProgram framework.
In WeChat,
    framework layer is written by Java,
    and communicate with the native layer by JNI.
Thus,
    % actually, it IS frida
    we leverage a dynamic binary instrumentation (DBI) framework to execute arbitrary code inside \code{V8} engine to finish our analysis.

\CW{here maybe need a figure as well...
I dont know if theres anymore time I can handle those figures...}

\CW{Should we present the MiniProgram startup workflow in background?}

First of all,
    \sysname look into the Java heap to search for a live \code{V8} runtime object,
    and invoke \code{getV8} method to obtain \code{V8} instance.

After that,
    \sysname register and initialize a new thread object into the Java heap,
    which carries our JavaScript payloads.
    
Finally,
    \sysname invoke the runtime evaluate methods to reschedule the previous created thread object into JavaScript runtime thread,
    which can execute our payloads directly in the MiniProgram runtime.

\noindent
\textbf{Enumerating Runtime Interfaces}

To obtain all of the interfaces in MiniProgram runtime,
    we utilized JavaScript built-in methods and developed a recursive search algorithm.

\CW{put a algorithm code here?}

Generally,
    WeChat MiniProgram runtime is implemented like \code{Node.JS} runtime,
    which has a global-accessibly object named \code{global}.
Though this object,
    we are able to enumerate object properties and methods in the runtime,
    as almost all of the built-in interfaces can be accessed from the property chain begun by \code{global} object.

Firstly,
    \sysname uses \code{Object.getOwnPropertyNames} to enumerate all of the properties of the initial object.
In our scenario,
    this object is \code{global} object.
Then,
    \sysname access this property of the object by its name,
    and determine the type of this property.
If the property is a function,
    \sysname record this property and gather more information such like argument length of this function.
If the property is a string or number,
    \sysname record this value for further analysis.
If the property is a object,
    \sysname uses recursively pass this object to the first step of our algorithm to analysis this object.
In the end,
    \sysname gather all of the functions and values and its access path for further analysis.

\CW{this section should have more contents,
    but I cannot produce more... (maybe writing some challenges \& solution?)}













% padding
% padding


==> paper/04_overview.tex <==
% High-level system design 

In this section,
    we introduce the overview of our \sysname and its workflow.
Then,
    we discuss the challenges we met and how we solved these.

\subsection{Overview}

\CW{I think firstly we should analysis gate interface, that is, if mini app could not exploit gate interface, the rest analysis is meaningless.}

The overview workflow of \sysname shown as Figure~\ref{fig:NULL}.
At the first beginning,
    we have to analyze the integrity of MiniProgram runtime before we analyze Service Abstraction Layer,
    that is,
    if the runtime of MiniProgram is well implemented with no vulnerability,
    the further analysis is not required as the attacker may not able to exploit SuperApp in our threat model.
When a vulnerable runtime is confirmed,
    we leverage static analysis against SuperApp to enumerate all of the APIs provided by Service Abstraction Layer.
To filter out Hidden APIs,
    we implement official document crawler to fetch all of the official APIs,
    and compare them to uncover all of the Hidden APIs.
To filter Privileged APIs from Hidden APIs,
    we set up an experiment to perform differential analysis and distinguish them.

\CW{Do we really need to present Privileged APIs? Cause I think the Hidden API is complex enough to understand, along with interfaces and functions etc. There are already too many definitions.}

We will give the detailed workflow in the next subsection.


\subsection{Workflow}

\CW{We need a workflow figure of our tool here.}

\noindent
\textbf{Check MiniProgram Runtime Integrity}
%  MiniProgram runtime  API ， MiniProgram  runtime  runtime  integrity。， FRIDA  MiniProgram ， V8 Engine  CpuProfiler  MiniProgram  profile， profile  MiniProgram  CpuProfiler 。 MiniProgram  profiler ，，， gate interface


\noindent
\textbf{Analyze SuperApp Service Abstraction Layer}
%  MiniProgram Runtime  vulnerable ， SuperApp  Service Abstraction Layer  API 。， Soot  SuperApp ， SuperApp  API  (i.e. API ).

\noindent
\textbf{Filter Hidden and Privileged APIs}
%  SuperApp  Service Abstraction Layer ， API。 SuperApp ， API （Official API）。 API  Official API  Hidden API。
%  Hidden API ， API  privileged。， MiniProgram  Hidden API 。， gate interface  Hidden API 。， Privileged API。

\noindent
\textbf{Exploit Hidden and Privileged APIs}
%  Hidden  Privileged API ， API  Service Abstraction Layer  data flow  control flow analysis， API 。， exploit  Application Layer  Service Abstraction Layer


To discover more vulnerabilities,
    we developed \sysname to automatically analysis Super Apps.

\sysname need open documents to build a base of APIs which is provided by official of Super Apps (step 1).
This procedure is various,
    as different vendors has different document structures,
    which is hard to implement a single crawler to be compatible with all of them.
Thus,
    the crawler is implemented manually to be compatible with different documents of Super Apps.

Then,
    \sysname statically analyze the package of Super Apps and generate a detailed analysis report (step 2).
As all of the APIs should be defined in framework layer from the architecture we previous presented,
    \sysname is able to analyze their package statically without running them,
    and giving a detailed analysis report which contains API name.

After the statically analysis,
    \sysname now is able to distinguish whether a API defined in framework layer is a hidden API or not (step 3).
In this step,
    \sysname collects the previous official APIs and APIs from analysis result,
    compares them and filters out hidden APIs.

In the last,
    \sysname gives all the parameters of hidden APIs by the static analysis report (step 4).
The parameters of API is vital to researchers to uncover more vulnerabilities of the corresponding hidden API.



% Official documents crawling ->
% WeChat MiniApp Runtime API enumerating ->
% Mapping ->
% uncovering & exploiting vulnerabilities




\subsection{Challenges and Solutions}

To attack from Application Layer straight down to Framework Layer requires plenty of reverse engineering works,
    to reduce the manual procedures,
    we developed this systematic analysis tool set.
Our tool needs to solve many challenges set by vendors of Super Apps.

\noindent
\CW{This one is indeed a great challenge, but maybe too weak in this research paper?}

\noindent
\textbf{Challenge \#1 Architecture and Workflow of Mini Program}
The first challenge we met is to build a whole and clear picture of Mini Program.
From the existing documents and publications of Mini Program,
    it is far more sufficient to build such a big picture.
More than that,
    analyzing Android package of Super Apps is also a challenge,
    as all of the Super Apps we are investigating are using obfuscation to protect their packages,
    and the method/class names after obfuscation is changing through the version iteration.


\noindent
\textbf{Solution to \#1}
To solve this challenge,
    we deeply investigated \wechat,
    leverage domain knowledge of reverse engineering to fully build the entire workflow of API invoke.
More than that,
    we then investigated other Super Apps,
    and discovered that they are sharing the similar architecture and workflow,
    that our picture is compatible to those Super Apps,
    and is able to analyze them sufficiently.

To avoid the impact of obfuscation of package in our tool implementation,
    we investigated the package of \wechat,
    and find out a set of classes are preserved for Java reflection.
Thus,
    we follow the execution flow of these classes and leverage heap memory searching techniques to implement our dynamic analysis tools,
    which are completely compatible to any recent version of Super Apps.

% This means our work is the first one to build a whole picture of Mini Program workflow,
%     introducing vulnerabilities of the implementation of Mini Programs.

\noindent
\textbf{Challenge \#1 Uncover Gate Interface in JavaScript Runtime}
A critical part in our threat model is,
    a gate interface should present in MiniProgram runtime,
    and can be accessed by MiniProgram.
However,
    as we discussed before,
    MiniProgram is a complete black-box for us when implementing analysis tools,
    and there is no official support for us to analyze the runtime.

\noindent
\textbf{Solution to Challenge \#1}
To solve this challenge,
% comment: keep this line if the previous challenge is dropped
    we take a great effort in reverse engineering the runtime implementation of SuperApp.
% After we build a whole picture of MiniProgram,
%     we are able to construct an analysis tool against runtime.
% % outline: V8 embedded CpuProfiler -> We leverage this profiler by DBI -> generate profile by implementing profile transformer and inject into process -> analyze profile to uncover gate interface
% % ， SuperApp  V8 Engine  MiniProgram  runtime， V8 Engine  CpuProfiler 。， V8 Engine  CpuProfiler  FRIDA  MiniProgram  profile， profile  FRIDA  MiniProgram ， profile 。



\noindent
\textbf{Challenge \#2 Identify Privileged API}
APIs presents in Service Abstraction Layer may include documented APIs and undocumented APIs,
    within the undocumented APIs,
    there are also privileged APIs for other usage purposes.
% The privileged APIs often contains more arbitrary operations,
%     which may be leveraged by malicious attackers to exploit victim.
However,
    the official documents are only able to help us distinguish the documented APIs and undocumented APIs.
We are not able to filter out potential privileged APIs for further analysis. 

\noindent
\textbf{Solution to \#2}
To solve this challenge,
    we utilize dynamic analysis to invoke these APIs,
    and collecting execution results to identify them.

We use official developer tools to build a Mini Program,
    which will enumerate all of APIs which are provided by official and invoke them.
This invoke results will be collected,
    that an unofficial API invoke will be giving a \code{fail: permission denied} result.

Then,
    we use dynamic analysis to inject our scripts directly into the Mini Program runtime to evaluate and capture execution results from the Service Abstraction Layer by DBI.

After obtained the two set of results,
    we utilize differential analysis to distinguish the privileged APIs from the unofficial APIs.

\noindent
\CW{This one is pending for dispose}

\noindent
\textbf{Challenge \#3 API Parameter Extraction}
To exploit a privileged API,
    input data is also vital to researchers to analyze the implementation of API in Framework Layer.
However,
    the parameters in the implementation of API is obfuscated,
    and we need to identify the actual handler of API to analyze the parameters.

\noindent
\textbf{Solution to \#3}
To solve this challenge,
    we leverage our domain knowledge of reverse engineering,
    combining with dynamic tracing,
    finally build a entire data flow and control flow from Application Layer to Framework Layer.
This big picture greatly in help with the development of our tools,
    that we are able to tracing the path of parameters delivered from upper layer to the lower layer.
We first identified the actual handler method of the API classes,
    then perform data flow analysis against the incoming data from the upper layer,
    and finally extract the parameter names and their default values by analyzing the related invoke statements.

% 1st challenge
% official api crawling
% reverse engineering -> not able to distinguish official & hidden
% -> crawling

% 2nd challenge
% hidden api enumerate

% % 3rd challenge
% % mapping challenge

% 3rd challenge
% extract jsapi parameters

% exploit apis
% sensitive resources
% private apis
% manual analysis -> tools


% input all api
% output mismatch & potentially mismatch sensitive apis
% might be challenged by reviewers about string matching



% \subsection{Threat Model}
% 
% In our motivate example,
%     we discovered a series of vulnerabilities present in the framework of Super Apps.
% The exploits of these vulnerabilities are all based on a single implementation flaw,
%     which is simple but fatal.
% Thus,
%     for an attacker,
%     writing a malicious Mini Program which contains exploits of these vulnerabilities is completely feasible.
% 
% In our threat model,
%     all things an attacker have to do is phishing victims to open a malicious Mini Program on the Android phone of victim.
% Considering the features of Mini Programs,
%     instant, light weighted and easy to share can reduce the cost of distribution massively.
% Considering the distribution methods of Mini Programs,
%     friend and community sharing, QR code scanning and inter-MiniProgram navigation can make malicious Mini Program execute instantly,
%     even not requiring the confirmation and permission from users.



% attacker may phish victim to run a malicious MiniApp on the device of victim
% **scope** Android version













% padding
% padding


==> paper/05_implementation.tex <==

In this section,
    we introduce the methods to analyze integrity of MiniProgram runtime,
    and uncover Hidden APIs.

\subsection{Analyze the Integrity of MiniProgram Runtime}

%  runtime  vulnerable ， SuperApp  runtime  JavaScript Framework Layer  Application Layer ，。
% ， JavaScript Framework Layer  gate interface， JavaScript (i.e. eval)。， gate interface，，， API  gate interface。

%  JavaScript （ Jalangi2 *cite here*） JavaScript （）， MiniProgram  JavaScript Framework Layer ， SuperApp  runtime ， Runtime 。， lite but powerful  trace JavaScript Framework Layer 

% ， SuperApp  V8 Engine  MiniProgram  runtime。，V8 Engine  CpuProfiler ，， MiniProgram Runtime。， Frida  MiniProgram process  instrument。， V8  CpuProfiler 。

%  V8 Engine  CpuProfiler ，\footnote{ profiler  v8::CpuProfiler::New}， frida  NativeFunction ， V8 Engine  Profiler。 API ， profiler  startProfiling  profiling。 API ， profiler  stopProfiling  profiling  API  JavaScript  sample profile。

%  sample profile ， profile ， stopProfiling  profile  profile 。， C++  profile ，， Linux (i.e. dlopen  dlsym) MiniProgram runtime ， frida  profile  V8 CpuProfile 。

% ，V8 Engine ， Frida attach  V8 Engine 。，， V8 Engine （i.e. v8::Isolate::GetCurrent）。，， V8 Engine 。



%  API  CpuProfiler  profile ， profile ，~\ref{fig:flamegraph}。

% ，：1)  X , 2) Y   3) (i.e. xx  xx )。，，，。， gate interface  Native Layer  JavaScript ， API  JavaScript ，gate interface 。

% ，。， native ， JavaScript ，。 tricky ， exitMiniProgram API， MiniProgram  gate interface 。

\subsection{Uncover Hidden and Privileged APIs}

% outline
% 1.  API  （getStorageSync  Service Abstraction Layer）
% 2. API 
% 3.  API /

% API implementation 
% 1. Parameter
% 2. Super Class
% 3. return type
% 4. Caller (Xref)
% 5. package name
% 6. method/class annotation
% 0. Symbolic Execution

%  MiniProgram Runtime  vulnerable ， SuperApp  Service Abstraction Layer  Service Abstraction Layer  API。 Android ，Service Abstraction Layer  Java ， JavaScript Framework Layer 。， Service Abstraction Layer  API 。

%  listing （maybe not）

% ， API  SuperApp ， API 。， API  SuperApp ，。 API  Service Abstraction Layer （package）（class）， API ，。，，，。

%  API  Service Abstraction Layer ，。 SuperApp  API ：1) Parameter，API ；2) Super Class，API  Java ， API  API ；3) return type，，API ；4) Caller， API ，；5) package name， API ；6) class/method annotation， API  API 。

% ，

% ， API 。，，， API ，。， API  pattern  API （ API ）， API 。

%% ：，， SuperApp ， pattern， API 。

% ， API。，，，， API 。 API  Service Abstraction Layer  API ， Hidden API。

%  Hidden API ， API  Privileged API。
%  API  JavaScript Framework Layer ， differential analysis  Hidden API 。 MiniProgram  API  API ，。， MiniProgram Runtime  JavaScript ， gate interface  API，。，， API  \code{fail: permission denied} ， gate interface ， API  Privileged API。






==> paper/05_mapping.tex <==

% Diff → Mapping → Access control breach

% Interfaces:
% 1. Documented APIs
% 2. Undocumented APIs (privileged official APIs/deprecated APIs & other Runtime functions/methods) (dangerous internal functions)

% Challenges:
% 1. Automatically analysis
% 2. Vulnerabilities discovery
% 3.

% Static analysis: Soot + flowdroid 
%                  -> enumerate APIs (official & hidden)
% Dynamic analysis: Attach to production V8 VM 
%                  -> execute scripts 
%                  -> enumerate APIs (official & hidden) & Interfaces

% Additional in dynamic analysis: 
%           running different MiniPrograms in production runtime 
%               -> execute our scripts 
%               -> compare results to kill false-positives

% Threats
% 1. Break integrity of V8 runtime (i.e. MiniProgram runtime)
% 2. Access sensitive functionality (e.g. File System, Hardware sensors, e.t.c)
% 3. Exploit WeChat main process via Binder IPC by breaking process isolation

% Why only WeChat and QQ:
% our tool is implemented based on 
% the aspect of similar (same) arch
% of the Super Apps,
% thus, it will be super easy to 
% work on other Super Apps with
% a little slight modification

In this section,
    we introduce the interfaces mapping and the methods to uncovering other hidden APIs in WeChat MiniProgram framework.


\subsection{Mapping Interfaces}

In section~\ref{sec:enumerate},
    we obtain the information of interfaces from official open documents and local MiniProgram runtime environment.
After the collected data,
    we try to compare them and gather different interfaces.

\CW{I really dont know how to write this part cause the local script has too many duplicate items and I am trying to avoid them...
And in here maybe we should talk about more state-of-art techniques (NLP xD)?
Actually I did not pay much attention on this script but on the \code{NativeGlobal} object...
}

Balabala...

% following maybe should be put in further sections...
According the mapping result,
    one interface needs to be specially concerned named \code{NativeGlobal}.
Like its name and compare to \code{global},
    \code{NativeGlobal} is a interface which is implemented by native libraries and inject into \code{V8} runtime engine.
We manually investigated this library by static analysis,
    and then noticed this library contains a vital \textbf{Bridge} in communicating with framework layer.
Thus,
    this interface plays a role of gate to guard the upcoming data and the data of specific API invoke between native and framework layers.



\subsection{Uncovering Hidden APIs}

Combine with interfaces mapping result and manual static analysis of WeChat package,
    we find there are more kind of interfaces that malicious attacker may use to compromise the MiniProgram framework.

\noindent
\textbf{Hidden APIs}

As we discussed before,
    API is a kind of special interfaces that needs application, native and framework layers to work together to complete specific behaviors.
Unlike APIs,
    the interfaces we discussed before is a set of functions that only works on native layer,
    which do not involve framework layer to obtain more sensitive privileges.

However,
    during our further investigation of WeChat Android packages,
    we discovered there are another series of APIs defined in framework layer to provide more features.

An obvious way to distinguish a small set of hidden API is simply by its name,
    such as a \code{private\_} prefix in the API name field defined in the framework.
For example,
    an open web page API named \code{wx.openUrl} is forbidden for normal developers,
    however,
    a malicious attacker may use \code{private\_openUrl} API directly by bypassing the check in application layer though \code{NativeGlobal} interface as we talked before.

\CW{needs to review here...}

Due to hidden APIs are invisible to normal developers,
    WeChat official may take much less care about the security of these APIs,
    which are easily vulnerable to malicious attackers.

\CW{I think here should explain the detail information of a \code{JsApi}...}

\noindent
\textbf{JsApi}

In order to help our analysis,
    through reverse engineering of WeChat Android package,
    we conclude multiple critical characteristics of an API.
These APIs in WeChat official open documents are named \code{JsApi},
    therefore,
    we use \code{JsApi} to refer to the APIs present in framework layer we are analyzing.

Shown in Listing~\ref{lst:jsapimodel},
    a \code{JsApi} contains the following parts.

\begin{enumerate}[1]
    \item \textbf{Class Name} The name of the JsApi class,
        which will be very helpful in the further analysis.
    \item \textbf{Api Name} The name of the JsApi,
        which can indexed by WeChat MiniProgram framework and be invoked by \code{NativeGlobal}.
    \item \textbf{Control Index} WeChat framework using this index to control the permission of the API invoke,
        such as insufficient permission in background usage of camera or microphone APIs.
    \item \textbf{Parameters} The parameters that the API needs to fulfill its features.
    \item \textbf{Api Type} The type of the API.
        WeChat defined two types of APIs: 1) synchronous APIs and 2) asynchronous APIs to meet different usage requirements.

\end{enumerate}

\ignore{
\begin{minted}[linenos,fontsize=\footnotesize,xleftmargin=.065\textwidth]{Java}
public enum Type {
    JS_API_SYNC,
    JS_API_ASYNC,
    NONE
}

public Param implements Serializable {
    public String type;
    public String name;
    public String value;
}

public JsApi implements Serializable {
    public String className;
    public String apiName;
    public int ctrlIndex;
    public Set<Param> params;
    public Type type;
}
\end{minted}
}


\lstset{style=myjavalistingstyle}
\begin{lstlisting}[
    language={Java},
    caption={JsApi Model Definition},
    label={lst:jsapimodel}
]
public enum Type {
    JS_API_SYNC,
    JS_API_ASYNC,
    NONE
}

public Param implements Serializable {
    public String type;
    public String name;
    public String value;
}

public JsApi implements Serializable {
    public String className;
    public String apiName;
    public int ctrlIndex;
    public Set<Param> params;
    public Type type;
}
\end{lstlisting}

In Listing~\ref{lst:jsapiclass},
    we take two typical \code{JsApi} classes to demonstrate.

\CW{Here needs some explanation of two demo...}

\begin{lstlisting}[
    language={Java},
    caption={Two Typical JsApi Classes},
    label={lst:jsapiclass}
]
// Async JsApi
public final class JsApiGetDeviceInfo extends JsApiAsync {
    public static final int CTRL_INDEX = 867;
    public static final String NAME = "getDeviceInfo";
    
    @Override
    public final void handle(IAppBrandComponent env, JSONObject data, int callbaclId) {
        String deviceInfo = AdDeviceInfo.getDeviceInfo(data.optString("imei"));
        env.doCallback(callbackId, deviceInfo);
    }
}

// Sync JsApi
public class JsApiGetSystemInfo extends JsApiSync {
    public static final int CTRL_INDEX = 40;
    public static final String NAME = "getSystemInfo";
    
    @Override
    public final String handle(IAppBrandComponent env, JSONObject data) {
        Map systemInfo = this.getInfo(env);
        return this.makeReturnJsonWithMap("ok", systemInfo);
    }
}
\end{lstlisting}

\noindent
\textbf{Static Analysis}

To uncover all of the hidden APIs present in framework layer,
    we adopt static analysis against WeChat Android package to automatically enumerate all of the APIs.

In the Android package,
    WeChat utilizes a very large number of inheritance features of Java,
    which help us a lot to distinguish implemented APIs from normal classes.
These APIs in Java bytecodes are extended from a single class named \code{AppBrandJsApi},
    and an implemented API has two static private fields: 1) \code{NAME} and 2) \code{CTRL\_INDEX}.
The former one is the name of that API,
    which can be directly invoked by \code{NativeGlobal} interface,
    and pass data to the specific handler of the API.
The latter one is the control index of that API,
    that WeChat framework using this index to control a part of the permission of the API.

In order to enumerate all of the APIs,
    we adopt \code{DexLib2} to statically analyze bytecodes of WeChat Android package.
First of all,
    \sysname loads the WeChat Android package into memory,
    create file input stream of all of the \code{dex} files.
    and initialize read buffer from these file stream for \code{DexLib2}.
Secondly,
    \sysname utilizes the \code{DexBackedDexFile} of \code{DexLib2} to create its instance,
    and gather all of the classes in these \code{dex} files.
Then,
    \sysname processes the first phase of filter.
From the previous gathered classes inside WeChat Android package,
    \sysname check the name of these classes,
    and filter out classes which names are beginning with a specific prefix
    \footnote{The prefix is \code{com.tencent.mm.plugin.appbrand.jsapi}}.
In another words,
    \sysname examines the classes are whether belong to a specific Java package or not.
If a class is match this signature,
    \sysname pushes them into an array and mark them as classes of \code{JsApi} package.
After obtained the array,
    \sysname processes the second phase of filter.
For each class of the array,
    \sysname inspects it for two private static fields 1) \code{NAME} and 2) \code{CTRL\_INDEX}.
If a class contains these two private static fields,
    \sysname will mark this as a valid \code{JsApi} class.
Finally,
    \sysname extract the name and control index of the API,
    and store them into an array for further analysis.


\subsection{Mapping APIs}

\CW{I'm considering put this section to the latter paragraph.}

From the previous analysis,
    we enumerate all of the APIs present in framework layer.
These APIs contain official APIs which are maintained by WeChat,
    and also contain hidden APIs which are in development or already deprecated,
    even official backdoor that only a set of MiniPrograms that developed by WeChat may use.

\CW{Here or in background we should talk about Inter-process Binder IPC of API workflow...}

Differ from hidden interfaces,
    as we demonstrated before,
    interfaces are works on native layer only,
    however,
    hidden APIs must need framework layer in operation.
This behavior may involve much more components of framework layer to handle the API invoke,
    such as Binder IPC to exchange data between WeChat main process and MiniProgram isolated process.
Thus,
    \sysname focus on the API mapping to uncover this mismatch behavior,
    and do further analysis on these hidden APIs.

During our investigation,
    we statically analysis the JavaScript codes of application layer,
    and discover that the APIs beginning with \code{wx.} described in open documents (such as \code{wx.getStorage}) are mapped to framework layer as \code{NAME} (the former corresponds to \code{NAME} is \code{getStorage}).
Combined with the previous analysis,
    we assert that all of the APIs discovered by static analysis are able to be invoked by \code{NativeGlobal} interface.

By applying this assumption,
    \sysname enumerates all of the APIs which are statically analyzed and maps to all of the APIs present in official documents.
After that,
    \sysname gathers all of the mismatch APIs,
    and mark them as hidden APIs which need to perform further analysis.

\CW{Seems that the implementation in this section is too short, I need to expand this...}





% \noindent
% \textbf{Static Analysis}
% According to WeChat open documentation,
%     developers can use APIs provided by WeChat to access network, hardware, file system, WeChat features, e.t.c.,
%     these APIs can be accessed by a global JavaScript object named \code{wx}.
% For example,
%     if a MiniProgram needs to cache a key-value data,
%     it can use \code{wx.setStorage(\{key: "key", data: "value"\})} to store that data.
% After the further reverse engineering of WeChat,
%     we discovered majority of these APIs are implemented in Android layer,
%     rather than V8 runtime.
% Thus,
%     we adopted \code{DexLib2} to statically analysis WeChat Android packages.
% 
% In Android packages,
%     WeChat utilizes a very large number of inheritance features of Java,
%     which help us a lot to distinguish implemented APIs from ordinary classes.
% These APIs in Java are extends from a single class named \code{AppBrandJsApi},
%     and an implemented API has two static private fields: \code{NAME} and \code{CTRL\_INDEX}.
% Therefore,
%     for the best performance,
%     we adopted \code{DexLib2} rather than \code{Soot} to implement our static analysis tool.
% \sysname will load the WeChat package into memory,
%     scan all of dex files (e.g. classes.dex) and generate file stream directly from memory,
%     disassemble them into smali,
%     and finally filter all the classes matches the characteristics we discovered above.
% 
% 
% \noindent
% \textbf{Dynamic Analysis}
% \review{Also put some dynamic analysis approaches here...}
% 
% 
% \subsection{Exploiting Interfaces}



==> paper/06_exploit.tex <==

In this section,
    we introduce the methods we implemented to further extract more information from WeChat Android packages,
    and exploit hidden APIs by these information.


\subsection{Extract JsApi Parameters}

As we discussed in Section~\ref{sec:mapping} and the \code{JsApi} example class in List~\ref{lst:jsapiclass},
    there are more information that \code{DexLib2} are inefficient to collect.
On Line 8 of the List~\ref{lst:jsapiclass},
    we can see that \code{JsApi} handler extract \code{imei} from the input JSON data,
    passing to \code{getDeviceInfo} to obtain device IMEI number.
In this demo,
    \code{imei} is the parameter that an API should examine to fulfill the specific features.
Thus,
    the parameters of an API is essential to further analysis.

% should be data flow analysis but I am not sure
As \code{DexLib2} is just a libraries providing dex file parsing,
    and this analysis needs more analytical techniques to be involved.
Therefore,
    we adopt \code{Soot} to track the data flow of the incoming JSON data to dump all of the parameters that an API may accept.

% still using DexLib2 for first phase 
% fast enumeration to enhance analysis 
% tool performance
% using Soot to do data flow analysis
% and extract all of the params


For a better analysis performance,
    we decide to reuse the previous framework API enumeration approach.
From the previous analysis,
    we obtained all of the classes of APIs,
    however,
    these classes are provided by \code{DexLib2},
    which need to be transformed into \code{Soot} classes.

Firstly,
    \sysname iterate the \code{JsApi} array and obtain each class name of the API.
After that,
    \sysname utilizes \code{Soot} to obtain \code{SootClass} instance of the API by the name of target class,
    and push them into a queue for further analysis.
When a queue is ready,
    \sysname pull instance from the queue and performing data flow analysis.

Before data flow analysis,
    \sysname needs to determine the handler method of a \code{JsApi} class.
Shown on List~\ref{lst:jsapiclass},
    we can see the prototype of a \code{JsApi} handler method.

\begin{itemize}
    \item \textbf{Asynchronous API}
        A asynchronous API handler method is taking three parameters:
            1) MiniProgram context,
            2) incoming JSON data and 3) invoke callback id.
        As an asynchronous API is not running in main thread but in another event thread,
            the framework layer needs to record the callback id to invoke corresponding callback methods.
    \item \textbf{Synchronous API}
        A synchronous API handler method is taking two parameters,
            MiniProgram context and incoming JSON data,
            and one return value processing result.
        Because synchronous API is processing in main thread,
            the processed string value are returned directly.
\end{itemize}

Also,
    these handler methods are inherited from the abstract methods of their parent classes,
    and override them to fulfill specific needs.

As the characteristics of the \code{JsApi} handler methods we described above,
    \sysname uses \code{Soot} to statically analyze these handler methods.
After obtaining the handler methods,
    \sysname is able to perform data flow analysis.
\sysname tags the second parameter of the handler methods,
    which is incoming JSON data,
    and tracks data flow of this variable.
If this tagged variable or the methods passing this variable contains invoke expression,
    \sysname analyze the invoke expression is whether an \code{opt} series JSON fetch value methods or not,
    such as \code{optString} and \code{optInt} etc.
If \sysname asserts the invoke expression is an \code{opt} series methods,
    it analysis the parameters of the invoke expression contains,
    which normally has one or two parameters:
    1) key of JSON object and 2) default value if the key is not exist.
When this expression contains only one parameter,
    \sysname convert the parameter to string value and store them in the database.
When this express contains two parameters,
    \sysname take the same operation on the first one and convert the second parameter into corresponding value,
    and finally take its string value into the database
    (e.g., \code{optInt("key", 10043)} will be convert into \code{"key"} and \code{"10043"}).

Also,
    \sysname maintains an map of these \code{opt} series methods,
    which maps method name to its value type,
    such as \code{optString} maps to \code{string} type and \code{optInt}, \code{optFloat} maps to \code{number} type.
This map is quiet helpful to our further analysis and exploits.

\CW{I don't know how to present data flow analysis cause I am not using that qaq.}


\CW{I think there are another aspect of mismatch: parameter mismatch
    (e.g., official gives two but we analyzed three parameters with one backdoor parameter),
    which maybe can be expand in the discussion of this paper or next work?}


% \subsection{Exploit Hidden APIs}

% \CW{I think in this section,
% it will be hard to tell how we do this exploit.
% Manually? Domain-knowledge? or something else that convincible/systematic...
% Actually I am doing this by my hand (aka. manually)
% }

% % automatically filter out sensitive APIs and resources
% % and inform developers to take care

% % sensitive resources life cycle
% % 1. create 2. delivery 3. access 4. destroy

% % why manually

% From the previous findings,
%     we have already gathered anything we need to perform the ultimate analysis: exploit the mismatch hidden APIs.
% In the previous phases,
%     \sysname has the hidden APIs and its parameters,
%     which has narrow down the scope our system needs to analysis.
% However,
%     there are still many APIs need to analysis.

% % so we need to present the challenge here 
% % that why we are not using automatic analysis
% % but manual processing
% In our investigation,
%     we discovered that \wechat framework is too complicate,
%     and the automatic analysis may facing a lot of roadblocks,
%     such as dead control flow and data flow of IPC,
%     obfuscation and dynamic analysis circumvention.

% Thus,
%     we implement \sysname to help researchers further narrow down the scope of the potential vulnerable hidden APIs.
% The post-analysis needs researchers to confirm manually.

% To address our key insights,
%     \sysname focuses on the suspicious hidden API names and the life cycle of sensitive resources.

% \noindent
% \textbf{Suspicious Names}
% For a quick filter,
%     \sysname firstly observer the names of hidden APIs.
% We implemented a set of keywords by empirical study,
%     including \code{private}, \code{native} and \code{straight} etc.
% In our empirical study,
%     the hidden APIs which contain these keywords are high probability of official backdoor or having vulnerabilities.

% Thus,
%     \sysname enumerates all of the hidden APIs,
%     and examine the name of API has specific patterns.
% If the name matches,
%     \sysname will mark the API as high risk hidden API.



% \noindent
% \textbf{Sensitive Resources Life Cycle}
% In order to propose a general discovery of vulnerabilities,
%     we define a life cycle of sensitive resources to help us systematically determine the critical ranking of a hidden API.

% To define the life cycle of sensitive resources,
%     we propose the following four parts of a complete life cycle.

% \begin{itemize}
%     \item \textbf{Create} The creation of sensitive resources,
%         such as \code{Intent} and task instance for IPC.
%     \item \textbf{Delivery} The delivery of sensitive resources,
%         such as the transmission of task instance between \wechat Mini-Program and main process.
%     \item \textbf{Access} The access of sensitive resources,
%         such as devices hardware APIs like Bluetooth.
%     \item \textbf{Destroy} The destroy of sensitive resources,
%         such as the deletion of sensitive file.
% \end{itemize}

% After we defined the life cycle,
%     we are now able to implement our approach to analyze \wechat framework.
% We firstly collected a set of sensitive resources APIs,
%     and analyze its methods to gather a group of sensitive methods.

% \CW{actually, my tool hasn't implement this part, so I don't know how to make it making sense (so do the first part in this section)... can I left this part to Yue (x }



\noindent
\textbf{Manual Analysis}
In the last,
    we now obtain a small set of hidden APIs,
    and are able to perform complete further analysis against them.

\CW{I don't know how to present manual analysis...}

% To demonstrate our analysis approach,
%     we also take Section~\ref{sec:motivation} for the example.
On the one hand,
    we use static analysis tools (i.e., JADX) to analyze corresponding hidden API handler method,
    and trying to analyze data flow and control flow within the method.
In a major part of hidden APIs,
    they use Binder IPC to send specific task request to \wechat main process.
Regarding to the IPC workflow,
    the dead control and data flow can be analyzed manually,
    and researchers may discover vulnerabilities which leads to sensitive resources.

On the other hand,
    we also use dynamic analysis tools (i.e., Frida) to dynamically instruct the specific methods.
For an instance,
    shown in List~\ref{lst:jsapiclass},
    we can record and intercept the \code{doCallback} method and \code{makeReturnJsonWithMap} method to obtain the execution stack,
    invoke parameters and return values.





\CW{Maybe we can say that we used static analysis to discover vulnerabilities and utilized dynamic analysis to verify the vulnerabilities}













% padding 
% padding 
% padding 


==> paper/cheat-classification-figure.tex <==
\begin{figure*}[t]
        \centering
        %\resizebox{\columnwidth}{!} 
        {\includegraphics[width=7in]{images/hkk_countermeasure.png}}
        \caption{\hkk{Overview of online game security countermeasures.\ZQ{This figure looks nice. The resolution of this figure isn't good. Can you please share the source of this figure? We may need to consolidate this figure with Table 1}} \hkk{got it. see the fig1.pptx . you can freely modify the file. }}
        \label{fig:game_countermeasure}
\end{figure*}



==> paper/cheat-classification-tbl.tex <==

\begin{table*}[t]
\centering
\caption{\hkk{Cheating detection methods on client-, network-, and server-side (will be re-written and polished)}}
\label{table:cheating_detection_method}

\scalebox{0.80}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
                                                              & \textbf{Method}                                                                          & \textbf{Example}                                                                                                                           & \textbf{Drawback}                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Client-side detection}}  & Signature-based                                                                          & PunkBuster                                                                                                                                 & - Only works for well-known cheats.                                                                                                                             \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Third-party security\\ solution\end{tabular}                  & Hackshield, GameGuard                                                                                                                      & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}- Occupying client's resources.\\ - Conflict with other security solution,\\ AV, or even system kernel\end{tabular}} \\ \cline{2-3}
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Game devloper's security\\ solution\end{tabular}              & Blizzard's Warden Client, TenGuard, NexonGuard                                                                                             &                                                                                                                                                                 \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & In-game trap                                                                             & Invisible NPC (Non-Player Character), dummy, or item                                                                                       & - Temporal method (trap only valid until unveiled)                                                                                                                    \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & Anti-debugger                                                                            & Themida, ArXan                                                                                                                             & - Game client might crash because of anti-debugging routines                                                                                                    \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Network-side detection}} & Payload encryption                                                                       & -                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}- High latency, more computing power\\  needed for en/decryption\end{tabular}                                                        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Packet header checking\\ (e.g. TTL, window size)\end{tabular} & -                                                                                                                                          & - High FP rate, heavy analysis cost                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Server-side detection}}  & \begin{tabular}[c]{@{}l@{}}In-game log analysis\\ Data mining\end{tabular}               & AION by NCSoft                                                                                                                             & \begin{tabular}[c]{@{}l@{}}- Low availability\\ - Performance degradation because of client activity analysis\end{tabular}                                      \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & Out-game log analysis                                                                    & \begin{tabular}[c]{@{}l@{}}Windows event sequence, geographical location, \\ input patterns from HID (Human Interface Device)\end{tabular} & - Privacy issue                                                                                                                                                 \\ \hline
\end{tabular}
}
\end{table*}







==> paper/cheat-examples-tbl.tex <==
% \begin{table*}[t]
% \centering
% \caption{\hkk{Cheating examples in FPS game}}
% \label{table:cheating_example}
% \begin{tabular}{l|p{7cm}|p{7cm}|}
% \cline{2-3}
%                                              & \textbf{Cheating examples in FPS game}  
%                                              & \textbf{Countermeasure}                                                                         \\ \hline
% \multicolumn{1}{|l|}{\textbf{Application-level}}  & Aimbot, triggerbot, world-hacking, ESP, Twinking, Scriptting, Game element manipulation 
% % & Signature-based, developer's/third-party's security solution, software obfuscation,  Sandboxing 
% \\ \hline
% \multicolumn{1}{|l|}{\textbf{OS-level}}      & Graphical data manipulation, Rapid firing assistance
% % & Verifying (graphic) driver sign                                                                   
% \\ \hline
% \multicolumn{1}{|l|}{\textbf{Network-level}} & Network lag induction, disconnecting 
% % & DDoS mitigation techniques                                                                      
% \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
\begin{tabular}{c|l|}
\cline{2-2}
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{Cheating examples in FPS games}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Application-level}} & \begin{tabular}[c]{@{}l@{}}Game element manipulation, World-hacking, \\ WSP, Scriptting\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{OS-level}} & \begin{tabular}[c]{@{}l@{}}Aim-bot, Map-hack, Graphical data manipulation, \\  Wall-hack, Rapid firing assistance \end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{Network-level}} & Network lag induction, Disconnecting \\ \hline
\end{tabular}
\caption{Cheating examples in FPS games}
\label{table:cheating_example}
\end{table}

==> tables/api-cat-heatmap.bak.tex <==
\begin{table*}[h]
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1.2}
\scriptsize

 
\begin{tabular}{clcrcrcr|crcrcr|crcrcr|crcrcr|crcrcr}
\toprule[1.5pt]

    \multicolumn{2}{c}{
        \multirow{2}{*}{\textbf{Available APIs}}} &

    \multicolumn{6}{c}{
        \textbf{WeChat}
    } &
    \multicolumn{6}{c}{
        \textbf{WeCom}
    } &
    \multicolumn{6}{c}{
        \textbf{Baidu}
    } & 
    \multicolumn{6}{c}{
        \textbf{TikTok}
    } & 
    \multicolumn{6}{c}{
        \textbf{QQ}
    } \\
    \cline{3-32}

    \multicolumn{2}{c}{} &
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} \\ 

\midrule[0.5pt]

\multirow{4}{*}{Base}  &  Basic                  & 5 & 71.4 & 2 & \ccell{2}{7}{28.6} & - & \ccell{0}{7}{0.0} & 6 & 66.7 & 3 & \ccell{3}{9}{33.3} & - & \ccell{0}{9}{0.0} & 7 & 72.7 & 4 & \ccell{2}{11}{18.2} & - & \ccell{1}{11}{9.1} &   7  & 63.6 &   4  & \ccell{4}{11}{36.4} &  0 & \ccell{0}{11}{0.0} & 3 & 100.0 & - & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0}\\ 
     &  App                    & 13 & 39.4 & 14 & \ccell{14}{33}{42.4} & 6 & \ccell{6}{33}{18.2} & 13 & 37.1 & 16 & \ccell{16}{35}{45.7} & 6 & \ccell{6}{35}{17.1} & 6 & 42.1 & 6 & \ccell{10}{19}{52.6} & - & \ccell{1}{19}{5.3} &   6  & 50.0 &   6  & \ccell{6}{12}{50.0} &  0 & \ccell{0}{12}{0.0} & 9 & 34.6 & 17 & \ccell{17}{26}{65.4} & - & \ccell{0}{26}{0.0}\\ 
     &  Debug                  & 15 & 88.2 & 2 & \ccell{2}{17}{11.8} & - & \ccell{0}{17}{0.0} & 15 & 88.2 & 2 & \ccell{2}{17}{11.8} & - & \ccell{0}{17}{0.0} & - & 3.3 & - & \ccell{28}{30}{93.3} & - & \ccell{1}{30}{3.3} &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & 20 & 100.0 & - & \ccell{0}{20}{0.0} & - & \ccell{0}{20}{0.0}\\ 
     &  Misc                   & 10 & 58.8 & 7 & \ccell{7}{17}{41.2} & - & \ccell{0}{17}{0.0} & 10 & 55.6 & 8 & \ccell{8}{18}{44.4} & - & \ccell{0}{18}{0.0} & 10 & 100.0 & 9 & \ccell{0}{9}{0.0} & - & \ccell{0}{9}{0.0} &  10  & 52.6 &   9  & \ccell{9}{19}{47.4} &  0 & \ccell{0}{19}{0.0} & 9 & 100.0 & - & \ccell{0}{9}{0.0} & - & \ccell{0}{9}{0.0}\\ \hhline{*{32}{-}}
\multirow{5}{*}{UI}  &  Interaction            & 6 & 46.2 & 7 & \ccell{7}{13}{53.8} & - & \ccell{0}{13}{0.0} & 6 & 46.2 & 7 & \ccell{7}{13}{53.8} & - & \ccell{0}{13}{0.0} & 9 & 41.2 & 2 & \ccell{10}{17}{58.8} & - & \ccell{0}{17}{0.0} &   9  & 81.8 &   2  & \ccell{2}{11}{18.2} &  0 & \ccell{0}{11}{0.0} & 6 & 40.0 & 9 & \ccell{9}{15}{60.0} & - & \ccell{0}{15}{0.0}\\ 
     &  Navigation             & 4 & 44.4 & 5 & \ccell{5}{9}{55.6} & - & \ccell{0}{9}{0.0} & 4 & 40.0 & 6 & \ccell{6}{10}{60.0} & - & \ccell{0}{10}{0.0} & 5 & 100.0 & - & \ccell{0}{4}{0.0} & - & \ccell{0}{4}{0.0} &   5  & 100.0 &  0 & \ccell{0}{5}{0.0} &  0 & \ccell{0}{5}{0.0} & 4 & 33.3 & 8 & \ccell{8}{12}{66.7} & - & \ccell{0}{12}{0.0}\\ 
     &  Animation              & 32 & 100.0 & - & \ccell{0}{32}{0.0} & - & \ccell{0}{32}{0.0} & 32 & 100.0 & - & \ccell{0}{32}{0.0} & - & \ccell{0}{32}{0.0} & 1 & 95.5 & - & \ccell{1}{22}{4.5} & - & \ccell{0}{22}{0.0} &   1  & 100.0 &  0 & \ccell{0}{1}{0.0} &  0 & \ccell{0}{1}{0.0} & 31 & 100.0 & - & \ccell{0}{31}{0.0} & - & \ccell{0}{31}{0.0}\\ 
     &  WebView                & - & 0.0 & 22 & \ccell{22}{23}{95.7} & 1 & \ccell{1}{23}{4.3} & - & 0.0 & 24 & \ccell{24}{25}{96.0} & 1 & \ccell{1}{25}{4.0} & - & 0.0 & 3 & \ccell{3}{4}{75.0} & - & \ccell{1}{4}{25.0} &   0  & 0.0 &   3  & \ccell{3}{3}{100.0} &  0 & \ccell{0}{3}{0.0} & - & 0.0 & 16 & \ccell{16}{16}{100.0} & - & \ccell{0}{16}{0.0}\\ 
     &  Misc                   & 20 & 27.0 & 54 & \ccell{54}{74}{73.0} & - & \ccell{0}{74}{0.0} & 20 & 25.6 & 58 & \ccell{58}{78}{74.4} & - & \ccell{0}{78}{0.0} & 14 & 77.1 & 5 & \ccell{11}{48}{22.9} & - & \ccell{0}{48}{0.0} &  14  & 73.7 &   5  & \ccell{5}{19}{26.3} &  0 & \ccell{0}{19}{0.0} & 18 & 42.9 & 24 & \ccell{24}{42}{57.1} & - & \ccell{0}{42}{0.0}\\ \hhline{*{32}{-}}
\multirow{5}{*}{Network}  &  Request                & 5 & 55.6 & 4 & \ccell{4}{9}{44.4} & - & \ccell{0}{9}{0.0} & 5 & 55.6 & 4 & \ccell{4}{9}{44.4} & - & \ccell{0}{9}{0.0} & 6 & 66.7 & 4 & \ccell{1}{3}{33.3} & - & \ccell{0}{3}{0.0} &   6  & 60.0 &   4  & \ccell{4}{10}{40.0} &  0 & \ccell{0}{10}{0.0} & 4 & 66.7 & 2 & \ccell{2}{6}{33.3} & - & \ccell{0}{6}{0.0}\\ 
     &  Download               & 7 & 24.1 & 21 & \ccell{21}{29}{72.4} & 1 & \ccell{1}{29}{3.4} & 7 & 23.3 & 22 & \ccell{22}{30}{73.3} & 1 & \ccell{1}{30}{3.3} & - & 100.0 & 4 & \ccell{0}{11}{0.0} & - & \ccell{0}{11}{0.0} &   0  & 0.0 &   4  & \ccell{4}{4}{100.0} &  0 & \ccell{0}{4}{0.0} & 6 & 60.0 & 4 & \ccell{4}{10}{40.0} & - & \ccell{0}{10}{0.0}\\ 
     &  Upload                 & 7 & 50.0 & 5 & \ccell{5}{14}{35.7} & 2 & \ccell{2}{14}{14.3} & 7 & 46.7 & 6 & \ccell{6}{15}{40.0} & 2 & \ccell{2}{15}{13.3} & - & 100.0 & 4 & \ccell{0}{6}{0.0} & - & \ccell{0}{6}{0.0} &   0  & 0.0 &   4  & \ccell{4}{4}{100.0} &  0 & \ccell{0}{4}{0.0} & 6 & 75.0 & 2 & \ccell{2}{8}{25.0} & - & \ccell{0}{8}{0.0}\\ 
     &  Websocket              & 14 & 93.3 & 1 & \ccell{1}{15}{6.7} & - & \ccell{0}{15}{0.0} & 14 & 93.3 & 1 & \ccell{1}{15}{6.7} & - & \ccell{0}{15}{0.0} & 7 & 100.0 & 2 & \ccell{0}{13}{0.0} & - & \ccell{0}{13}{0.0} &   7  & 77.8 &   2  & \ccell{2}{9}{22.2} &  0 & \ccell{0}{9}{0.0} & 13 & 86.7 & 2 & \ccell{2}{15}{13.3} & - & \ccell{0}{15}{0.0}\\ 
     &  Misc                   & 23 & 88.5 & 3 & \ccell{3}{26}{11.5} & - & \ccell{0}{26}{0.0} & 23 & 85.2 & 4 & \ccell{4}{27}{14.8} & - & \ccell{0}{27}{0.0} & - & 0.0 & - & 0.0 & - & 0.0 &  0 & 0.0 &  0 & 0.0 &  0 & 0.0 & 10 & 55.6 & 8 & \ccell{8}{18}{44.4} & - & \ccell{0}{18}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{Storage}   & 10 & 66.7 & 5 & \ccell{5}{15}{33.3} & - & \ccell{0}{15}{0.0} & 10 & 66.7 & 5 & \ccell{5}{15}{33.3} & - & \ccell{0}{15}{0.0} & 10 & 100.0 & 1 & \ccell{0}{10}{0.0} & - & \ccell{0}{10}{0.0} &  10  & 90.9 &   1  & \ccell{1}{11}{9.1} &  0 & \ccell{0}{11}{0.0} & 10 & 83.3 & 2 & \ccell{2}{12}{16.7} & - & \ccell{0}{12}{0.0}\\ \hhline{*{32}{-}}
\multirow{8}{*}{Media}  &  Map                    & 8 & 14.3 & 48 & \ccell{48}{56}{85.7} & - & \ccell{0}{56}{0.0} & 8 & 14.3 & 48 & \ccell{48}{56}{85.7} & - & \ccell{0}{56}{0.0} & 6 & 100.0 & - & \ccell{0}{7}{0.0} & - & \ccell{0}{7}{0.0} &   6  & 100.0 &  0 & \ccell{0}{6}{0.0} &  0 & \ccell{0}{6}{0.0} & 9 & 36.0 & 16 & \ccell{16}{25}{64.0} & - & \ccell{0}{25}{0.0}\\ 
     &  Image                  & 6 & 60.0 & 4 & \ccell{4}{10}{40.0} & - & \ccell{0}{10}{0.0} & 6 & 60.0 & 4 & \ccell{4}{10}{40.0} & - & \ccell{0}{10}{0.0} & 5 & 85.7 & 1 & \ccell{1}{7}{14.3} & - & \ccell{0}{7}{0.0} &   5  & 83.3 &   1  & \ccell{1}{6}{16.7} &  0 & \ccell{0}{6}{0.0} & 6 & 60.0 & 4 & \ccell{4}{10}{40.0} & - & \ccell{0}{10}{0.0}\\ 
     &  Video                  & 14 & 35.0 & 26 & \ccell{26}{40}{65.0} & - & \ccell{0}{40}{0.0} & 14 & 31.8 & 30 & \ccell{30}{44}{68.2} & - & \ccell{0}{44}{0.0} & 8 & 95.0 & 2 & \ccell{1}{20}{5.0} & - & \ccell{0}{20}{0.0} &   8  & 80.0 &   2  & \ccell{2}{10}{20.0} &  0 & \ccell{0}{10}{0.0} & 14 & 63.6 & 8 & \ccell{8}{22}{36.4} & - & \ccell{0}{22}{0.0}\\ 
     &  Audio                  & 64 & 84.2 & 9 & \ccell{9}{76}{11.8} & 3 & \ccell{3}{76}{3.9} & 64 & 79.0 & 14 & \ccell{14}{81}{17.3} & 3 & \ccell{3}{81}{3.7} & 44 & 100.0 & 10 & \ccell{0}{44}{0.0} & - & \ccell{0}{44}{0.0} &  44  & 81.5 &  10  & \ccell{10}{54}{18.5} &  0 & \ccell{0}{54}{0.0} & 61 & 85.9 & 10 & \ccell{10}{71}{14.1} & - & \ccell{0}{71}{0.0}\\ 
     &  Live                   & 26 & 46.4 & 30 & \ccell{30}{56}{53.6} & - & \ccell{0}{56}{0.0} & 26 & 39.4 & 40 & \ccell{40}{66}{60.6} & - & \ccell{0}{66}{0.0} & 19 & 100.0 & - & \ccell{0}{8}{0.0} & - & \ccell{0}{8}{0.0} &  19  & 100.0 &  0 & \ccell{0}{19}{0.0} &  0 & \ccell{0}{19}{0.0} & 23 & 57.5 & 17 & \ccell{17}{40}{42.5} & - & \ccell{0}{40}{0.0}\\ 
     &  Recorder               & 16 & 84.2 & 3 & \ccell{3}{19}{15.8} & - & \ccell{0}{19}{0.0} & 16 & 84.2 & 3 & \ccell{3}{19}{15.8} & - & \ccell{0}{19}{0.0} & 11 & 100.0 & 1 & \ccell{0}{12}{0.0} & - & \ccell{0}{12}{0.0} &  11  & 91.7 &   1  & \ccell{1}{12}{8.3} &  0 & \ccell{0}{12}{0.0} & 15 & 88.2 & 2 & \ccell{2}{17}{11.8} & - & \ccell{0}{17}{0.0}\\ 
     &  Camera                 & 9 & 60.0 & 6 & \ccell{6}{15}{40.0} & - & \ccell{0}{15}{0.0} & 9 & 52.9 & 8 & \ccell{8}{17}{47.1} & - & \ccell{0}{17}{0.0} & 20 & 50.0 & 1 & \ccell{9}{18}{50.0} & - & \ccell{0}{18}{0.0} &  20  & 95.2 &   1  & \ccell{1}{21}{4.8} &  0 & \ccell{0}{21}{0.0} & 4 & 36.4 & 7 & \ccell{7}{11}{63.6} & - & \ccell{0}{11}{0.0}\\ 
     &  Misc                   & 12 & 75.0 & 3 & \ccell{3}{16}{18.8} & 1 & \ccell{1}{16}{6.3} & 12 & 75.0 & 3 & \ccell{3}{16}{18.8} & 1 & \ccell{1}{16}{6.3} & - & 100.0 & - & \ccell{0}{18}{0.0} & - & \ccell{0}{18}{0.0} &  0 & 0.0 &  0 & 0.0 &  0 & 0.0 & 6 & 100.0 & - & \ccell{0}{6}{0.0} & - & \ccell{0}{6}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{Location}     & 3 & 42.9 & 4 & \ccell{4}{7}{57.1} & - & \ccell{0}{7}{0.0} & 3 & 42.9 & 4 & \ccell{4}{7}{57.1} & - & \ccell{0}{7}{0.0} & 3 & 100.0 & - & \ccell{0}{7}{0.0} & - & \ccell{0}{7}{0.0} &   3  & 100.0 &  0 & \ccell{0}{3}{0.0} &  0 & \ccell{0}{3}{0.0} & 3 & 100.0 & - & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{Share}   & 4 & 33.3 & 7 & \ccell{7}{12}{58.3} & 1 & \ccell{1}{12}{8.3} & 4 & 16.7 & 19 & \ccell{19}{24}{79.2} & 1 & \ccell{1}{24}{4.2} & 5 & 100.0 & 2 & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0} &   5  & 71.4 &   2  & \ccell{2}{7}{28.6} &  0 & \ccell{0}{7}{0.0} & 5 & 35.7 & 9 & \ccell{9}{14}{64.3} & - & \ccell{0}{14}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{Canvas}  & 60 & 74.1 & 21 & \ccell{21}{81}{25.9} & - & \ccell{0}{81}{0.0} & 60 & 74.1 & 21 & \ccell{21}{81}{25.9} & - & \ccell{0}{81}{0.0} & 49 & 92.0 & 1 & \ccell{4}{50}{8.0} & - & \ccell{0}{50}{0.0} &  49  & 98.0 &   1  & \ccell{1}{50}{2.0} &  0 & \ccell{0}{50}{0.0} & 48 & 92.3 & 4 & \ccell{4}{52}{7.7} & - & \ccell{0}{52}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{File}  & 39 & 97.5 & 1 & \ccell{1}{40}{2.5} & - & \ccell{0}{40}{0.0} & 39 & 92.9 & 3 & \ccell{3}{42}{7.1} & - & \ccell{0}{42}{0.0} & 34 & 100.0 & 1 & \ccell{0}{35}{0.0} & - & \ccell{0}{35}{0.0} &  34  & 97.1 &   1  & \ccell{1}{35}{2.9} &  0 & \ccell{0}{35}{0.0} & 37 & 97.4 & 1 & \ccell{1}{38}{2.6} & - & \ccell{0}{38}{0.0}\\ \hhline{*{32}{-}}
\multirow{7}{*}{Open API}  &  Login                  & 2 & 100.0 & - & \ccell{0}{2}{0.0} & - & \ccell{0}{2}{0.0} & 5 & 83.3 & 1 & \ccell{1}{6}{16.7} & - & \ccell{0}{6}{0.0} & 2 & 50.0 & - & \ccell{0}{6}{0.0} & - & \ccell{3}{6}{50.0} &   2  & 100.0 &  0 & \ccell{0}{2}{0.0} &  0 & \ccell{0}{2}{0.0} & 2 & 100.0 & - & \ccell{0}{2}{0.0} & - & \ccell{0}{2}{0.0}\\ 
     &  Navigate               & 2 & 33.3 & 2 & \ccell{2}{6}{33.3} & 2 & \ccell{2}{6}{33.3} & 2 & 22.2 & 5 & \ccell{5}{9}{55.6} & 2 & \ccell{2}{9}{22.2} & 7 & 100.0 & - & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0} &   7  & 100.0 &  0 & \ccell{0}{7}{0.0} &  0 & \ccell{0}{7}{0.0} & 2 & 50.0 & 1 & \ccell{1}{4}{25.0} & 1 & \ccell{1}{4}{25.0}\\ 
     &  User Info              & 2 & 16.7 & 7 & \ccell{7}{12}{58.3} & 3 & \ccell{3}{12}{25.0} & 5 & 23.8 & 13 & \ccell{13}{21}{61.9} & 3 & \ccell{3}{21}{14.3} & 2 & 10.0 & 13 & \ccell{6}{10}{60.0} & - & \ccell{3}{10}{30.0} &   2  & 13.3 &  13  & \ccell{13}{15}{86.7} &  0 & \ccell{0}{15}{0.0} & 2 & 28.6 & 4 & \ccell{4}{7}{57.1} & 1 & \ccell{1}{7}{14.3}\\ 
     &  Payment                & 1 & 3.4 & 13 & \ccell{13}{29}{44.8} & 15 & \ccell{15}{29}{51.7} & 1 & 3.2 & 15 & \ccell{15}{31}{48.4} & 15 & \ccell{15}{31}{48.4} & 1 & 50.0 & 1 & \ccell{0}{2}{0.0} & 1 & \ccell{1}{2}{50.0} &   1  & 33.3 &   2  & \ccell{1}{3}{33.3} &   1  & \ccell{1}{3}{33.3} & 2 & 22.2 & 7 & \ccell{7}{9}{77.8} & - & \ccell{0}{9}{0.0}\\ 
     &  Bio-Auth               & 3 & 27.3 & 3 & \ccell{3}{11}{27.3} & 5 & \ccell{5}{11}{45.5} & 3 & 21.4 & 6 & \ccell{6}{14}{42.9} & 5 & \ccell{5}{14}{35.7} & - & 0.0 & 1 & 0.0 & - & 0.0 &   0  & 0.0 &   1  & \ccell{1}{1}{100.0} &  0 & \ccell{0}{1}{0.0} & 3 & 100.0 & - & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0}\\ 
     &  Enterprise             & - & 0.0 & 1 & \ccell{1}{1}{100.0} & - & \ccell{0}{1}{0.0} & 5 & 17.9 & 6 & \ccell{6}{28}{21.4} & 17 & \ccell{17}{28}{60.7} & - & 0.0 & - & 0.0 & - & 0.0 &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & - & 0.0 & - & 0.0 & - & 0.0\\ 
     &  Misc                   & 14 & 19.4 & 42 & \ccell{42}{72}{58.3} & 16 & \ccell{16}{72}{22.2} & 14 & 16.7 & 54 & \ccell{54}{84}{64.3} & 16 & \ccell{16}{84}{19.0} & 25 & 57.1 & 20 & \ccell{2}{28}{7.1} & - & \ccell{10}{28}{35.7} &  25  & 55.6 &  20  & \ccell{20}{45}{44.4} &  0 & \ccell{0}{45}{0.0} & 12 & 13.0 & 78 & \ccell{78}{92}{84.8} & 2 & \ccell{2}{92}{2.2}\\ \hhline{*{32}{-}}
\multirow{7}{*}{Device}  &  Wi-Fi                  & 9 & 100.0 & - & \ccell{0}{9}{0.0} & - & \ccell{0}{9}{0.0} & 9 & 100.0 & - & \ccell{0}{9}{0.0} & - & \ccell{0}{9}{0.0} & 4 & 100.0 & - & \ccell{0}{10}{0.0} & - & \ccell{0}{10}{0.0} &   4  & 100.0 &  0 & \ccell{0}{4}{0.0} &  0 & \ccell{0}{4}{0.0} & 9 & 100.0 & - & \ccell{0}{9}{0.0} & - & \ccell{0}{9}{0.0}\\ 
     &  Bluetooth              & 18 & 60.0 & 11 & \ccell{11}{30}{36.7} & 1 & \ccell{1}{30}{3.3} & 18 & 58.1 & 12 & \ccell{12}{31}{38.7} & 1 & \ccell{1}{31}{3.2} & - & 0.0 & - & 0.0 & - & 0.0 &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & 18 & 100.0 & - & \ccell{0}{18}{0.0} & - & \ccell{0}{18}{0.0}\\ 
     &  Contact                & 1 & 10.0 & 5 & \ccell{5}{10}{50.0} & 4 & \ccell{4}{10}{40.0} & 1 & 9.1 & 6 & \ccell{6}{11}{54.5} & 4 & \ccell{4}{11}{36.4} & - & 33.3 & - & \ccell{2}{3}{66.7} & - & \ccell{0}{3}{0.0} &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & 1 & 25.0 & 2 & \ccell{2}{4}{50.0} & 1 & \ccell{1}{4}{25.0}\\ 
     &  NFC                    & 5 & 26.3 & 14 & \ccell{14}{19}{73.7} & - & \ccell{0}{19}{0.0} & 9 & 39.1 & 14 & \ccell{14}{23}{60.9} & - & \ccell{0}{23}{0.0} & - & 0.0 & - & 0.0 & - & 0.0 &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & 5 & 100.0 & - & \ccell{0}{5}{0.0} & - & \ccell{0}{5}{0.0}\\ 
     &  Screen                 & 4 & 36.4 & 6 & \ccell{6}{11}{54.5} & 1 & \ccell{1}{11}{9.1} & 4 & 36.4 & 6 & \ccell{6}{11}{54.5} & 1 & \ccell{1}{11}{9.1} & 9 & 100.0 & - & \ccell{0}{3}{0.0} & - & \ccell{0}{3}{0.0} &   9  & 100.0 &  0 & \ccell{0}{9}{0.0} &  0 & \ccell{0}{9}{0.0} & 4 & 100.0 & - & \ccell{0}{4}{0.0} & - & \ccell{0}{4}{0.0}\\ 
     &  Phone                  & 1 & 4.3 & 21 & \ccell{21}{23}{91.3} & 1 & \ccell{1}{23}{4.3} & 1 & 4.3 & 21 & \ccell{21}{23}{91.3} & 1 & \ccell{1}{23}{4.3} & 1 & 100.0 & - & \ccell{0}{1}{0.0} & - & \ccell{0}{1}{0.0} &   1  & 100.0 &  0 & \ccell{0}{1}{0.0} &  0 & \ccell{0}{1}{0.0} & 1 & 50.0 & 1 & \ccell{1}{2}{50.0} & - & \ccell{0}{2}{0.0}\\ 
     &  Misc                   & 28 & 63.6 & 15 & \ccell{15}{44}{34.1} & 1 & \ccell{1}{44}{2.3} & 28 & 59.6 & 18 & \ccell{18}{47}{38.3} & 1 & \ccell{1}{47}{2.1} & 16 & 80.8 & 7 & \ccell{5}{26}{19.2} & - & \ccell{0}{26}{0.0} &  16  & 69.6 &   7  & \ccell{7}{23}{30.4} &  0 & \ccell{0}{23}{0.0} & 28 & 82.4 & 6 & \ccell{6}{34}{17.6} & - & \ccell{0}{34}{0.0}\\ \hhline{*{32}{-}}
\multirow{2}{*}{AI}  &  CV                     & 19 & 100.0 & - & \ccell{0}{19}{0.0} & - & \ccell{0}{19}{0.0} & 19 & 100.0 & - & \ccell{0}{19}{0.0} & - & \ccell{0}{19}{0.0} & - & 90.0 & - & \ccell{2}{20}{10.0} & - & \ccell{0}{20}{0.0} &   0  & 0.0 &  0 & 0.0 &  0 & 0.0 & - & 0.0 & - & 0.0 & - & 0.0\\ 
     &  Misc                   & - & 0.0 & - & 0.0 & - & 0.0 & - & 0.0 & 1 & \ccell{1}{1}{100.0} & - & \ccell{0}{1}{0.0} & 7 & 100.0 & - & \ccell{0}{11}{0.0} & - & \ccell{0}{11}{0.0} &   7  & 100.0 &  0 & \ccell{0}{7}{0.0} &  0 & \ccell{0}{7}{0.0} & - & 0.0 & - & 0.0 & - & 0.0\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{AD}          & 19 & 95.0 & 1 & \ccell{1}{20}{5.0} & - & \ccell{0}{20}{0.0} & 19 & 95.0 & 1 & \ccell{1}{20}{5.0} & - & \ccell{0}{20}{0.0} & 13 & 64.3 & 8 & \ccell{4}{14}{28.6} & - & \ccell{1}{14}{7.1} &  13  & 61.9 &   8  & \ccell{8}{21}{38.1} &  0 & \ccell{0}{21}{0.0} & 3 & 25.0 & 9 & \ccell{9}{12}{75.0} & - & \ccell{0}{12}{0.0}\\ \hhline{*{32}{-}}
\multicolumn{2}{c}{Uncategorized}        & 30 & 38.5 & 47 & \ccell{47}{78}{60.3} & 1 & \ccell{1}{78}{1.3} & 30 & 36.6 & 51 & \ccell{51}{82}{62.2} & 1 & \ccell{1}{82}{1.2} & 17 & 53.6 & 7 & \ccell{10}{28}{35.7} & 1 & \ccell{3}{28}{10.7} &  17  & 68.0 &   8  & \ccell{7}{25}{28.0} &   1  & \ccell{1}{25}{4.0} & 34 & 68.0 & 15 & \ccell{15}{50}{30.0} & 1 & \ccell{1}{50}{2.0}\\

\midrule[0.5pt]

\multicolumn{2}{c}{\textbf{All}}  & 590 & 51.0 & 502 & \ccell{502}{1157}{43.4} & 65 & \ccell{65}{1157}{5.6} & 606 & 47.3 & 593 & \ccell{593}{1281}{46.3} & 82 & \ccell{82}{1281}{6.4} & 383 & 77.2 & 120 & \ccell{112}{601}{18.6} & 2 & \ccell{25}{601}{4.2} & 383  & 75.8 & 122  & \ccell{120}{505}{23.8} &   2  & \ccell{2}{505}{0.4} & 506 & 62.7 & 295 & \ccell{295}{807}{36.6} & 6 & \ccell{6}{807}{0.7}\\

\bottomrule[1.5pt]
\end{tabular}
 
\caption{Categories of Documented and Undocumented APIs. ``D'' means documented APIs;  ``UU'' means undocumented unchecked APIs; ``UC'' means undocumented checked APIs.}  
 
\label{tab:compare:api}
 \vspace{-0.25in}
\end{table*}


==> tables/api-cat.tex <==


\begin{table*}[h]
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1.2}
\scriptsize

 
\begin{tabular}{clcrcrcr|crcrcr|crcrcr|crcrcr|crcrcr}
\toprule[1.5pt]

    \multicolumn{2}{c}{
        \multirow{2}{*}{\textbf{Available APIs}}} &

    \multicolumn{6}{c}{
        \textbf{WeChat}
    } &
    \multicolumn{6}{c}{
        \textbf{WeCom}
    } &
    \multicolumn{6}{c}{
        \textbf{Baidu}
    } & 
    \multicolumn{6}{c}{
        \textbf{Tiktok}
    } & 
    \multicolumn{6}{c}{
        \textbf{QQ}
    } \\
    \cline{3-32}

    \multicolumn{2}{c}{} &
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UU
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            UC
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} \\ 

\midrule[0.5pt]


\multirow{4}{*}{Base}
    & Basic                 & 5 &71.4 &  2 &28.6 &  - & 0.0 &  6 &66.7 &  3 &33.3 &  - & 0.0 &  8 &72.7 &  3 &27.3 &  1 & 9.1 &  7 &63.6 &  4 &36.4 &  - & 0.0 &  3 &100.0& - & 0.0 &  - & 0.0 \\ 
    & App                   & 13 &39.4 & 20 &60.6 & 6 &18.2 & 13 &37.1 & 22 &62.9 &  6 &17.1 &  8 &42.1 & 11 &57.9 &  1 & 5.3 &  6 &50.0 &  6 &50.0 &  - & 0.0 &  9 &34.6 & 17 &65.4 &  - & 0.0 \\ 
    & Debug                 & 15 &88.2 &  2 &11.8 &  - & 0.0 & 15 &88.2 &  2 &11.8 &  - & 0.0 &  1 & 3.3 & 29 &96.7 &  1 & 3.3 &  0 & 0.0 &  - & 0.0 &  - & 0.0 & 20 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Misc                  & 10 &58.8 &  7 &41.2 &  - & 0.0 & 10 &55.6 &  8 &44.4 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 & 10 &52.6 &  9 &47.4 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multirow{5}{*}{UI}
    & Interaction           &  6 &46.2 &  7 &53.8 &  - & 0.0 &  6 &46.2 &  7 &53.8 &  - & 0.0 &  7 &41.2 & 10 &58.8 &  - & 0.0 &  9 &81.8 &  2 &18.2 &  - & 0.0 &  6 &40.0 &  9 &60.0 &  - & 0.0 \\ 
    & Navigation            &  4 &44.4 &  5 &55.6 &  - & 0.0 &  4 &40.0 &  6 &60.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 &  5 &100.0&  - & 0.0 &  - & 0.0 &  4 &33.3 &  8 &66.7 &  - & 0.0 \\ 
    & Animation             & 32 &100.0&  - & 0.0 &  - & 0.0 & 32 &100.0&  - & 0.0 &  - & 0.0 & 21 &95.5 &  1 & 4.5 &  - & 0.0 &  1 &100.0&  - & 0.0 &  - & 0.0 & 31 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & WebView               &  0 & 0.0 & 23 &100.0&  1 & 4.3 &  0 & 0.0 & 25 &100.0&  1 & 4.0 &  0 & 0.0 &  4 &100.0&  1 &25.0 &  0 & 0.0 &  3 &100.0&  - & 0.0 &  0 & 0.0 & 16 &100.0&  - & 0.0 \\ 
    & Misc                  & 20 &27.0 & 54 &73.0 &  - & 0.0 & 20 &25.6 & 58 &74.4 &  - & 0.0 & 37 &77.1 & 11 &22.9 &  - & 0.0 & 14 &73.7 &  5 &26.3 &  - & 0.0 & 18 &42.9 & 24 &57.1 &  - & 0.0 \\ \cline{1-32}

\multirow{5}{*}{Network}
    & Request               &  5 &55.6 &  4 &44.4 &  - & 0.0 &  5 &55.6 &  4 &44.4 &  - & 0.0 &  2 &66.7 &  1 &33.3 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  4 &66.7 &  2 &33.3 &  - & 0.0 \\ 
    & Download              &  7 &24.1 & 22 &75.9 & 1 & 3.4 &  7 &23.3 & 23 &76.7 &  1 & 3.3 & 11 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  4 &100.0&  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 \\ 
    & Upload                &  7 &50.0 &  7 &50.0 &  2 &14.3 &  7 &46.7 &  8 &53.3 &  2 &13.3 &  6 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  4 &100.0&  - & 0.0 &  6 &75.0 &  2 &25.0 &  - & 0.0 \\ 
    & Websocket             & 14 &93.3 &  1 & 6.7 &  - & 0.0 & 14 &93.3 &  1 & 6.7 &  - & 0.0 & 13 &100.0&  - & 0.0 &  - & 0.0 &  7 &77.8 &  2 &22.2 &  - & 0.0 & 13 &86.7 &  2 &13.3 &  - & 0.0 \\ 
    & Misc                  & 23 &88.5 &  3 &11.5 &  - & 0.0 & 23 &85.2 &  4 &14.8 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 & 10 &55.6 &  8 &44.4 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Storage}
                            & 10 &66.7 &  5 &33.3 &  - & 0.0 & 10 &66.7 &  5 &33.3 &  - & 0.0 & 10 &100.0&  - & 0.0 &  - & 0.0 & 10 &90.9 &  1 & 9.1 &  - & 0.0 & 10 &83.3 &  2 &16.7 &  - & 0.0 \\ \cline{1-32}

\multirow{8}{*}{Media}
    & Map                   &  8 &14.3 & 48 &85.7 &  - & 0.0 &  8 &14.3 & 48 &85.7 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  6 &100.0&  - & 0.0 &  - & 0.0 &  9 &36.0 & 16 &64.0 &  - & 0.0 \\ 
    & Image                 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  6 &85.7 &  1 &14.3 &  - & 0.0 &  5 &83.3 &  1 &16.7 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 \\ 
    & Video                 & 14 &35.0 & 26 &65.0 &  - & 0.0 & 14 &31.8 & 30 &68.2 &  - & 0.0 & 19 &95.0 &  1 & 5.0 &  - & 0.0 &  8 &80.0 &  2 &20.0 &  - & 0.0 & 14 &63.6 &  8 &36.4 &  - & 0.0 \\ 
    & Audio                 & 64 &84.2 & 12 &15.8 &  3 & 0.0 & 64 &79.0 & 17 &21.0 &  3 & 3.7 & 44 &100.0&  - & 0.0 &  - & 0.0 & 44 &81.5 & 10 &18.5 &  - & 0.0 & 61 &85.9 & 10 &14.1 &  - & 0.0 \\ 
    & Live                  & 26 &46.4 & 30 &53.6 &  - & 3.9 & 26 &39.4 & 40 &60.6 &  - & 0.0 &  8 &100.0&  - & 0.0 &  - & 0.0 & 19 &100.0&  - & 0.0 &  - & 0.0 & 23 &57.5 & 17 &42.5 &  - & 0.0 \\ 
    & Recorder              & 16 &84.2 &  3 &15.8 &  - & 0.0 & 16 &84.2 &  3 &15.8 &  - & 0.0 & 12 &100.0&  - & 0.0 &  - & 0.0 & 11 &91.7 &  1 & 8.3 &  - & 0.0 & 15 &88.2 &  2 &11.8 &  - & 0.0 \\ 
    & Camera                &  9 &60.0 &  6 &40.0 &  - & 0.0 &  9 &52.9 &  8 &47.1 &  - & 0.0 &  9 &50.0 &  9 &50.0 &  - & 0.0 & 20 &95.2 &  1 & 4.8 &  - & 0.0 &  4 &36.4 &  7 &63.6 &  - & 0.0 \\ 
    & Misc                  & 12 &75.0 &  4 &25.0 &  1 & 0.0 & 12 &75.0 &  4 &25.0 &  1 & 6.3 & 18 &100.0&  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  6 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Location} 
                            &  3 &42.9 &  4 &57.1 &  - & 6.3 &  3 &42.9 &  4 &57.1 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Share}
                            &  4 &33.3 &  8 &66.7 &  1 & 0.0 &  4 &16.7 & 20 &83.3 &  1 & 4.2 &  3 &100.0&  - & 0.0 &  - & 0.0 &  5 &71.4 &  2 &28.6 &  - & 0.0 &  5 &35.7 &  9 &64.3 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Canvas}
                            & 60 &74.1 & 21 &25.9 &  - & 8.3 & 60 &74.1 & 21 &25.9 &  - & 0.0 & 46 &92.0 &  4 & 8.0 &  - & 0.0 & 49 &98.0 &  1 & 2.0 &  - & 0.0 & 48 &92.3 &  4 & 7.7 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{File}
                            & 39 &97.5 &  1 & 2.5 &  - & 0.0 & 39 &92.9 &  3 & 7.1 &  - & 0.0 & 35 &100.0&  - & 0.0 &  - & 0.0 & 34 &97.1 &  1 & 2.9 &  - & 0.0 & 37 &97.4 &  1 & 2.6 &  - & 0.0 \\ \cline{1-32}

\multirow{7}{*}{Open API}
    & Login                 &  2 &100.0&  - & 0.0 &  - & 0.0 &  5 &83.3 &  1 &16.7 &  - & 0.0 &  3 &75.0 &  1 &25.0 &  3 &75.0 &  2 &100.0&  - & 0.0 &  - & 0.0 &  2 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Navigate              &  2 &33.3 &  4 &66.7 &  2 & 0.0 &  2 &22.2 &  7 &77.8 &  2 &22.2 &  3 &100.0&  - & 0.0 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  2 &50.0 &  2 &50.0 &  1 &25.0 \\ 
    & User Info             &  2 &16.7 & 10 &83.3 &  3 &33.3 &  5 &23.8 & 16 &76.2 &  3 &14.3 &  1 &10.0 &  9 &90.0 &  3 &30.0 &  2 &13.3 & 13 &86.7 &  - & 0.0 &  2 &28.6 &  5 &71.4 &  1 &14.3 \\ 
    & Payment               &  1 & 3.4 & 28 &96.6 & 15 &25.0 &  1 & 3.2 & 30 &96.8 & 15 &48.4 &  1 &50.0 &  1 &50.0 &  1 &50.0 &  1 &33.3 &  2 &66.7 &  1 &33.3 &  2 &22.2 &  7 &77.8 &  - & 0.0 \\ 
    & Bio-Auth              &  3 &27.3 &  8 &72.7 &  5 &51.7 &  3 &21.4 & 11 &78.6 &  5 &35.7 &  0 & 0.0 &  0 & 0.0 &  - & 0.0 &  0 & 0.0 &  1 &100.0&  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Enterprise            &  0 & 0.0 &  1 &100.0&  - &45.5 &  5 &17.9 & 23 &82.1 & 17 &60.7 &  0 & 0.0 &  0 & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ 
    & Misc                  & 14 &19.4 & 58 &80.6 & 16 & 0.0 & 14 &16.7 & 70 &83.3 & 16 &19.0 & 16 &57.1 & 12 &42.9 & 10 &35.7 & 25 &55.6 & 20 &44.4 &  - & 0.0 & 12 &13.0 & 80 &87.0 &  2 & 2.2 \\ \cline{1-32}

\multirow{7}{*}{Device}
    & Wi-Fi                 &  9 &100.0&  - & 0.0 &  - &22.2 &  9 &100.0&  - & 0.0 &  - & 0.0 & 10 &100.0&  - & 0.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Bluetooth             & 18 &60.0 & 12 &40.0 &  1 & 0.0 & 18 &58.1 & 13 &41.9 &  1 & 3.2 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 & 18 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Contact               &  1 &10.0 &  9 &90.0 &  4 & 3.3 &  1 & 9.1 & 10 &90.9 &  4 &36.4 &  1 &33.3 &  2 &66.7 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  1 &25.0 &  3 &75.0 &  1 &25.0 \\ 
    & NFC                   &  5 &26.3 & 14 &73.7 &  - &40.0 &  9 &39.1 & 14 &60.9 &  - & 0.0 &  - &33.3 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  5 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Screen                &  4 &36.4 &  7 &63.6 &  1 & 0.0 &  4 &36.4 &  7 &63.6 &  1 & 9.1 &  3 &100.0&  - & 0.0 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 \\ 
    & Phone                 &  1 & 4.3 & 22 &95.7 &  1 & 9.1 &  1 & 4.3 & 22 &95.7 &  1 & 4.3 &  1 &100.0&  - & 0.0 &  - & 0.0 &  1 &100.0&  - & 0.0 &  - & 0.0 &  1 &50.0 &  1 &50.0 &  - & 0.0 \\ 
    & Misc                  & 28 &63.  & 16 &36.4 &  1 & 4.3 & 28 &59.6 & 19 &40.4 &  1 & 2.1 & 21 &80.8 &  5 &19.2 &  - & 0.0 & 16 &69.6 &  7 &30.4 &  - & 0.0 & 28 &82.4 &  6 &17.6 &  - & 0.0 \\ \cline{1-32}

\multirow{2}{*}{AI}
    & CV                    & 19 &100.0&  - & 0.0 &  - & 2.3 & 19 &100.0&  - & 0.0 &  - & 0.0 & 18 &90.0 &  2 &10.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ 
    & Misc                  &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  1 &100.0&  - & 0.0 & 11 &100.0&  - & 0.0 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{AD}
                            & 19 &95.0 &  1 & 5.0 &  - & 0.0 & 19 &95.0 &  1 & 5.0 &  - & 0.0 &  9 &64.3 &  5 &35.7 &  1 & 7.1 & 13 &61.9 &  8 &38.1 &  - & 0.0 &  3 &25.0 &  9 &75.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Uncategorized}
                            & 30 &38.5 & 48 &61.5 &  1 & 1.3 & 30 &36.6 & 52 &63.4 &  1 & 1.2 & 15 &53.6 & 13 &46.4 &  3 &10.7 & 17 &68.0 &  8 &32.0 &  1 & 4.0 & 34 &68.0 & 16 &32.0 &  1 & 2.0 \\

\midrule[0.5pt]

\multicolumn{2}{c}{\textbf{All}}
                            &590 &51.0 &567 &49.0 & 65 & 5.6 &606 &47.3 &675 &52.7 & 82 & 6.4 &464 &77.5 &135 &22.5 & 25 & 4.2 &383 &75.8 &122 &24.2 &  2 & 0.4 &506 &62.7 &301 &37.3 &  6 & 0.7 \\
\bottomrule[1.5pt]
\end{tabular}
\vspace{2mm}
\caption{Categories of Official and Hidden APIs. ``D'' means documented APIs;  ``UU'' means undocumented unchecked APIs; ``UC'' means undocumented checked APIs \ZY{HEATMAP}} 
% due to page limit
\label{tab:compare:api}
\end{table*}

% undefined means no subcategory
% | category | subcategory | # of WeChat Official API | # of WeCom Official API | # of Baidu Official API | # of WeChat Hidden API | # of WeCom Hidden API | # of Baidu Hidden API | Required Permission |
% | base     | undefined            |  3 |  4 |  5 |   |   |    |    | 
% | base     | system               |  2 |  2 |  3 |   |   |    |    |
% | base     | update               |  6 |  6 |  5 |   |   |    |    |
% | base     | app                  | 13 | 13 |  8 |   |   |    |    |
% | base     | debug                | 15 | 15 |  1 |   |   |    |    |
% | base     | timer                |  4 |  4 |  4 |   |   |    |    |
% | route    | undefined            |  5 |  5 |  5 |   |   |    |    |
% | ui       | interaction          |  6 |  6 |  7 |   |   |    |    |
% | ui       | navigation-bar       |  4 |  4 |  4 |   |   |    |    |
% | ui       | background           |  2 |  2 |  2 |   |   |    |    |
% | ui       | tab-bar              |  8 |  8 |  8 |   |   |    |    |
% | ui       | pull-down-refresh    |  2 |  2 |  3 |   |   |    |    |
% | ui       | scroll               |  1 |  1 |  1 |   |   |    |    |
% | ui       | animation            | 32 | 32 | 21 |   |   |    |    |
% | ui       | sticky               |  1 |  1 |  0 |   |   |    |    |
% | ui       | custom-component     |  1 |  1 |  1 |   |   |    |    |
% | ui       | menu                 |  1 |  1 |  1 |   |   |    |    |
% | ui       | window               |  2 |  2 |  4 |   |   |    |    |
% | ui       | keyboard             |  2 |  2 |  3 |   |   |    |    |
% | ui       | node-info            |  0 |  0 | 14 |   |   |    |    |
% | network  | request              |  5 |  5 |  2 |   |   |    |    |
% | network  | download             |  7 |  7 | 11 |   |   |    |    |
% | network  | upload               |  7 |  7 |  6 |   |   |    |    |
% | network  | websocket            | 14 | 14 | 13 |   |   |    |    |
% | network  | mdns                 | 10 | 10 |  0 |   |   |    |    |
% | network  | udp                  | 13 | 13 |  0 |   |   |    |    |
% | storage  | undefined            | 10 | 10 | 10 |   |   |    |    |
% | media    | map                  |  8 |  8 |  7 |   |   |    |    |
% | media    | image                |  6 |  6 |  6 |   |   |    |    |
% | media    | video                | 14 | 14 | 19 |   |   |    |    |
% | media    | audio                | 38 | 38 | 27 |   |   |    |    |
% | media    | background-audio     | 26 | 26 | 17 |   |   |    |    |
% | media    | live                 | 26 | 26 |  8 |   |   |    |    |
% | media    | recorder             | 16 | 16 | 12 |   |   |    |    |
% | media    | camera               |  9 |  9 |  9 |   |   |    |    |
% | media    | editor               | 11 | 11 |  4 |   |   |    |    |
% | media    | font                 |  1 |  1 |  0 |   |   |    |    |
% | media    | RTC                  |  0 |  0 | 13 |   |   |    |    |
% | media    | TTS                  |  0 |  0 |  1 |   |   |    |    |
% | location | undefined            |  3 |  3 |  7 |   |   |    |    |
% | share    | undefined            |  4 |  4 |  3 |   |   |    |    |
% | canvas   | undefined            | 60 | 60 | 46 |   |   |    |    |
% | file     | undefined            | 39 | 39 | 35 |   |   |    |    |
% | open-api | login                |  2 |  5 |  3 |   |   |    |    | 
% | open-api | miniprogram-navigate |  2 |  2 |  3 |   |   |    |    |
% | open-api | account-info         |  1 |  1 |  0 |   |   |    |    |
% | open-api | user-info            |  2 |  5 |  1 |   |   |    |    |
% | open-api | report               |  1 |  1 |  0 |   |   |    |    |
% | open-api | data-analysis        |  1 |  1 |  1 |   |   |    |    |
% | open-api | payment              |  1 |  1 |  1 |   |   |    |    |
% | open-api | authorize            |  1 |  1 |  1 |   |   |    |    |
% | open-api | setting              |  3 |  3 |  2 |   |   |    |    |
% | open-api | address              |  1 |  1 |  1 |   |   |    |    |
% | open-api | card                 |  2 |  2 |  0 |   |   |    |    |
% | open-api | invoice              |  2 |  2 |  1 |   |   |    |    |
% | open-api | subscribe            |  1 |  1 |  1 |   |   |    |    |
% | open-api | soter                |  3 |  3 |N/A |   |   |N/A |    |
% | open-api | werun                |  1 |  1 |N/A |   |   |N/A |    |
% | open-api | enterprise           |  0 |  5 |N/A |   |   |N/A |    |
% | open-api | package              |  0 |  0 |  3 |   |   |    |    |
% | open-api | system-risk          |  0 |  0 |  1 |   |   |    |    |
% | open-api | Bookshelf            |N/A |N/A |  5 |   |   |    |    |
% | device   | ibeacon              |  6 |  6 |  0 |   |   |    |    |
% | device   | wifi                 |  9 |  9 | 10 |   |   |    |    |
% | device   | bluetooth-ble        |  9 |  9 |  0 |   |   |    |    |
% | device   | contact              |  1 |  1 |  1 |   |   |    |    |
% | device   | bluetooth            |  9 |  9 |  0 |   |   |    |    |
% | device   | battery              |  2 |  2 |  2 |   |   |    |    |
% | device   | clipboard            |  2 |  2 |  2 |   |   |    |    |
% | device   | nfc                  |  5 |  9 |  0 |   |   |    |    |
% | device   | network              |  2 |  2 |  2 |   |   |    |    |
% | device   | screen               |  4 |  4 |  3 |   |   |    |    |
% | device   | phone                |  1 |  1 |  1 |   |   |    |    |
% | device   | accelerometer        |  3 |  3 |  3 |   |   |    |    |
% | device   | compass              |  3 |  3 |  3 |   |   |    |    |
% | device   | motion               |  3 |  3 |  3 |   |   |    |    |
% | device   | gyroscope            |  3 |  3 |  0 |   |   |    |    |
% | device   | performance          |  1 |  1 |  1 |   |   |    |    |
% | device   | scan                 |  1 |  1 |  1 |   |   |    |    |
% | device   | vibrate              |  2 |  2 |  2 |   |   |    |    |
% | device   | calendar             |  0 |  0 |  2 |   |   |    |    |
% | cloud    | storage              |N/A |N/A |  3 |   |   |    |    |
% | cloud    | function             |N/A |N/A |  1 |   |   |    |    |
% | cloud    | init                 |N/A |N/A |  1 |   |   |    |    |
% | cloud    | database             |N/A |N/A |  3 |   |   |    |    |
% | ai       | vision               | 16 | 16 |N/A |   |   |    |    |
% | ai       | OCR                  |  0 |  0 |  4 |   |   |    |    |
% | ai       | voice-recognition    |  0 |  0 |  8 |   |   |    |    |
% | ai       | text-to-audio        |  0 |  0 |  1 |   |   |    |    |
% | ai       | text-review          |  0 |  0 |  1 |   |   |    |    |
% | ai       | nlp-lexer            |  0 |  0 |  1 |   |   |    |    |
% | ai       | image-classify       |  0 |  0 |  7 |   |   |    |    |
% | ai       | image-audit          |  0 |  0 |  1 |   |   |    |    |
% | ai       | face-detection       |  3 |  3 |  6 |   |   |    |    |
% | worker   | undefined            |  5 |  5 |  0 |   |   |    |    |
% | ext      | undefined            |  2 |  2 |  2 |   |   |    |    |
% | wxml     | undefined            | 18 | 18 |  0 |   |   |N/A |    |
% | ad       | undefined            | 19 | 19 |  9 |   |   |  5 |    |
% | misc     | undefined            |N/A |N/A |N/A |   |   |    |    |    

% total baidu hidden API: 135
\ignore{
[x] /swanAPI/dataChannel',      other
[x] /swanAPI/cloudRequest',     cloud other
[x] /swanAPI/aiRequest',        ai other
[x] /swanAPI/im/pullMsg',       other
[x] /swanAPI/privateGetUserInfo',  open-api user-info
[x] /swanAPI/publishThread',       open-api other
[x] /swanAPI/camera/update',       media camera
[x] /swanAPI/camera/remove',       media camera
[x] /swanAPI/camera/insert',       media camera
[x] /swanAPI/setTplBdussSync',     open-api user-info
[x] /swanAPI/setSelectedAddressSync', open-api user-info
[x] /swanAPI/installApp4Ad',       ad
[x] /swanAPI/getChannelID',        other
[x] /swanAPI/getPushSettingStateSync', device other
[x] /swanAPI/guidePushSetting',        device other
[x] /swanAPI/coverimage',              ui interaction
[x] /swanAPI/coverview',               ui interaction
[x] /swanAPI/debuggerlaunch',          debug
[x] /swanAPI/remoteDebug',             debug
[x] /swanAPI/sConsole',                debug
[x] /swanAPI/joinActivity',            open-api other
[x] /swanAPI/activityRequest',         open-api other
[x] /swanAPI/addActivityFavor',        open-api other
[x] /swanAPI/wirelessdebuglaunch',     debug
[x] /swanAPI/launch',                  base app
[x] /swanAPI/perfCat',                 debug
[x] /swanAPI/ARCamera/detectContent',  media camera
[x] /swanAPI/ARCamera/insert',         media camera
[x] /swanAPI/ARCamera/remove',         media camera
[x] /swanAPI/ARCamera/changeARStatus', media camera
[x] /swanAPI/ARCamera/arMessage',      media camera
[x] /swanAPI/ARCamera/update',         media camera
[x] /swanAPI/adRequest',               ad
[x] /swanAPI/openAdWebPage',           ad
[x] /swanAPI/openAdLandingPage',       ad
[x] /swanAPI/debug/setWebDegradeDebugHost', debug
[x] /swanAPI/localdebuglaunch',             debug
[x] /swanAPI/openFullScreenView',           ui window
[x] /swanAPI/closeFullScreenView',          ui window
[x] /swanAPI/imageRecognition',             ai vision
[x] /swanAPI/debug/setReplaceSwanCoreConfig',  debug
[x] /swanAPI/debugSwanCore',                   debug
[x] /swanAPI/debug/setReplaceDynamicLibConfig', debug
[x] /swanAPI/debug/setExtensionConfig',         debug
[x] /swanAPI/debug/setCtsConfig',               debug
[x] /swanAPI/debug/setReplaceDependencyConfig', debug
[x] /swanAPI/debug/replaceSwanCore',            debug
[x] /swanAPI/debug/setDebugConfig',             debug
[x] /swanAPI/debug/replaceDependency',          debug
[x] /swanAPI/debug/replaceDynamicLib',          debug
[x] /swanAPI/debug/downloadExtension',          debug
[x] /swanAPI/debug/getDebugConfig',             debug
[x] /swanAPI/getLaunchAppInfo',                 base app
[x] /swanAPI/launchCloudGame',                  base app
[x] /swanAPI/menu',                             ui menu
[x] /swanAPI/getPhoneNumberByLogin',            open-api user-info
[x] /swanAPI/thirdPartyLogin',                  ext
[x] /swanAPI/getRealNameInfo',                  open-api user-info
[x] /swanAPI/getStoken',                        open-api user-info
[x] /swanAPI/getBDUSS',                         open-api user-info
[x] /swanAPI/faceResultVerify',                 ai vision
[x] /swanAPI/canvas/drawCanvas',                canvas
[x] /swanAPI/canvas/remove',                    canvas
[x] /swanAPI/canvas/insert',                    canvas
[x] /swanAPI/canvas/update',                    canvas
[x] /swanAPI/button',                           ui interaction
[x] /swanAPI/recommendProducts',                open-api other
[x] /swanAPI/recommendSimilarProducts',         open-api other
[x] /swanAPI/exit',                             base app
[x] /swanAPI/postPageInfo',                     ui interaction
[x] /swanAPI/cancelRequest',                    network request
[x] /swanAPI/prefetchAppData',                  base app
[x] /swanAPI/installApp',                       base app
[x] /swanAPI/addComponentToFullScreenSync',     ui window
[x] /swanAPI/setFullscreenOrientationSync',     ui window
[x] /swanAPI/removeComponentFromFullScreenSync', ui window
[x] /swanAPI/updateInput',                       ui keyboard
[x] /swanAPI/openInput',                         ui keyboard
[x] /swanAPI/closeInput',                        ui keyboard
[x] /swanAPI/debugGameCore',                    debug
[x] /swanAPI/openApp4Ad',                       ad
[x] /swanAPI/openApp',                          base app
[x] /swanAPI/getSlaveIdSync',                   other
[x] /swanAPI/openStatisticFlowJar',             report
[x] /swanAPI/openStatisticEvent',               report
[x] /swanAPI/postMessage',                      other
[x] /swanAPI/preloadSubPackage',                base app
[x] /swanAPI/pageTransition',                   ui interaction
[x] /swanAPI/performancePanel',                 debug
[x] /swanAPI/preloadSwanCore',                  debug
[x] /swanAPI/preventPullDownRefresh',           ui pulldown refresh
[x] /swanAPI/abTestConfig',                     debug
[x] /swanAPI/confirmSwanClose',                 debug
[x] /swanAPI/getLocalImgData',                  media image
[x] /swanAPI/getAppInfoSync',                   base app
[x] /swanAPI/getFormId',                        ui node-info
[x] /swanAPI/animView',                         ui animation
[x] /swanAPI/insertWebView',                    ui webview
[x] /swanAPI/updateWebView',                    ui webview
[x] /swanAPI/removeWebView',                    ui webview
[x] /swanAPI/webviewPostMessage',               ui webview
[x] /swanAPI/quickPay',                         open-api payment
[x] /swanAPI/updateTextarea',                   ui interaction
[x] /swanAPI/openTextarea',                     ui interaction
[x] /swanAPI/getScreenshot',                    base system
[x] /swanAPI/closeTextarea',                    ui interaction
[x] /swanAPI/community/openReplyEditor',        ui interaction
[x] /swanAPI/community/closeReplyEditor',       ui interaction
[x] /swanAPI/addFavor',                         open-api other
[x] /swanAPI/deleteFavor',                      open-api other
[x] /swanAPI/isFavor',                          open-api other
[x] /swanAPI/topFavor',                         open-api other
[x] /swanAPI/hideOpenAppGuide',                 base app
[x] /swanAPI/showOpenAppGuide',                 base app
[x] /swanAPI/getCommonSysInfo',                 base system
[x] /swanAPI/getUserInfo',                      open-api user-info
[x] /swanAPI/login',                            open-api login
[x] /swanAPI/multiAuthorize',                   open-api authorize
[x] /swanAPI/getPhoneNumber',                   open-api user-info
[x] /swanAPI/debugGameExtensionCore',           debug
[x] /swanAPI/debug/replaceGameCore',            debug
[x] /swanAPI/debug/setReplaceGameCoreConfig',   debug
[x] /swanAPI/debug/dashboardConnect',           debug
[x] /swanAPI/getRegionData',                    open-api other
[x] /swanAPI/getAutoRotationSync',              device other
[x] /swanAPI/debugGameSconsole',                debug
[x] /swanAPI/startMediaVolumeListen',           device other
[x] /swanAPI/stopMediaVolumeListen',           device other
[x] /swanAPI/vrvideo',                         media video
[x] /swanAPI/setPhoneContact',                 device contacts
[x] /swanAPI/getPhoneContacts',                device contacts
[x] /swanAPI/checkAppInstalled',               base system
[x] /swanAPI/ubcFlowJar',                      other
[x] /swanAPI/getHistory',                      other
[x] /swanAPI/deleteHistory',                   other
}
% baidu hidden category result:
\ignore{
  other: 8,
  'cloud other': 1,
  'ai other': 1,
  'open-api user-info': 9,
  'open-api other': 11,
  'media camera': 9,
  ad: 5,
  'device other': 5,
  'ui interaction': 10,
  debug: 29,
  'base app': 11,
  'ui window': 9,
  'ai vision': 2,
  'ui menu': 1,
  ext: 1,
  canvas: 4,
  'network request': 1,
  'ui keyboard': 3,
  report: 2,
  'ui pulldown refresh': 1,
  'media image': 1,
  'ui node-info': 1,
  'ui animation': 1,
  'open-api payment': 1,
  'base system': 3,
  'open-api login': 1,
  'open-api authorize': 1,
  'media video': 1,
  'device contacts': 2
}

% following is WeChat data
\ignore{
[x]  'addNativeDownloadTask',                     network download
[x]  'getABTestConfig',                           base app
[x]  'launchApplication',                         base app
[x]  'makeVoIPCall',                              device phone
[x]  'private_onWebPageUrlExposed',               ui other
[x]  'openADCanvas',                              canvas
[x]  'resumeDownloadTask',                        network download
[x]  'writeCommData',                             other
[x]  'addPhoneCalendar',                          open-api phone
[x]  'WEB_INVOKE_APPSERVICE',                     other
[x]  'onWebviewFinishLoad',                       ui webview
[x]  'onWebviewStartLoad',                        ui webview
[x]  'onWebviewError',                            ui webview
[x]  'insertHTMLWebView',                        ui webview
[x]  'updateHTMLWebView',  ui webview
[x]  'updateXWebCanvas', ui webview
[x]  'addDownloadTask',    network download
[x]  'addDownloadTaskForNative', network download
[x]  'addDownloadTaskStraight', network download
[x]  'cancelDownloadTask', network download
[x]  'cancelDownloadTaskForNative', network download
[x]  'getInstallState', base app
[x]  'getInstallStateForNative', base app
[x]  'installDownloadTask',  network download
[x]  'installDownloadTaskForNative', network download
[x]  'jumpDownloaderWidgetForNative', network download
[x]  'launchApplicationForNative', base app
[x]  'pauseDownloadTask', network download
[x]  'pauseDownloadTaskForNative', network download
[x]  'queryDownloadTask', network download
[x]  'queryDownloadTaskForNative', network download
[x]  'resumeDownloadTaskForNative', network download
[x]  'onDownloadAppStateChangeForNative', network download
[x]  'getDownloadWidgetTaskInfoForNative', network download
[x]  'bindGroup', open-api account-info
[x]  'joinGroup', open-api account-info 
[x]  'getMusicPlayerState', media audio
[x]  'openRealnameAuth', open-api authorize
[x]  'requestAuthUserAutoFillData',  open-api authorize
[x]  'canvasToTempFilePathSync', canvas
[x]  'chooseShareGroup', open-api share
[x]  'setBackgroundFetchToken', other
[x]  'triggerBackgroundFetch', other
[x]  'getBackgroundFetchToken', other
[x]  'getAppConfig',  base app
[x]  'getOAID', open-api account-info 
[x]  'checkIsSupportFacialRecognition', open-api soter
[x]  'faceVerifyForPay', open-api payment
[x]  'handleMPChannelAction', other
[x]  'openWebViewUseFastLoad', ui webview
[x]  'onUpdateChannelFeeds', other
[x]  'getRandomValues', other
[x]  'jumpRedPacketEnvelopeList', open-api payment
[x]  'jumpRedPacketEnvelopePreview', open-api payment
[x]  'requestQueryCashier', open-api payment
[x]  'requestOfflineUserBindQuery', other
[x]  'opNativeRedDot', other
[x]  'openAddress', open-api address
[x]  'openWCCardHomePage', open-api other
[x]  'openWCCertHomePage', open-api other
[x]  'openDeliveryList', open-api other
[x]  'openLink', base other
[x]  'openOfflinePayView', open-api payment
[x]  'openUrl', base other
[x]  'openWCExDeviceList', open-api other
[x]  'openWCPayLQTDepositPlan',  open-api payment
[x]  'openWCPayLQTDepositPlanAdd', open-api payment
[x]  'openWCPayLQTDetail', open-api payment
[x]  'openWCPayLQTSave', open-api payment
[x]  'phoneBindCardVerifySms', open-api authorize
[x]  'predownloadMiniProgramPackage', base app
[x]  'private_openUrl', base other
[x]  'chooseWeChatContact', device contacts
[x]  'searchContacts', device contacts
[x]  'reportSubmitForm', other
[x]  'restart', base basic
[x]  'saveWaid', other
[x]  'systemLog', base debug
[x]  'uploadToCommonCDN', network upload
[x]  'removeSplashScreenshot', device screen
[x]  'saveSplashScreenshot', device screen
[x]  'private_fileSystemConvert', storage
[x]  'declareOriginalFinished', other
[x]  'deleteFinderDataItem', other
[x]  'endorsementFinished', other
[x]  'postFinderDataItem', other
[x]  'resendProfileFeed', other
[x]  'kvReport', open-api data-analysis
[x]  'openFinderProfile', other
[x]  'onH5Data', other
[x]  'sendDataToH5', other
[x]  'openRedPacket', open-api payment
[x]  'sendRedPacket', open-api payment
[x]  'getLabInfo', open-api other
[x]  'setLabInfo', open-api other
[x]  'onReceiveMsgChannel', other
[x]  'previewMedia', media other
[x]  'isSupportNFC', device nfc
[x]  'onNFCDiscovered', device nfc
[x]  'isNFCTechConnected', device nfc
[x]  'NFCGetMaxTransceiveLength', device nfc
[x]  'NFCSetTimeout', device nfc
[x]  'NFCTransceive', device nfc
[x]  'startNFCDiscovery', device nfc
[x]  'stopNFCDiscovery', device nfc
[x]  'writeNdefMessage', device nfc
[x]  'secureTunnel', other
[x]  'loadPaySpeechDialectConfig', open-api payment
[x]  'setCurrentPaySpeech', open-api payment
[x]  'onStartReportPageData',  open-api data-analysis
[x]  'exitVoIPChat', device phone
[x]  'setStatusBarStyle', ui other
[x]  'setMenuStyle', ui menu
[x]  'bindPaymentCard', open-api payment
[x]  'getWCPayOverseaPrepayRequest', open-api payment
[x]  'handleWCPayOverseaWalletBuffer', open-api payment
[x]  'openSelectPayment', open-api payment
[x]  'openWCPayOverseaPaymentReceive', open-api payment
[x]  'requestBizSplitBillPayment', open-api payment
[x]  'requestEntrustAuthorization', open-api authorize
[x]  'requestH5Transaction', open-api payment
[x]  'requestPaymentToBank', open-api payment
[x]  'requestVerifyUserIdentity', open-api authorize
[x]  'requestVirtualPayment', open-api payment
[x]  'sendBizRedPacket', open-api payment
[x]  'verifyPaymentPassword', open-api payment
[x]  'openQRCode', device scan
[x]  'showUpdatableMessageSubscribeButton', open-api subscribe
[x]  'showVirtualBottomNavigationBar', ui other
[x]  'openWeAppHistoryList', open-api other
[x]  'openWeAppStarList', open-api other
[x]  'reportAction', open-api data-analysis
[x]  'reportIDKey', open-api data-analysis
[x]  'checkIsOpenAccessibility', device other
[x]  'getVolume', device other
[x]  'setVolume', device other
[x]  'launchApplicationDirectly', base app
[x]  'onDownloadAppStateChange', network download
[x]  'startCustomFacialRecognitionVerify',  open-api soter
[x]  'startCustomFacialRecognitionVerifyAndUploadVideo', open-api soter
[x]  'startFacialRecognitionVerify', open-api soter
[x]  'startFacialRecognitionVerifyAndUploadVideo', open-api soter
[x]  'openAddressWithLightMode', open-api address
[x]  'openMapApp', base app
[x]  'NFCClose', device nfc
[x]  'NFCConnect', device nfc
[x]  'NFCGetAtqa', device nfc
[x]  'NFCGetHistoricalBytes', device nfc
[x]  'NFCGetSak', device nfc
[x]  'requestJointPayment', open-api payment
[x]  'requestMallPayment', open-api payment
[x]  'uploadWeRunData', open-api werun
[x]  'onXWebCastingInterrupt',  ui webview
[x]  'onXWebCastingUserSelect', ui webview
[x]  'onXWebVideoEnded', ui webview
[x]  'onXWebVideoPause', ui webview
[x]  'onXWebVideoPlay', ui webview
[x]  'onXWebVideoProgress', ui webview
[x]  'onXWebVideoTimeUpdate', ui webview
[x]  'onXWebVideoWaiting', ui webview
[x]  'onXWebDLNACastingStateChange', ui webview
[x]  'removeXWebWebGLCanvas', canvas
[x]  'updateXWebWebGLCanvas', canvas
[x]  'editTextWithPopForm', other
[x]  'onBLEPeripheralConnectionStateChanged', device bluetooth-ble
[x]  'onCharacteristicReadRequest', other
[x]  'onCharacteristicWriteRequest', other
[x]  'openChannelsActivity', open-api other
[x]  'openChannelsLive', open-api other
[x]  'openChannelsUserProfile', open-api other
[x]  'fetchSendingAndFailProfileFeed', open-api other
[x]  'getFinderAccount', open-api other
[x]  'onFeedPostCallback', open-api other
[x]  'fetchFinderProfileFeed', open-api other
[x]  'modifyFinderAccountAvatar', open-api other
[x]  'modifyFinderAccountNickname', open-api other
[x]  'openFinderPostPicker', open-api other
[x]  'shareFinderEndorsementToFriend', open-api other
[x]  'setPageOrientation', ui other
[x]  'private_setNavigationBarRightButton', ui navigation-bar
[x]  'getRecentUsageList', other
[x]  'onGetRecentUsageListResult', other
[x]  'onRealtimeDataResponse', other
[x]  'onXWebLivePlayerOrientationChanged', ui webview
[x]  'onXWebVideoOrientationChanged', ui webview
[x]  'addWeRunData', open-api werun
[x]  'insertXWebWebGLCanvas', canvas
[x]  'getAppContact', open-api account-info
[x]  'getPublicLibVersion', base app
[x]  'loadWAFile', base app
[x]  'loadWAFileSync', base app
[x]  'onLocalServiceEvent', other
[x]  'operateLocalServicesScan', other
[x]  'getRegionData', open-api other
[x]  'getBackgroundFetchData', open-api other
[x]  'operateRealtimeData', open-api other
[x]  'reportKeyValue', open-api data-analysis
[x]  'xwebCanvasToTempFilePath', canvas
[x]  'enableLocationUpdate', location
[x]  'openVideoEditor', media video
[x]  'operateMediaContainer', media other
[x]  'operateMediaTrack', media other
[x]  'onLongPress', device other
[x]  'onTouchCancel', device screen
[x]  'onTouchStart', device screen
[x]  'onTouchMove', device screen
[x]  'onTouchEnd', device screen
[x]  'updateXWebVoIPView', device phone
[x]  'insertXWebVoIPView', device phone
[x]  'removeXWebVoIPView', device phone
[x]  'insertXWebCamera', device phone
[x]  'removeXWebCamera', device phone
[x]  'updateXWebCamera', device phone
[x]  'onSkiaCanvasLongPress', canvas
[x]  'onSkiaCanvasTouchEnd', canvas
[x]  'insertXWebCanvas', canvas
[x]  'onXWebCanvasSurfaceChange', canvas
[x]  'removeXWebCanvas', canvas
[x]  'insertXWebLivePlayer', media live
[x]  'operateXWebLivePlayer', media live
[x]  'removeXWebLivePlayer', media live
[x]  'updateXWebLivePlayer', media live
[x]  'onXWebLivePlayerAudioVolume', media live
[x]  'onXWebLivePlayerBackgroundPlaybackChange', media live
[x]  'onXWebLivePlayerEvent', media live
[x]  'onXWebLivePlayerNetStatus', media live
[x]  'insertXWebLivePusher', media live 
[x]  'operateXWebLivePusher', media live
[x]  'removeXWebLivePusher', media live
[x]  'updateXWebLivePusher', media live
[x]  'onXWebLivePusherAudioVolume', media live
[x]  'onXWebLivePusherBGMComplete',  media live
[x]  'onXWebLivePusherBGMProgress', media live
[x]  'onXWebLivePusherBGMStart', media live
[x]  'onXWebLivePusherError', media live
[x]  'onXWebLivePusherEvent', media live
[x]  'onXWebLivePusherNetStatus', media live
[x]  'insertXWebMap', media map
[x]  'removeXWebMap', media map
[x]  'updateXWebMap', media map
[x]  'insertXWebVideo', media video
[x]  'operateXWebVideo', media video
[x]  'removeXWebVideo', media video
[x]  'updateXWebVideo', media video
[x]  'onXWebVideoBackgroundPlaybackChange', media video
[x]  'onXWebVideoError', media video
[x]  'onXWebVideoLoadedMetaData', media video 
[x]  'onXWebVideoPreloadedMetaData', media video
[x]  'onXWebVideoSeekComplete', media video
[x]  'onContactUpdate', device contacts
[x]  'onAudioStateChange', media audio
[x]  'onTextViewLinkClick', ui interaction
[x]  'onUpdateWXConfig', base app
[x]  'onCameraInitDone', media camera
[x]  'onCameraNeedAuthCancel', media camera
[x]  'onCameraScanCode', media camera
[x]  'onCameraStop', media camera
[x]  'onCameraVideoTaken', media camera
[x]  'onImagePreviewerLoadFail', media image
[x]  'onImageViewLoad', media image
[x]  'onImageViewClick', media image
[x]  'onTextViewClick', ui interaction 
[x]  'onTextViewDrag', ui interaction
[x]  'onScrollViewScroll', ui interaction
[x]  'onBeaconServiceChanged', device iBeacon
[x]  'onBeaconUpdated', device iBeacon
[x]  'onLocationChangeError', location
[x]  'enableLocationUpdateBackground', location
[x]  'onMapControlClick', media map
[x]  'onMapMarkerClusterClick', media map
[x]  'onMapMarkerClusterCreate', media map
[x]  'onMapAnchorPointClick', media map
[x]  'onMapCalloutClick', media map
[x]  'onMapClick', media map
[x]  'onMapIndoorChange', media map
[x]  'onMapLabelClick', media map
[x]  'onMapMarkerClick', media map
[x]  'onMapPoiClick', media map
[x]  'onMapRegionChange', media map
[x]  'onLivePlayerAudioVolume', media live
[x]  'onLivePlayerFullScreenChange', media live
[x]  'onLivePlayerNetStatus', media live
[x]  'onLivePlayerEvent', media live
[x]  'onLivePusherAudioVolume', media live
[x]  'onLivePusherBGMComplete', media live
[x]  'onLivePusherBGMProgress', media live
[x]  'onLivePusherBGMStart', media live
[x]  'onLivePusherError', media live
[x]  'onLivePusherNetStatus', media live
[x]  'onLivePusherEvent', media live
[x]  'onDownloadTaskStateChange', network download
[x]  'onRequestTaskStateChange', network request
[x]  'onUploadTaskStateChange', network upload
[x]  'onSocketTaskStateChange', network websocket
[x]  'onMultiPickerViewChange', ui other
[x]  'onVideoCanPlay', media video
[x]  'onVideoClickDanmuBtn', media video
[x]  'onVideoEnded', media video
[x]  'onVideoError', media video
[x]  'onVideoFullScreenChange', media video
[x]  'onVideoLoadedMetaData',  media video
[x]  'onVideoPause', media video
[x]  'onVideoPlay', media video
[x]  'onVideoProgress', media video
[x]  'onVideoResourceError', media video
[x]  'onVideoResourceLoad', media video
[x]  'onVideoTimeUpdate', media video
[x]  'onVideoWaiting', media video 
[x]  'onDeviceOrientationChange', device other
[x]  'addToFavorites', open-api other
[x]  'navigateBackApplication', open-api miniprogram-navigate
[x]  'openWeRunSetting', open-api werun
[x]  'private_addContact', device contact
[x]  'refreshSession', other
[x]  'showImageOperateSheet', media image
[x]  'onViewDidResize', ui other
[x]  'updateApp', base update
[x]  'onUpdateStatusChange', base update
[x]  'operateXWebLivePlayerBackground', ui webview
[x]  'operateXWebVideoBackground', ui webview
[x]  'adDataReport', open-api data-analysis
[x]  'addFileToFavorites', open-api 
[x]  'addImageToFavorites', open-api other
[x]  'addVideoToFavorites', open-api other
[x]  'batchGetContact', device contact
[x]  'getBackgroundAudioState', media audio
[x]  'onMusicEnd', media audio
[x]  'onMusicPause', media audio
[x]  'onMusicPlay', media audio
[x]  'operateMusicPlayer', media audio
[x]  'createAudioInstance', media audio
[x]  'createAudioInstanceAsync', media audio
[x]  'destroyAudioInstance', media audio
[x]  'getAudioState', media audio
[x]  'operateAudio', media audio
[x]  'onRecorderStateChange', media recorder
[x]  'operateRecorder', media recorder
[x]  'setAudioState', media recorder
[x]  'createVestUser', open-api user-info
[x]  'deleteUserAutoFillData', open-api user-info
[x]  'getPhoneNumber', open-api user-info
[x]  'getUserAutoFillData', open-api user-info
[x]  'setUserAutoFillData', open-api user-info
[x]  'batchPreloadMiniProgram', base app
[x]  'captureScreen', device screen
[x]  'functionalPageStartGame', other
[x]  'getPermissionBytes', base other
[x]  'getPluginPermissionBytes', base other
[x]  'getBLEDeviceRSSI', device bluetooth-ble
[x]  'makeBluetoothPair', device bluetooth
[x]  'notifyBLECharacteristicValueChanged', device bluetooth-ble
[x]  'setBLEMTU', device bluetooth-ble
[x]  'addBLEPeripheralService', device bluetooth-ble
[x]  'closeBLEPeripheralServer', device bluetooth-ble
[x]  'createBLEPeripheralServer', device bluetooth-ble
[x]  'removeBLEPeripheralService', device bluetooth-ble
[x]  'startBLEPeripheralAdvertising', device bluetooth-ble
[x]  'stopBLEPeripheralAdvertising', device bluetooth-ble
[x]  'writeBLEPeripheralCharacteristicValue', device bluetooth-ble
[x]  'markScene', other
[x]  'operateCamera', media camera
[x]  'openChannelsCreateContact', other
[x]  'openChannelsPostPage', other
[x]  'pageNotFoundCallback', ui other
[x]  'chooseContact', device contact
[x]  'enterContact', device contact
[x]  'privateEnterContact', device contact
[x]  'measureTextString', other
[x]  'returnCopyUrl', other
[x]  'sendRedCoverAppMsg', open-api other
[x]  'traceEvent', base debug
[x]  'updatePerfData', open-api performance
[x]  'verifyPlugin', base app
[x]  'preloadMiniProgramEnv', base app
[x]  'faceDetect', open-api soter
[x]  'faceProcessInit', open-api soter
[x]  'faceProcessStop', open-api soter
[x]  'checkHandoffEnabled', other
[x]  'startHandoff', other
[x]  'hideSplashScreenshot', ui other
[x]  'navigateBackH5', open-api miniprogram-navigate
[x]  'loadJsFiles', file
[x]  'createFinderAccount', open-api other
[x]  'hideKeyboard', ui keyboard
[x]  'onTextAreaHeightChange', ui other
[x]  'removeTextArea', ui other
[x]  'restoreWebviewFocus', ui webview
[x]  'setKeyboardValue', ui keyboard
[x]  'onKeyboardValueChange', ui keyboard
[x]  'disableLocationUpdate', location
[x]  'onLoadSubPackageTaskStateChange', base app
[x]  'chooseMultiMedia', media other
[x]  'onUploadEncryptedFileToCDNProgress', network upload
[x]  'uploadEncryptedFileToCDN', network upload
[x]  'compressVideo', media video
[x]  'getVideoInfo', media video
[x]  'launchMiniProgram', base app
[x]  'requestSubscribeMessage', open-api subscribe
[x]  'navigateBackNative', open-api miniprogram-navigate
[x]  'operateDownloadTask', network download
[x]  'operateRequestTask', network request
[x]  'operateUploadTask', network  upload
[x]  'checkNetworkAPIURL', network other
[x]  'operateSocketTask', network socket
[x]  'reportPageData', open-api data-analysis
[x]  'onVoIPChatInterrupted', device phone
[x]  'onVoIPChatMembersChanged', device phone
[x]  'onVoIPChatSpeakersChanged', device phone
[x]  'onVoIPVideoMembersChanged',  device phone
[x]  'onNavigateBackIntercept', ui interaction
[x]  'setNavigationBarRightButton', navigation-bar
[x]  'showNavigationBar', ui navigation-bar
[x]  'hideHomeButton', ui other
[x]  'hideNavigationBar', ui navigation-bar
[x]  'initReady', other
[x]  'initReadyAfterRenderingCache', other
[x]  'initReadyForPrerender', other
[x]  'preloadWebview', ui webview
[x]  'rewriteRoute', route
[x]  'scrollWebviewTo', ui scroll
[x]  'setNavigateBackConfirmDialog', ui interaction
[x]  'setNavigateBackInterception', ui interaction
[x]  'requestFacetoFacePayment', open-api payment
[x]  'requestPersonalPay', open-api payment
[x]  'openBizProfile', open-api enterprise
[x]  'openUserProfile', open-api user-info
[x]  'profile', other
[x]  'noticePerformanceMetrics', device performance
[x]  'operateRecentUsageList', other
[x]  'scanItem', device scan
[x]  'hideShareTimelineMenu', open-api share
[x]  'shareTimeline', open-api share
[x]  'showShareMenuWithShareTicket', ui other
[x]  'showShareTimelineMenu', ui other
[x]  'updateShareMenuDynamic', ui other
[x]  'updateShareMenuShareTicket', ui other
[x]  'updateShareMenuToDo', ui other
[x]  'updateShareMenuUpdatable', ui other
[x]  'onCopyUrl', other
[x]  'hideVirtualBottomNavigationBar', ui navigation-bar
[x]  'openWeAppSearch', open-api other
[x]  'openWeAppProfile', open-api other
[x]  'onInitialRenderingCacheReady', other
[x]  'saveInitialRenderingCache', other
[x]  'onMemoryWarningReceive', device performance
[x]  'loadVideoResource', media video
[x]  'reportRealtimeAction', open-api data-analysis
[x]  'enableAccelerometer', device accelerometer
[x]  'enableCompass', device compass
[x]  'enableDeviceMotionChangeListening', device motion
[x]  'enableDeviceOrientationChangeListening', device other
[x]  'enableGyroscope', device gyroscope
[x]  'getSystemInfoAsync', base system
[x]  'onEnterLivePlayerPictureInPicture', ui other
[x]  'onLeaveLivePlayerPictureInPicture', ui other
[x]  'onEnterVideoPictureInPicture', ui other
[x]  'onLeaveVideoPictureInPicture', ui other
[x]  'operateWXData', open-api other
[x]  'adOperateWXData', ad
[x]  'private_quicklyAddBrandContact', device contact
[x]  'openBusinessView', ui other
[x]  'showKeyboard', ui keyboard
[x]  'updateInput', ui keyboard
[x]  'removeMapMarkers', media map
[x]  'setMapCenterOffset', media map
[x]  'setMapIndoorFloor', media map
[x]  'setMapIndoorMaskColor', media map
[x]  'setMapLocMarkerIcon', media map 
[x]  'toScreenLocation', media map
[x]  'translateMapMarker', media map
[x]  'updateMapGroundOverlay', media map
[x]  'updateMapMarkers', media map
[x]  'addMapCircles', media map
[x]  'addMapControls', media map
[x]  'addMapCustomLayer', media map
[x]  'addMapGroundOverlay', media map
[x]  'addMapLines', media map
[x]  'addMapMarkers', media map
[x]  'addMapPolygons', media map
[x]  'eraseMapLines', media map
[x]  'fromScreenLocation', media map
[x]  'getMapCenterLocation', media map
[x]  'getMapIndoorFloor', media map
[x]  'getMapRegion', media map
[x]  'getMapRotate', media map
[x]  'getMapScale', media map
[x]  'getMapSkew', media map
[x]  'includeMapPoints', media map
[x]  'initMapMarkerCluster', media map
[x]  'moveMapMarkerAlong', media map
[x]  'moveToMapLocation', media map
[x]  'removeMapGroundOverlay', media map
[x]  'removeMapCustomLayer', media map
[x]  'removeMapLines', media map
[x]  'createLoadSubPackageTask', base app
[x]  'navigateToDevMiniProgram', open-api miniprogram-navigate
[x]  'launchDevMiniProgram', base app
[x]  'createDownloadTask', network download
[x]  'createDownloadTaskAsync', network download 
[x]  'createRequestTask', network request
[x]  'createRequestTaskAsync', network request
[x]  'createUploadTask', network upload
[x]  'createUploadTaskAsync', network upload
[x]  'createSocketTask', network socket
[x]  'joinVoIPChat', device phone
[x]  'updateVoIPChatMuteConfig', device phone
[x]  'hasJoinVoIPChat', device phone
[x]  'operateCallTone', device phone
[x]  'subscribeVoIPMembers', device phone
[x]  'setDisplayOrientation', ui other
[x]  'private_setPageOrientation', ui other
[x]  'disableScrollBounce', ui scroll
[x]  'showDatePickerView', ui other
[x]  'showMultiPickerView', ui other
[x]  'showPickerView', ui other
[x]  'updateMultiPickerView', ui other
[x]  'shareAppMessage', open-api share
[x]  'shareAppMessageDirectly', open-api share
[x]  'shareAppMessageForFakeNative', open-api share
[x]  'getGlobalStorage', storage
[x]  'getGlobalStorageInfo', storage
[x]  'removeGlobalStorage', storage
[x]  'setGlobalStorage', storage
[x]  'removeHTMLWebView', ui webview
[x]  'drawCanvas', canvas
[x]  'insertCanvas', canvas
[x]  'insertWebGLCanvas', canvas
[x]  'removeCanvas', canvas
[x]  'removeWebGLCanvas', canvas
[x]  'updateCanvas', canvas
[x]  'updateWebGLCanvas', canvas
[x]  'insertCamera', canvas
[x]  'removeCamera', canvas
[x]  'updateCamera', canvas
[x]  'insertPositioningContainer', ui other
[x]  'removePositioningContainer', ui other
[x]  'updatePositioningContainer', ui other
[x]  'animateCoverView', ui other
[x]  'insertImagePreviewer', ui other
[x]  'insertImageView', ui other
[x]  'insertScrollView', ui other
[x]  'insertTextView', ui other
[x]  'removeImagePreviewer', ui other
[x]  'removeImageView', ui other
[x]  'removeScrollView', ui other
[x]  'removeTextView', ui other
[x]  'updateImagePreviewer', ui other
[x]  'updateImageView', ui other
[x]  'updateScrollView', ui other
[x]  'updateTextView', ui other
[x]  'insertTextArea', ui other
[x]  'updateTextArea', ui other
[x]  'updateMap', media map
[x]  'insertMap', media map
[x]  'removeMap', media map
[x]  'insertVoIPView', device phone
[x]  'removeVoIPView', device phone
[x]  'updateVoIPView', device phone
[x]  'join1v1VoIPChat', device phone
[x]  'shareAppMessageToSpecificContactDirectly', open-api share
[x]  'shareAppMessageToSpecificContactForFakeNativeDirectly', open-api share
[x]  'checkTrafficCardConditions', open-api other
[x]  'deleteTrafficCard', open-api other
[x]  'issueTrafficCard', open-api other
[x]  'queryTrafficCardInfo', open-api other
[x]  'rechargeTrafficCard', open-api other
[x]  'setDefaultTrafficCard', open-api other
}

% result of WeChat, total: 567
\ignore{
'network download': 22,
'base app': 20,
'device phone': 21,
'ui other': 46,
canvas: 21,
other: 47,
'open-api phone': 1,
'ui webview': 23,
'open-api account-info': 4,
'media audio': 12,
'open-api authorize': 5,
'open-api share': 8,
'open-api soter': 8,
'open-api payment': 28,
'open-api address': 2,
'open-api other': 36,
'base other': 5,
'device contacts': 3,
'base basic': 1,
'base debug': 2,
'network upload': 6,
'device screen': 7,
storage: 5,
'open-api data-analysis': 8,
'media other': 4,
'device nfc': 14,
'ui menu': 1,
'device scan': 2,
'open-api subscribe': 2,
'device other': 6,
'open-api werun': 3,
'device bluetooth-ble': 11,
'ui navigation-bar': 4,
location: 4,
'media video': 26,
'media live': 30,
'media map': 48,
'ui interaction': 7,
'media camera': 6,
'media image': 4,
'device iBeacon': 2,
'network request': 4,
'network websocket': 1,
'open-api miniprogram-navigate': 4,
'device contact': 6,
'base update': 2,
'open-api': 1,
'media recorder': 3,
'open-api user-info': 6,
'device bluetooth': 1,
'open-api performance': 1,
file: 1,
'ui keyboard': 5,
'network  upload': 1,
'network other': 1,
'network socket': 2,
'navigation-bar': 1,
route: 1,
'ui scroll': 2,
'open-api enterprise': 1,
'device performance': 2,
'device accelerometer': 1,
'device compass': 1,
'device motion': 1,
'device gyroscope': 1,
'base system': 1,
ad: 1
}

% following is wecom data
\ignore{
[x] sdk_navigateToMiniProgram, open-api miniprogram-navigation
[x] onAddToFavorites, open-api other
[x] onBackgroundAudioNext, media audio
[x] onBackgroundAudioPrev, media audio
[x] onBackgroundAudioStateChange, media audio
[x] onBLEConnectionStateChanged, device bluetooth-ble
[x] onCameraOutput, media camera
[x] operateBackgroundAudio, media audio
[x] setBackgroundAudioState, media audio
[x] qy__navigateBackNative, open-api miniprogram-navigation
[x] onCheckAppShareMessageEnable, open-api share
[x] onForwardAppMessage, open-api other
[x] loadLibFiles, base app
[x] onKeyboardComplete, ui keyboard
[x] onKeyboardConfirm, ui keyboard
[x] onKeyboardShow, ui keyboard
[x] exitMiniProgram, base app
[x] onUserOpStatistic, open-api data-analysis
[x] getCurrentRoute, route
[x] onNetworkWeakChange, network other
[x] onTapNavigationBarRightButton, ui navigation-bar
[x] qy__applyCodeForRestrictedChat, open-api enterprise
[x] qy__bioassayAuthentication, open-api soter
[x] qy__checkAppShareMessageEnable, open-api share
[x] qy__chooseAttach, file
[x] qy__chooseFile, file
[x] qy__chooseInvoice, open-api invoice
[x] qy__chooseWxworkContact, open-api enterprise
[x] qy__selectConvAndAction, open-api enterprise
[x] qy__chooseWxworkVisibleRange, open-api enterprise
[x] qy__getContext, base other
[x] qy__getMacAddress, device other
[x] qy__idcardVerify, open-api other 
[x] qy__bioassayFaceCompare, open-api soter
[x] qy__openChatWithMsg, open-api enterprise
[x] qy__openWechatWebviewUrl, ui webview
[x] qy__openWebview, ui webview
[x] qy__postNotification, base system
[x] qy__requestPayment, open-api payment
[x] qy__openWechatMiniProgram, open-api miniprogram-navigate
[x] qy__sendMessageToConv, open-api enterprise
[x] qy__sendMessageToWX, open-api other
[x] qy__shareAppMessageEx, open-api share
[x] qy__shareToExternalChat, open-api share
[x] qy__shareToExternalContact, open-api share
[x] qy__shareToTrainee, open-api share
[x] qy__shareToTraineeChat, open-api share
[x] qy__startWecast, open-api other
[x] qy__translateVoice, voice-recognition
[x] qy__wwLog, other
[x] qy__wwlogicInternal, other
[x] qy__wwOpenUrlScheme, other
[x] qy__showUserProfile, open-api user-info
[x] qy__enableShareToWxMenuGlobal, open-api share
[x] qy__openDeviceProfile, device other
[x] qy__enterHWOpenTalk, open-api other
[x] qy__queryCurrHWOpenTalk, open-api other
[x] qy__canIUsePrivate, open-api login
[x] qy__operatePrivate, open-api other
[x] qy__updateEnterpriseChat, open-api enterprise
[x] qy__chooseMessageFile, open-api enterprise
[x] qy__claimClassAdmin, open-api other
[x] qy__createCorpGroupChat, open-api enterprise
[x] qy__createSchoolPayment, open-api payment
[x] qy__getAvatar, open-api user-info
[x] qy__getCurExternalContact, open-api enterprise
[x] qy__getEmail, open-api user-info
[x] qy__getEnterpriseUserInfo, open-api enterprise
[x] qy__getMobile, open-api user-info
[x] qy__getQrCode, open-api enterprise
[x] qy__getShareInfo, open-api share
[x] qy__hideChatAttachmentMenu, ui menu
[x] qy__navigateToAddCustomer, open-api enterprise
[x] qy__navigateToKfChat, open-api enterprise
[x] qy__openEnterpriseContact, open-api enterprise
[x] qy__openExistChat, open-api enterprise
[x] qy__openThirdAppServiceChat, open-api enterprise
[x] qy__openUrl, open-api other
[x] qy__openUserProfile, open-api user-info
[x] qy__replayLiving, media live
[x] qy__selectPrivilegedContact, device contact
[x] qy__sendChatMessage, open-api enterprise
[x] qy__setShareAttr, open-api share
[x] qy__shareAppMessageToAdmin, open-api share
[x] qy__shareToExternalMoments, open-api share
[x] qy__startLiving, media live
[x] qy__startMeeting, open-api enterprise
[x] qy__updateCorpGroupChat, open-api enterprise
[x] qy__updateMomentsSetting,  open-api enterprise
[x] qy__downloadMedia, network download
[x] qy__uploadMedia, network upload
[x] qy__selectCorpGroupContact, open-api enterprise
[x] qy__discoverDevice, device other
[x] insertLivePlayer, media live
[x] insertLivePusher,  media live
[x] operateLivePlayer, media live
[x] operateLivePusher, media live
[x] removeLivePlayer, media live
[x] removeLivePusher, media live
[x] updateLivePlayer, media live
[x] updateLivePusher, media live
[x] insertVideoPlayer, media video
[x] operateVideoPlayer, media video
[x] removeVideoPlayer, media video
[x] updateVideoPlayer, media video
[x] qy__getUserInfo, open-api user-info
}

% final result:
\ignore{
  'open-api miniprogram-navigation': 2,
  'open-api other': 10,
  'media audio': 5,
  'device bluetooth-ble': 1,
  'media camera': 1,
  'open-api share': 12,
  'base app': 2,
  'ui keyboard': 3,
  'open-api data-analysis': 1,
  route: 1,
  'network other': 1,
  'ui navigation-bar': 1,
  'open-api enterprise': 22,
  'open-api soter': 2,
  file: 2,
  'open-api invoice': 1,
  'base other': 1,
  'device other': 3,
  'ui webview': 2,
  'base system': 1,
  'open-api payment': 2,
  'open-api miniprogram-navigate': 1,
  'voice-recognition': 1,
  other: 3,
  'open-api user-info': 6,
  'open-api login': 1,
  'ui menu': 1,
  'media live': 10,
  'device contact': 1,
  'network download': 1,
  'network upload': 1,
  'media video': 4
}

% following is tiktok
\ignore{
operateModalWebviewState, ui webview
hostLogin, open-api misc
startMock, device misc
stopMock, device misc
showActivityAd, ad
prefetchImages, media image
getUseDuration, open-api user-info
base64ToTempFilePath, base basic
base64ToTempFilePathSync, base basic
getCloudStorageByLocation, open-api misc
operateRecorder, media recorder
createAudioInstance, media audio
operateAudio, media audio
checkFollowAwemeState, open-api misc
destroyAudioInstance, media audio
setAudioState, media audio
getAudioState, media audio
getAudioStateSync, media audio
showEncourageCard, open-api misc
getBackgroundAudioContext, media audio
startFacialRecognitionVerify, open-api bio-auth
operateBgAudio, media audio
requestPayment, open-api payment
setBgAudioState, media audio
requestWXH5Payment, open-api payment
getBgAudioState, media audio
createPreloadVideoTask, media video
operatePreloadVideoTask, media video
createRequestTask, network request
operateRequestTask, network request
createInnerRequestTask, network request
operateInnerRequestTask, network request
createDownloadTask, network download
operateDownloadTask, network download
createInnerDownloadTask, network download
operateInnerDownloadTask, network download
createUploadTask, network upload
operateUploadTask, network upload
createInnerUploadTask, network upload
operateInnerUploadTask, network upload
createSocketTask, network websocket
operateSocketTask, network websocket
openUserProfile, open-api user-info
dealUserRelation, open-api user-info
createBannerAd, ad
openCustomerService, open-api misc
updateBannerAd, ad
operateBannerAd, ad
createVideoAd, ad
joinChatGroup, open-api misc
getAwemeChatGroupInfo, open-api misc
operateVideoAd, ad
operateInterstitialAd, ad
joinAwemeConversation, open-api misc
showECommerceAd, ad
launchApp, base app
setAnalyticsConfigSync, open-api misc
checkShortcut, uncatgorized
systemLog, base system
reportTimelinePoints, open-api misc
addShortcut, uncatgorized
_webviewGetPhoneNumber, open-api user-info
reportJsRuntimeError, open-api misc
sentryReport, open-api misc
_serviceGetPhoneNumber, open-api user-info
getLocalPhoneNumber, open-api user-info
reportMetrics, open-api misc
reportAppLog, open-api misc
getLocalPhoneNumberToken, open-api user-info
onBeforeCloseReturnSync, uncatgorized
getHostLaunchQuery, uncatgorized
createFollowButton, ui interaction
getHostLaunchQuerySync, uncatgorized
operateFollowButton, ui interaction
getCloudStorageByRelation, open-api misc
getUserCloudStorage, open-api misc
setSystemVolume, device misc
setUserCloudStorage, open-api misc
removeUserCloudStorage, open-api misc
getSystemVolume, device misc
getBatteryInfoSync, device misc
getBatteryInfo, device misc
isInUserFavoritesSync, open-api user-info
addToFavorites, open-api user-info
addToUserFavorites, open-api user-info
createDxppTask, uncatgorized
getFavoritesList, open-api user-info
operateDxppTask, uncatgorized
removeFromFavorites, open-api user-info
sortFavorites, open-api user-info
getDxppTaskStatusSync, uncatgorized
getSavedFileInfo, file
shareAppMessageDirectly, share
shareVideo, share
operateInternalStorageSync, storage
setMenuButtonVisibility, ui misc
showMorePanel, ui misc
protocolPathToAbsPath, base basic
getAppInfoSync, base app
setInputValue, ui misc
getRenderEnvSync, ui misc
getGeneralInfo, base basic
hideKeyboard, ui keyboard
getPerformanceTimingSync, open-api misc
getAppbrandSettingsSync, base app
callHostMethodSync, base system
callHostMethod, base system
addHostEventListener, base system
removeHostEventListener, base system
checkAppInstall, base system
launchAppDirectly, base app
canLaunchAppSync, base app
getRecentAppList, base system
sendUmengEventV1, open-api misc
removeFromRecentAppList, base system
showErrorPage, base misc
createCanvasEnvSync, canvas
preloadMiniProgram, base app
createHeliumCameraEnvSync, device camera
enableAccelerometer, device misc
openModalWebview, ui webview
closeModalWebview, ui webview
}

\ignore{
  'ui webview': 3,
  'open-api misc': 20,
  'device misc': 7,
  ad: 8,
  'media image': 1,
  'open-api user-info': 13,
  'base basic': 4,
  'media recorder': 1,
  'media audio': 10,
  'open-api bio-auth': 1,
  'open-api payment': 2,
  'media video': 2,
  'network request': 4,
  'network download': 4,
  'network upload': 4,
  'network websocket': 2,
  'base app': 6,
  uncatgorized: 8,
  'base system': 8,
  'ui interaction': 2,
  file: 1,
  share: 2,
  storage: 1,
  'ui misc': 4,
  'ui keyboard': 1,
  'base misc': 1,
  canvas: 1,
  'device camera': 1
}

% following is qq raw data
\ignore{
addMapCircles, media map
addMapControls, media map
addMapLines, media map
addMapMarkers, media map
addMapPolygons, media map
getMapCenterLocation, media map
getMapRegion, media map
getMapRotate, media map
getMapScale, media map
getMapSkew, media map
includeMapPoints, media map
insertMap, media map
moveToMapLocation, media map
removeMapMarkers, media map
translateMapMarker, media map
updateMap, media map
createAudioInstance, media audio
destroyAudioInstance, media audio
getAudioState, media audio
getBackgroundAudioState, media audio
getMusicPlayerState, media audio
operateAudio, media audio
operateBackgroundAudio, media audio
operateMusicPlayer, media audio
operateRecorder, media recorder
setAudioState, media audio
setBackgroundAudioState, media audio
drawCanvas, canvas
insertCanvas, canvas
updateCanvas, canvas
removeCanvas, canvas
hideVirtualBottomNavigationBar, ui navigation
hideVirtualBottomNavigationBar, ui navigation
insertXWebLivePlayer, media live
operateXWebLivePlayer, media live
removeXWebLivePlayer, media live
setDisplayOrientation, ui misc
showVirtualBottomNavigationBar, ui navigation
showVirtualBottomNavigationBar, ui navigation
updateXWebLivePlayer, media live
hideVirtualBottomNavigationBar, ui navigation
insertXWebLivePusher, media live
operateXWebLivePusher, media live
removeXWebLivePusher, media live
setDisplayOrientation, ui misc
showVirtualBottomNavigationBar, ui navigation
updateXWebLivePusher, media live
getVolume, device misc
hideVirtualBottomNavigationBar, ui navigation
insertXWebVideo, ui webview
operateXWebVideo, ui webview
removeXWebVideo, ui webview
setDisplayOrientation, ui misc
setVolume, device misc
showVirtualBottomNavigationBar, ui navigation
updateXWebVideo, ui webview
insertXWebExternalElement, ui webview
operateXWebExternalElement, ui webview
removeXWebExternalElement, ui webview
updateXWebExternalElement, ui webview
insertImageView, media image
removeImageView, media image
updateImageView, media image
customWebviewPostMessage, ui webview
insertCustomHTMLWebView, ui webview
insertHTMLWebView, ui webview
scrollWebviewTo, ui webview
removeHTMLWebView, ui webview
scrollWebviewTo, ui webview
updateCustomHTMLWebView, ui webview
updateHTMLWebView, ui webview
insertLivePlayer, media live
operateLivePlayer, media live
removeLivePlayer, media live
updateLivePlayer, media live
insertLivePusher, media live
operateLivePusher, media live
removeLivePusher, media live
updateLivePusher, media live
insertCamera, media camera
insertVideoPlayer, media video
operateCamera, media camera
operateVideoPlayer, media video
removeCamera, media camera
removeVideoPlayer, media video
updateCamera, media camera
updateVideoPlayer, media video
getRegionData, open-api misc
showDatePickerView, ui interaction
showMultiPickerView, ui interaction
showPickerView, ui interaction
updateMultiPickerView, ui interaction
disableScrollBounce, ui interaction
insertScrollView, ui interaction
removeScrollView, ui interaction
updateScrollView, ui interaction
toggleSecureWindow, ui interaction
createLoadSubPackageTask, base app
detectAbnormalLog, open-api misc
insertTextView, ui misc
removeTextView, ui misc
updateTextView, ui misc
operateRecorder, media recorder
createBlockAd, ad
operateBlockAd, ad
updateBlockAdSize, ad
operateCustomButton, ui misc
getOpenDataUserInfo, open-api user-info
navigateToMiniProgramConfig, open-api navigation
recordOffLineResourceState, open-api misc
downloadWithCache, network download
setMenuStyle, ui menu
setStatusBarStyle, ui misc
onAppEnterBackground, base app
onAppEnterForeground, base app
onAppStop, base app
registerProfile, open-api misc
timePerformanceResult, open-api misc
onRaffleShareSucNotice, share
minigameRaffle, uncategorized
onUpdateCheckResult, base app
onUpdateDownloadResult, base app
updateApp, base app
insertVideoPlayer, media video
operateVideoPlayer, media video
removeVideoPlayer, media video
updateVideoPlayer, media video
operateAppBox, uncategorized
cancelDownloadAppTask, base app
installApp, base app
isMicroAppInstalled, base app
queryAppInfo, base app
queryDownloadAppTask, base app
startApp, base app
startDownloadAppTask, base app
refreshSession, open-api misc
createBannerAd, ad
operateBannerAd, ad
updateBannerAdSize, ad
insertBookshelf, open-api misc
enterContact, device contact
openCustomerServiceConversation, open-api misc
getTextLineHeight, ui misc
private_addContact, device contact
batchGetContact, device contact
getCloudTicket, open-api misc
getGroupInfo, open-api misc
getGroupInfoExtra, open-api misc
getNativeUserInfo, open-api user-info
getNativeWeRunData, open-api misc
openWeRunSetting, open-api misc
getPerformance, open-api misc
getUserInfoExtra, open-api user-info
invokeGroupJSApi, open-api misc
operateAppAdData, ad
operateWXData, open-api misc
profile, uncategorized
reportSubmitForm, open-api misc
verifyPlugin, base app
addFavorites, open-api misc
addToFavorites, open-api misc
createDownloadTask, network download
createFileSystemInstance, file
createUploadTask, network upload
operateDownloadTask, network download
operateUploadTask, network upload
compressImage, media image
hideKeyboard, ui misc
setKeyboardValue, ui misc
showKeyboard, ui misc
updateInput, ui misc
updateKeyboard, ui misc
getQua, uncategorized
getStoreAppList, open-api misc
launchApplication, base app
notifyNative, open-api misc
openUrl, network misc
private_openUrl, network misc
operateInterstitialAd, ad
saveAppToDesktop, open-api misc
invokeNativePlugin, open-api misc
openNativePage, open-api misc
canUseComponent, uncategorized
getFriendCloudStorage, open-api misc
getGroupCloudStorage, open-api misc
getPotentialFriendList, open-api misc
getReactiveFriendList, open-api misc
getUserCloudStorage, open-api misc
getUserInteractiveStorage, open-api misc
modifyFriendInteractiveStorage, open-api misc
removeUserCloudStorage, open-api misc
setMessageToFriendQuery, open-api misc
setUserCloudStorage, open-api misc
shareMessageToFriend, share
checkH5PayStatus, open-api payment
consumeStarCurrency, open-api misc
queryStarCurrency, open-api misc
rechargeAndConsumeStarCurrency, open-api misc
rechargeStarCurrency, open-api misc
requestFriendPayment, open-api payment
requestMidasCoinPaymentByH5, open-api payment
requestMidasGoodsPay, open-api payment
requestMidasMonthCardPay, open-api payment
requestMidasPayment, open-api payment
requestMidasPaymentByH5, open-api payment
Personalize, open-api misc
preloadPackage, base app
addFriend, open-api misc
api_report, open-api misc
realtimeLog, open-api misc
reportDC, open-api misc
reportDataToDC, open-api misc
reportKeyValue, open-api misc
reportRealtimeAction, open-api misc
addGroupApp, open-api misc
createRequestTask, network request
createSocketTask, network websocket
getGroupAppStatus, open-api misc
operateRequestTask, network request
operateSocketTask, network websocket
wnsCgiRequest, network misc
wnsGroupRequest, network misc
wnsGuildRequest, network misc
wnsRequest, network misc
operateRewardedAd, ad
openScheme, open-api misc
enableAccelerometer, device misc
enableCompass, device misc
enableDeviceMotionChangeListening, device misc
enableGyroscope, device misc
openAddress, open-api misc
openQzonePublish, open-api misc
shareAppMessage, share
shareAppMessageDirectlyToFriendList, share
shareAppMessageDirectly, share
shareAppPictureMessage, share
shareAppPictureMessageDirectly, share
showShareMenuWithShareTicket, share
updateShareMenuShareTicket, share
getGlobalStorage, storage
setGlobalStorage, storage
getPhoneNumber, device phone
createUDPTask, network misc
operateUDPTask, network misc
insertTextArea, ui misc
updateTextArea, ui misc
removeTextArea, ui misc
hideHomeButton, ui misc
updateQQApp, open-api misc
hideMiniAIOEntrance, open-api misc
showMiniAIOEntrance, open-api misc
addColorSign, ui misc
addColorSignDirectly, ui misc
addRecentColorSign, ui misc
isColorSignExistSync, ui misc
exitMiniProgram, open-api misc
navigateToWeMiniProgram, open-api navigation
tav_createObject, uncategorized
tav_sendMsgToObject, uncategorized
tav_releaseObject, uncategorized
tav_util, uncategorized
tav_createObject, uncategorized
tav_sendMsgToObject, uncategorized
tav_releaseObject, uncategorized
tav_checkInit, uncategorized
getCMShowInfo, uncategorized
setCMShowPetStatus, uncategorized
getChannelUserInfo, open-api user-info
openExpandChat, open-api misc
getExpandUserInfo, open-api user-info
checkin_uploadRes, open-api misc
getMultiMemList, open-api misc
play_invokeGYCamera, media camera
checkin_invokeGYCamera, media camera
miniApp_invokeGYCamera, media camera
launchApp, open-api misc
nowlive, media live
openConnectAuthorize, open-api misc
qsubscribe_getdeviceinfo, open-api misc
qsubscribe_opendetail, open-api misc
qsubscribe_opendiscover, open-api misc
qsubscribe_openhomepage, open-api misc
checkin_qzoneUploadAndPublish, open-api misc
refreshQzoneFeed, open-api misc
uploadAvatar, open-api misc
tdoc_channel, uncategorized
openTenpayView, ui misc
qWalletBridge, open-api misc
tim_space, open-api misc
freeTrafficCardModel, open-api misc
groupAlbum_downloadGroupAlbumPhoto, open-api misc
groupAlbum_groupUploadPhoto, open-api misc
groupAlbum_importGroupAIO, open-api misc
groupAlbum_jumpCategoryAlbum, open-api misc
groupAlbum_jumpGroupAlbumSendBox, open-api misc
groupAlbum_openUserQzoneHome, open-api misc
groupAlbum_pickQzoneAlbum, open-api misc
groupAlbum_showGroupPhotoBrowser, open-api misc
groupAlbum_start, open-api misc
requestWebSSO, open-api misc
weiyunDownload, network download
}

\ignore{
'media map': 16,
  'media audio': 10,
  'media recorder': 2,
  canvas: 4,
  'ui navigation': 8,
  'media live': 17,
  'ui misc': 23,
  'device misc': 6,
  'ui webview': 16,
  'media image': 4,
  'media camera': 7,
  'media video': 8,
  'open-api misc': 80,
  'ui interaction': 9,
  'base app': 17,
  ad: 9,
  'open-api': 1,
  'open-api navigation': 2,
  'network download': 4,
  'ui menu': 1,
  share: 9,
  uncategorized: 16,
  'device contact': 3,
  'open-api user-info': 4,
  file: 1,
  'network upload': 2,
  'network misc': 8,
  'open-api payment': 7,
  'network request': 2,
  'network websocket': 2,
  storage: 2,
  'device phone': 1
}

% following is wechat privileged raw data
\ignore{
uploadToCommonCDN, network upload
navigateToMiniProgramDirectly, open-api navigate
batchGetContactDirectly, device contact
preloadMiniProgramEnvDirectly, base app
predownloadMiniProgramPackageDirectly, base app
getABTestConfig, base app
setCookies, open-api misc
getCookies, open-api misc
enterContact, device contact
playBackgroundAudio, media audio
pauseBackgroundAudio, media audio
stopBackgroundAudio, media audio
sendBizRedPacket, open-api payment
requestVirtualPayment, open-api payment
chooseMultiMedia, media other
chooseWeChatContact, device contacts
uploadEncryptedFileToCDN, network upload
checkIsSupportFacialRecognition, open-api bio-auth
startFacialRecognitionVerify, open-api bio-auth
startFacialRecognitionVerifyAndUploadVideo, open-api bio-auth
startCustomFacialRecognitionVerify, open-api bio-auth
startCustomFacialRecognitionVerifyAndUploadVideo, open-api bio-auth
launchMiniProgram, base app
launchApplicationDirectly, base app
launchApplicationForNative, base app
captureScreen, device screen
quicklyAddBrandContact, device contact
preloadWebview, ui webview
openDeliveryList, open-api misc
navigateBackNative, open-api navigate
stopHCE, device bluetooth
addNativeDownloadTask, network download
secureTunnel, uncategorized
verifyPaymentPassword, open-api payment
bindPaymentCard, open-api payment
requestPaymentToBank, open-api payment
openOfflinePayView, open-api payment
requestMallPayment, open-api payment
setCurrentPaySpeech, open-api payment
loadPaySpeechDialectConfig, open-api payment
requestJointPayment, open-api payment
openWCPayOverseaPaymentReceive, open-api payment
handleWCPayOverseaWalletBuffer, open-api payment
requestVerifyUserIdentity, open-api misc
faceVerifyForPay, open-api payment
openOfficialAccountProfile, open-api misc
openUserProfile, open-api user-info
openSelectPayment, open-api payment
requestEntrustAuthorization, open-api misc
requestFacetoFacePayment, open-api payment
openWeAppProfile, open-api misc
openWeAppSearch, open-api misc
openWeAppHistoryList, open-api misc
openWeAppStarList, open-api misc
checkTrafficCardConditions, open-api misc
queryTrafficCardInfo, open-api misc
issueTrafficCard, open-api misc
rechargeTrafficCard, open-api misc
setDefaultTrafficCard, open-api misc
openQRCode, device scan
makeVoIPCall, device phone
showShareActionSheet, share
bindGroup, open-api account-info
joinGroup, open-api account-info
chooseShareGroup, open-api misc

  'network upload': 2,
  'open-api navigate': 2,
  'device contact': 3,
  'base app': 6,
  'open-api misc': 16,
  'media audio': 3,
  'open-api payment': 15,
  'media other': 1,
  'device contacts': 1,
  'open-api bio-auth': 5,
  'device screen': 1,
  'ui webview': 1,
  'device bluetooth': 1,
  'network download': 1,
  uncategorized: 1,
  'open-api user-info': 1,
  'device scan': 1,
  'device phone': 1,
  share: 1,
  'open-api account-info': 2
}

% following is wecom priviledged data
\ignore{
qy__showUserProfile
qy__postNotification
qy__canIUsePrivate
qy__chooseAttach
qy__wwOpenUrlScheme
qy__sendMessageToWX
qy__chooseWxworkContact
qy__selectConvAndAction
qy__chooseWxworkVisibleRange
qy__openEnterpriseContact
qy__startWecast
qy__operatePrivate
qy__shareAppMessageToAdmin
qy__shareToExternalContact
qy__shareToExternalChat
qy__shareToTraineeChat
qy__shareToTrainee
}

% following is baidu priviledged data
\ignore{
quickLogin, open-api login
faceVerify, open-api bio-auth
getRealNameInfo, open-api user-info
queryQuickLoginInfo, open-api login
getFaceVerifyImage, open-api bio-auth
getChannelID, open-api misc
thirdPartyLogin, open-api misc
getExtensionJSVersion, base basic
getSeid, uncategorized
getPayStatus, open-api payment
getZidInfo, uncategorized
getAbSwitches, uncategorized
callGC, base system
getSystemStatus, base system
getBDUSS, open-api user-info
getCommonSysInfo, base system
getAdDeviceInfo, ad
login, open-api login
getDeviceInfo, open-api misc
getFavor, open-api misc
checkPhoneContactsAuthorization, device contact
getDebugConfig, base debug
confirmAppClose, base app
getHistory, open-api misc
getPhoneContacts, device contact
openBdboxWebview, ui webview
getUnionBDUSS, open-api user-info

'open-api login': 3,
  'open-api bio-auth': 2,
  'open-api user-info': 3,
  'open-api misc': 5,
  'base basic': 1,
  uncategorized: 3,
  'open-api payment': 1,
  'base system': 3,
  ad: 1,
  'device contact': 2,
  'base debug': 1,
  'base app': 1,
  'ui webview': 1
}

% following is tiktok
\ignore{
  downloadFile: '{"errMsg":"downloadFile:fail param.url should pass String, not Undefined"}',
  createMapContext: 'parameter mapId should be a string.',
  requestPayment: '{"errMsg":"requestPayment:fail param.data should pass Object, not Undefined"}',
  requestWXH5Payment: '{"errMsg":"requestWXH5Payment:fail permission denied"}',
  ucRequestPayment: '{"errMsg":"requestPayment:fail param.data should pass Object, not Undefined"}',
  performance: 'globalThis.tt[l] is not a function',
  cloud: 'globalThis.tt[l] is not a function',
  requestSubscribeMessage: '{"errMsg":"requestSubscribeMessage:fail params.tmplIds should be array, but got undefined","errNo":20000}',
  checkAppInstall: '{"errMsg":"checkAppInstall:fail param.packageName should pass String, not Undefined"}',
  requestSafari: '{"errMsg":"requestSafari:fail android does not support"}',
  launchAppDirectly: '{"errMsg":"launchAppDirectly:fail param.scheme should pass String, not Undefined"}',
  showActionSheet: '{"errMsg":"showActionSheet:fail params.itemList should be array, but got undefined","errNo":20000}',
  canIPutStuffOverComponent: 'canIPutStuffOverComponent:fail inputs[0] should be string, but got a(n) object',
  canIUse: 'canIUse: schema should be string',
  connectSocket: '{"errMsg":"connectSocket:fail params.url should be string, but got undefined","errNo":20000}',
  compressImage: '{"errMsg":"compressImage:fail params.src should be string, but got undefined","errNo":20000}',
  previewImage: '{"errMsg":"previewImage:fail params.urls should be array, but got undefined","errNo":20000}',
  interactionAnalysis: '{"errMsg":"interactionAnalysis:fail expect params.type to be one of "like", "favorite", "post_comment", but got undefined","errNo":20000}',
  showLoading: '{"errMsg":"showLoading:fail params.title should be string, but got undefined","errNo":20000}',
  makePhoneCall: '{"errMsg":"makePhoneCall:fail params.phoneNumber should be string, but got undefined","errNo":20000}',
  navigateTo: '{"errMsg":"navigateTo:fail params.url should be string, but got undefined","errNo":20000}',
  redirectTo: '{"errMsg":"redirectTo:fail params.url should be string, but got undefined","errNo":20000}',
  reLaunch: '{"errMsg":"reLaunch:fail params.url should be string, but got undefined","errNo":20000}',
  switchTab: '{"errMsg":"switchTab:fail params.url should be string, but got undefined","errNo":20000}',
  openSchema: '{"errMsg":"openSchema:fail params.schema should be string, but got undefined","errNo":20000}',
  request: '{"errMsg":"request:fail params.url should be string, but got undefined","errNo":20000}',
  showECommerceAd: '{"errMsg":"showECommerceAd:fail params.ad_unit_id should be string, but got undefined","errNo":20000}',
  saveVideoToPhotosAlbum: '{"errMsg":"saveVideoToPhotosAlbum:fail params.filePath should be string, but got undefined","errNo":20000}',
  authorize: '{"errMsg":"authorize:fail params.scope should be string, but got undefined","errNo":20000}',
  onBeforeExitMiniProgram: 'onBeforeExitMiniProgram:fail inputs[0] should be function, but got a(n) object',
  navigateToMiniProgram: '{"errMsg":"navigateToMiniProgram:fail params.appId should be string, but got undefined","errNo":20000}',
  getMoreGamesInfo: '{"errMsg":"getMoreGamesInfo:fail params.appId should be string, but got undefined\n' +
    'params.ticket should be string, but got undefined","errNo":20000}',
  openLocation: '{"errMsg":"openLocation:fail params.latitude should be number, but got undefined\n' +
    'params.longitude should be number, but got undefined","errNo":20000}',
  showDouyinOpenAuth: '{"errMsg":"showDouyinOpenAuth:fail params.scopes should be object, but got undefined","errNo":20000}',
  onAccelerometerChange: 'onAccelerometerChange:fail inputs[0] should be function, but got a(n) object',
  offAccelerometerChange: 'offAccelerometerChange:fail inputs[0] should be function or undefined, but got a(n) object',
  openDocument: '{"errMsg":"openDocument:fail params.filePath should be string, but got undefined","errNo":20000}',
  onCompassChange: 'onCompassChange:fail inputs[0] should be function, but got a(n) object',
  offCompassChange: 'offCompassChange:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppShow: 'onAppShow:fail inputs[0] should be function, but got a(n) object',
  offAppShow: 'offAppShow:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppHide: 'onAppHide:fail inputs[0] should be function, but got a(n) object',
  offAppHide: 'offAppHide:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppLaunch: 'onAppLaunch:fail inputs[0] should be function, but got a(n) object',
  offAppLaunch: 'offAppLaunch:fail inputs[0] should be function or undefined, but got a(n) object',
  openEcGood: '{"errMsg":"openEcGood:fail params.promotionId should be string, but got undefined","errNo":20000}',
  openDouyinProfile: '{"errMsg":"openDouyinProfile:fail params.userId should be string, but got undefined\n' +
    'params.shopId should be string, but got undefined","errNo":20000}',
  openEcCart: '{"errMsg":"openEcCart:fail params.shopId should be string, but got undefined","errNo":20000}',
  openEcCoupon: '{"errMsg":"openEcCoupon:fail params.shopId should be string, but got undefined\n' +
    'params.couponId should be string, but got undefined","errNo":20000}',
  openEcIm: '{"errMsg":"openEcIm:fail params.shopId should be string, but got undefined","errNo":20000}',
  openEcOrderDetail: '{"errMsg":"openEcOrderDetail:fail params.orderId should be string, but got undefined\n' +
    'params.shopId should be string, but got undefined","errNo":20000}',
  setTabBarBadge: '{"errMsg":"setTabBarBadge:fail params.index should be number, but got undefined\n' +
    'params.text should be string, but got undefined","errNo":20000}',
  removeTabBarBadge: '{"errMsg":"removeTabBarBadge:fail params.index should be number, but got undefined","errNo":20000}',
  showTabBarRedDot: '{"errMsg":"showTabBarRedDot:fail params.index should be number, but got undefined","errNo":20000}',
  hideTabBarRedDot: '{"errMsg":"hideTabBarRedDot:fail params.index should be number, but got undefined","errNo":20000}',
  setTabBarItem: '{"errMsg":"setTabBarItem:fail params.index should be number, but got undefined","errNo":20000}',
  setNavigationBarTitle: '{"errMsg":"setNavigationBarTitle:fail params.title should be string, but got undefined","errNo":20000}',
  setNavigationBarColor: '{"errMsg":"setNavigationBarColor:fail params.frontColor should be string, but got undefined\n' +
    'params.backgroundColor should be string, but got undefined","errNo":20000}',
  saveFile: '{"errMsg":"saveFile:fail params.tempFilePath should be string, but got undefined","errNo":20000}',
  getFileInfo: '{"errMsg":"getFileInfo:fail params.filePath should be string, but got undefined","errNo":20000}',
  removeSavedFile: '{"errMsg":"removeSavedFile:fail params.filePath should be string, but got undefined","errNo":20000}',
  reportAnalytics: 'reportAnalytics:fail the length of inputs should be greater than or equal to 2',
  getImageInfo: '{"errMsg":"getImageInfo:fail params.src should be string, but got undefined","errNo":20000}',
  getStorage: '{"errMsg":"getStorage:fail params.key should be string, but got undefined","errNo":20000}',
  setStorage: '{"errMsg":"setStorage:fail params.key should be string, but got undefined","errNo":20000}',
  removeStorage: '{"errMsg":"removeStorage:fail params.key should be string, but got undefined","errNo":20000}',
  setClipboardData: '{"errMsg":"setClipboardData:fail params.data should be string, but got undefined","errNo":20000}',
  preloadMiniProgram: '{"errMsg":"preloadMiniProgram:fail params.appList should be array, but got undefined","errNo":20000}',
  env: 'globalThis.tt[l] is not a function',
  createRewardedVideoAd: 'createRewardedVideoAd:fail inputs[0].adUnitId should be string, but got undefined',
  createEffectCameraStream: 'createEffectCameraStream:fail inputs[0].__webviewId__ should be number, but got undefined',
  uploadFile: '{"errMsg":"uploadFile:fail params.url should be string, but got undefined\n' +
    'params.filePath should be string, but got undefined\n' +
    'params.name should be string, but got undefined","errNo":20000}',
  getDownloadAppTaskStatusSync: 'getDownloadAppTaskStatusSync:fail inputs[0].app_name should be string, but got undefined\n' +
    'inputs[0].pkg_name should be string, but got undefined\n' +
    'inputs[0].download_url should be string, but got undefined',
  setSwipeBackMode: 'setSwipeBackMode:fail expect inputs[0] to be one of 0, 1, 2, but got a(n) object',
  offUserScreenRecord: 'offUserScreenRecord:fail inputs[0] should be function or undefined, but got a(n) object',
  createDownloadAppTask: 'createDownloadAppTask:fail inputs[0].apple_id should be string, but got undefined\n' +
    'inputs[0].download_url should be string, but got undefined\n' +
    'inputs[0].app_name should be string, but got undefined\n' +
    'inputs[0].pkg_name should be string, but got undefined',
  preloadVideo: '{"errMsg":"preloadVideo:fail the resource of video cannot be empty","errNo":21500}',
  getAmaz: 'getAmaz:fail platform auth deny',
  getAlgorithmManager: '{"errMsg":"getAlgorithmManager:fail params.width should be number, but got undefined\n' +
    'params.height should be number, but got undefined\n' +
    'params.useSyncMode should be boolean, but got undefined","errNo":20000}',
  createInterstitialAd: 'createInterstitialAd:fail inputs[0].adUnitId should be string, but got undefined',
  reportPOI: 'reportPOI:fail the length of inputs should be greater than or equal to 2',
  prefetchImages: '{"errMsg":"prefetchImages:fail params.images should be array, but got undefined","errNo":20000}',
  createTradeOrder: '{"errMsg":"createTradeOrder:fail params.goodsInfo should be array, but got undefined\n' +
    'params.totalAmount should be number, but got undefined","errNo":20000}',
  getTradeOrder: '{"errMsg":"getTradeOrder:fail params.orderId should be string, but got undefined","errNo":20000}',
  createTradeRefundOrder: '{"errMsg":"createTradeRefundOrder:fail params.orderId should be string, but got undefined\n' +
    'params.reason should be string, but got undefined\n' +
    'params.type should be string, but got undefined\n' +
    'params.description should be string, but got undefined","errNo":20000}',
  getTradeRefundOrder: '{"errMsg":"getTradeRefundOrder:fail params.refundOrderId should be string, but got undefined","errNo":20000}',
  completeRefundSync: 'completeRefundSync:fail the length of inputs should be greater than or equal to 2',
  onError: 'onError:fail inputs[0] should be function, but got a(n) object',
  offError: 'offError:fail inputs[0] should be function or undefined, but got a(n) object',
  callHostMethod: '{"errMsg":"callHostMethod:fail params.method should be string, but got undefined","errNo":20000}',
  callHostMethodSync: 'callHostMethodSync:fail inputs[0].method should be string, but got undefined',
  addHostEventListener: 'addHostEventListener:fail the length of inputs should be greater than or equal to 2',
  rateAwemeOrder: '{"errMsg":"rateAwemeOrder:fail params.orderId should be string, but got undefined","errNo":20000}',
  canRateAwemeOrders: '{"errMsg":"canRateAwemeOrders:fail params.orderIds should be array, but got undefined","errNo":20000}'
}

% following is qq raw data
\ignore{
  enterContact: '{"errMsg":"enterContact:fail no permission"}',
  getQimei36: '{"errMsg":"getQimei36:fail no permission"}',
  openScheme: '{"errMsg":"openScheme:fail no permission"}',
  invokeNativePlugin: '{"errMsg":"invokeNativePlugin:fail no permission"}',
  navigateToBookshelf: '{"errMsg":"navigateToBookshelf:fail no permission"}',
  getUserInfo: '{"errMsg":"getUserInfo:fail auth deny"}'
}


==> tables/api-category.tex <==


\begin{table*}[h]
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1.2}
\scriptsize

 
\begin{tabular}{cccrcrcrcrcrcrcrcrcrcrcrcrcrcrcr}
\toprule[1.5pt]

    \multicolumn{2}{c}{
        \multirow{2}{*}{\textbf{Available APIs}}} &

    \multicolumn{6}{c}{
        \textbf{WeChat}
    } &
    \multicolumn{6}{c}{
        \textbf{WeCom}
    } &
    \multicolumn{6}{c}{
        \textbf{Baidu}
    } & 
    \multicolumn{6}{c}{
        \textbf{Tiktok}
    } & 
    \multicolumn{6}{c}{
        \textbf{QQ}
    } \\
    \cline{3-32}

    \multicolumn{2}{c}{} &
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            U
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            P
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            U
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            P
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            U
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            P
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            U
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            P
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            D
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            U
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}
            P
        \end{tabular} &
        \begin{tabular}[c]{@{}c@{}}
            \%
        \end{tabular} \\ 

\midrule[0.5pt]


\multirow{4}{*}{Base}
    & Basic                 &  5 &71.4 &  2 &28.6 &  - & 0.0 &  6 &66.7 &  3 &33.3 &  - & 0.0 &  8 &72.7 &  3 &27.3 &  1 & 9.1 &  7 &63.6 &  4 &36.4 &  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & App                   & 13 &39.4 & 20 &60.6 &  6 &18.2 & 13 &37.1 & 22 &62.9 &  6 &17.1 &  8 &42.1 & 11 &57.9 &  1 & 5.3 &  6 &50.0 &  6 &50.0 &  - & 0.0 &  9 &34.6 & 17 &65.4 &  - & 0.0 \\ \cline{2-32}
    & Debug                 & 15 &88.2 &  2 &11.8 &  - & 0.0 & 15 &88.2 &  2 &11.8 &  - & 0.0 &  1 & 3.3 & 29 &96.7 &  1 & 3.3 &  0 & 0.0 &  - & 0.0 &  - & 0.0 & 20 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Misc                  & 10 &58.8 &  7 &41.2 &  - & 0.0 & 10 &55.6 &  8 &44.4 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 & 10 &52.6 &  9 &47.4 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multirow{5}{*}{UI}
    & Interaction           &  6 &46.2 &  7 &53.8 &  - & 0.0 &  6 &46.2 &  7 &53.8 &  - & 0.0 &  7 &41.2 & 10 &58.8 &  - & 0.0 &  9 &81.8 &  2 &18.2 &  - & 0.0 &  6 &40.0 &  9 &60.0 &  - & 0.0 \\ \cline{2-32}
    & Navigation            &  4 &44.4 &  5 &55.6 &  - & 0.0 &  4 &40.0 &  6 &60.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 &  5 &100.0&  - & 0.0 &  - & 0.0 &  4 &33.3 &  8 &66.7 &  - & 0.0 \\ \cline{2-32}
    & Animation             & 32 &100.0&  - & 0.0 &  - & 0.0 & 32 &100.0&  - & 0.0 &  - & 0.0 & 21 &95.5 &  1 & 4.5 &  - & 0.0 &  1 &100.0&  - & 0.0 &  - & 0.0 & 31 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & WebView               &  0 & 0.0 & 23 &100.0&  1 & 4.3 &  0 & 0.0 & 25 &100.0&  1 & 4.0 &  0 & 0.0 &  4 &100.0&  1 &25.0 &  0 & 0.0 &  3 &100.0&  - & 0.0 &  0 & 0.0 & 16 &100.0&  - & 0.0 \\ \cline{2-32}
    & Misc                  & 20 &27.0 & 54 &73.0 &  - & 0.0 & 20 &25.6 & 58 &74.4 &  - & 0.0 & 37 &77.1 & 11 &22.9 &  - & 0.0 & 14 &73.7 &  5 &26.3 &  - & 0.0 & 18 &42.9 & 24 &57.1 &  - & 0.0 \\ \cline{1-32}

\multirow{5}{*}{Network}
    & Request               &  5 &55.6 &  4 &44.4 &  - & 0.0 &  5 &55.6 &  4 &44.4 &  - & 0.0 &  2 &66.7 &  1 &33.3 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  4 &66.7 &  2 &33.3 &  - & 0.0 \\ \cline{2-32}
    & Download              &  7 &24.1 & 22 &75.9 &  1 & 3.4 &  7 &23.3 & 23 &76.7 &  1 & 3.3 & 11 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  4 &100.0&  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 \\ \cline{2-32}
    & Upload                &  7 &50.0 &  7 &50.0 &  2 &14.3 &  7 &46.7 &  8 &53.3 &  2 &13.3 &  6 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  4 &100.0&  - & 0.0 &  6 &75.0 &  2 &25.0 &  - & 0.0 \\ \cline{2-32}
    & Websocket             & 14 &93.3 &  1 & 6.7 &  - & 0.0 & 14 &93.3 &  1 & 6.7 &  - & 0.0 & 13 &100.0&  - & 0.0 &  - & 0.0 &  7 &77.8 &  2 &22.2 &  - & 0.0 & 13 &86.7 &  2 &13.3 &  - & 0.0 \\ \cline{2-32}
    & Misc                  & 23 &88.5 &  3 &11.5 &  - & 0.0 & 23 &85.2 &  4 &14.8 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 & 10 &55.6 &  8 &44.4 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Storage}
                            & 10 &66.7 &  5 &33.3 &  - & 0.0 & 10 &66.7 &  5 &33.3 &  - & 0.0 & 10 &100.0&  - & 0.0 &  - & 0.0 & 10 &90.9 &  1 & 9.1 &  - & 0.0 & 10 &83.3 &  2 &16.7 &  - & 0.0 \\ \cline{1-32}

\multirow{8}{*}{Media}
    & Map                   &  8 &14.3 & 48 &85.7 &  - & 0.0 &  8 &14.3 & 48 &85.7 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  6 &100.0&  - & 0.0 &  - & 0.0 &  9 &36.0 & 16 &64.0 &  - & 0.0 \\ \cline{2-32}
    & Image                 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 &  6 &85.7 &  1 &14.3 &  - & 0.0 &  5 &83.3 &  1 &16.7 &  - & 0.0 &  6 &60.0 &  4 &40.0 &  - & 0.0 \\ \cline{2-32}
    & Video                 & 14 &35.0 & 26 &65.0 &  - & 0.0 & 14 &31.8 & 30 &68.2 &  - & 0.0 & 19 &95.0 &  1 & 5.0 &  - & 0.0 &  8 &80.0 &  2 &20.0 &  - & 0.0 & 14 &63.6 &  8 &36.4 &  - & 0.0 \\ \cline{2-32}
    & Audio                 & 64 &84.2 & 12 &15.8 &  3 & 0.0 & 64 &79.0 & 17 &21.0 &  3 & 3.7 & 44 &100.0&  - & 0.0 &  - & 0.0 & 44 &81.5 & 10 &18.5 &  - & 0.0 & 61 &85.9 & 10 &14.1 &  - & 0.0 \\ \cline{2-32}
    & Live                  & 26 &46.4 & 30 &53.6 &  - & 3.9 & 26 &39.4 & 40 &60.6 &  - & 0.0 &  8 &100.0&  - & 0.0 &  - & 0.0 & 19 &100.0&  - & 0.0 &  - & 0.0 & 23 &57.5 & 17 &42.5 &  - & 0.0 \\ \cline{2-32}
    & Recorder              & 16 &84.2 &  3 &15.8 &  - & 0.0 & 16 &84.2 &  3 &15.8 &  - & 0.0 & 12 &100.0&  - & 0.0 &  - & 0.0 & 11 &91.7 &  1 & 8.3 &  - & 0.0 & 15 &88.2 &  2 &11.8 &  - & 0.0 \\ \cline{2-32}
    & Camera                &  9 &60.0 &  6 &40.0 &  - & 0.0 &  9 &52.9 &  8 &47.1 &  - & 0.0 &  9 &50.0 &  9 &50.0 &  - & 0.0 & 20 &95.2 &  1 & 4.8 &  - & 0.0 &  4 &36.4 &  7 &63.6 &  - & 0.0 \\ \cline{2-32}
    & Misc                  & 12 &75.0 &  4 &25.0 &  1 & 0.0 & 12 &75.0 &  4 &25.0 &  1 & 6.3 & 18 &100.0&  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  6 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Location} 
                            &  3 &42.9 &  4 &57.1 &  - & 6.3 &  3 &42.9 &  4 &57.1 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Share}
                            &  4 &33.3 &  8 &66.7 &  1 & 0.0 &  4 &16.7 & 20 &83.3 &  1 & 4.2 &  3 &100.0&  - & 0.0 &  - & 0.0 &  5 &71.4 &  2 &28.6 &  - & 0.0 &  5 &35.7 &  9 &64.3 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Canvas}
                            & 60 &74.1 & 21 &25.9 &  - & 8.3 & 60 &74.1 & 21 &25.9 &  - & 0.0 & 46 &92.0 &  4 & 8.0 &  - & 0.0 & 49 &98.0 &  1 & 2.0 &  - & 0.0 & 48 &92.3 &  4 & 7.7 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{File}
                            & 39 &97.5 &  1 & 2.5 &  - & 0.0 & 39 &92.9 &  3 & 7.1 &  - & 0.0 & 35 &100.0&  - & 0.0 &  - & 0.0 & 34 &97.1 &  1 & 2.9 &  - & 0.0 & 37 &97.4 &  1 & 2.6 &  - & 0.0 \\ \cline{1-32}

\multirow{7}{*}{Open API}
    & Login                 &  2 &100.0&  - & 0.0 &  - & 0.0 &  5 &83.3 &  1 &16.7 &  - & 0.0 &  3 &75.0 &  1 &25.0 &  3 &75.0 &  2 &100.0&  - & 0.0 &  - & 0.0 &  2 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Navigate              &  2 &33.3 &  4 &66.7 &  2 & 0.0 &  2 &22.2 &  7 &77.8 &  2 &22.2 &  3 &100.0&  - & 0.0 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  2 &50.0 &  2 &50.0 &  1 &25.0 \\ \cline{2-32}
    & User Info             &  2 &16.7 & 10 &83.3 &  3 &33.3 &  5 &23.8 & 16 &76.2 &  3 &14.3 &  1 &10.0 &  9 &90.0 &  3 &30.0 &  2 &13.3 & 13 &86.7 &  - & 0.0 &  2 &28.6 &  5 &71.4 &  1 &14.3 \\ \cline{2-32}
    & Payment               &  1 & 3.4 & 28 &96.6 & 15 &25.0 &  1 & 3.2 & 30 &96.8 & 15 &48.4 &  1 &50.0 &  1 &50.0 &  1 &50.0 &  1 &33.3 &  2 &66.7 &  1 &33.3 &  2 &22.2 &  7 &77.8 &  - & 0.0 \\ \cline{2-32}
    & Bio-Auth              &  3 &27.3 &  8 &72.7 &  5 &51.7 &  3 &21.4 & 11 &78.6 &  5 &35.7 &  0 & 0.0 &  0 & 0.0 &  - & 0.0 &  0 & 0.0 &  1 &100.0&  - & 0.0 &  3 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Enterprise            &  0 & 0.0 &  1 &100.0&  - &45.5 &  5 &17.9 & 23 &82.1 & 17 &60.7 &  0 & 0.0 &  0 & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Misc                  & 14 &19.4 & 58 &80.6 & 16 & 0.0 & 14 &16.7 & 70 &83.3 & 16 &19.0 & 16 &57.1 & 12 &42.9 & 10 &35.7 & 25 &55.6 & 20 &44.4 &  - & 0.0 & 12 &13.0 & 80 &87.0 &  2 & 2.2 \\ \cline{1-32}

\multirow{7}{*}{Device}
    & Wi-Fi                 &  9 &100.0&  - & 0.0 &  - &22.2 &  9 &100.0&  - & 0.0 &  - & 0.0 & 10 &100.0&  - & 0.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Bluetooth             & 18 &60.0 & 12 &40.0 &  1 & 0.0 & 18 &58.1 & 13 &41.9 &  1 & 3.2 &  - & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 & 18 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Contact               &  1 &10.0 &  9 &90.0 &  4 & 3.3 &  1 & 9.1 & 10 &90.9 &  4 &36.4 &  1 &33.3 &  2 &66.7 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  1 &25.0 &  3 &75.0 &  1 &25.0 \\ \cline{2-32}
    & NFC                   &  5 &26.3 & 14 &73.7 &  - &40.0 &  9 &39.1 & 14 &60.9 &  - & 0.0 &  - &33.3 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  5 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Screen                &  4 &36.4 &  7 &63.6 &  1 & 0.0 &  4 &36.4 &  7 &63.6 &  1 & 9.1 &  3 &100.0&  - & 0.0 &  - & 0.0 &  9 &100.0&  - & 0.0 &  - & 0.0 &  4 &100.0&  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Phone                 &  1 & 4.3 & 22 &95.7 &  1 & 9.1 &  1 & 4.3 & 22 &95.7 &  1 & 4.3 &  1 &100.0&  - & 0.0 &  - & 0.0 &  1 &100.0&  - & 0.0 &  - & 0.0 &  1 &50.0 &  1 &50.0 &  - & 0.0 \\ \cline{2-32}
    & Misc                  & 28 &63.  & 16 &36.4 &  1 & 4.3 & 28 &59.6 & 19 &40.4 &  1 & 2.1 & 21 &80.8 &  5 &19.2 &  - & 0.0 & 16 &69.6 &  7 &30.4 &  - & 0.0 & 28 &82.4 &  6 &17.6 &  - & 0.0 \\ \cline{1-32}

\multirow{2}{*}{AI}
    & CV                    & 19 &100.0&  - & 0.0 &  - & 2.3 & 19 &100.0&  - & 0.0 &  - & 0.0 & 18 &90.0 &  2 &10.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ \cline{2-32}
    & Misc                  &  0 & 0.0 &  - & 0.0 &  - & 0.0 &  0 & 0.0 &  1 &100.0&  - & 0.0 & 11 &100.0&  - & 0.0 &  - & 0.0 &  7 &100.0&  - & 0.0 &  - & 0.0 &  0 & 0.0 &  - & 0.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{AD}
                            & 19 &95.0 &  1 & 5.0 &  - & 0.0 & 19 &95.0 &  1 & 5.0 &  - & 0.0 &  9 &64.3 &  5 &35.7 &  1 & 7.1 & 13 &61.9 &  8 &38.1 &  - & 0.0 &  3 &25.0 &  9 &75.0 &  - & 0.0 \\ \cline{1-32}

\multicolumn{2}{c}{Uncategorized}
                            & 30 &38.5 & 48 &61.5 &  1 & 1.3 & 30 &36.6 & 52 &63.4 &  1 & 1.2 & 15 &53.6 & 13 &46.4 &  3 &10.7 & 17 &68.0 &  8 &32.0 &  1 & 4.0 & 34 &68.0 & 16 &32.0 &  1 & 2.0 \\

\midrule[0.5pt]

\multicolumn{2}{c}{\textbf{All}}
                            &590 &51.0 &567 &49.0 & 65 & 5.6 &606 &47.3 &675 &52.7 & 82 & 6.4 &464 &77.5 &135 &22.5 & 25 & 4.2 &383 &75.8 &122 &24.2 &  2 & 0.4 &506 &62.7 &301 &37.3 &  6 & 0.7 \\
\bottomrule[1.5pt]
\end{tabular}
\vspace{2mm}
\caption{Categories of Official and Hidden APIs. ``D'' means documented APIs;  ``U'' means undocumented APIs; ``P'' means privileged APIs \ZY{HEATMAP}} 
% due to page limit
\label{tab:compare:api}
\end{table*}

% undefined means no subcategory
% | category | subcategory | # of WeChat Official API | # of WeCom Official API | # of Baidu Official API | # of WeChat Hidden API | # of WeCom Hidden API | # of Baidu Hidden API | Required Permission |
% | base     | undefined            |  3 |  4 |  5 |   |   |    |    | 
% | base     | system               |  2 |  2 |  3 |   |   |    |    |
% | base     | update               |  6 |  6 |  5 |   |   |    |    |
% | base     | app                  | 13 | 13 |  8 |   |   |    |    |
% | base     | debug                | 15 | 15 |  1 |   |   |    |    |
% | base     | timer                |  4 |  4 |  4 |   |   |    |    |
% | route    | undefined            |  5 |  5 |  5 |   |   |    |    |
% | ui       | interaction          |  6 |  6 |  7 |   |   |    |    |
% | ui       | navigation-bar       |  4 |  4 |  4 |   |   |    |    |
% | ui       | background           |  2 |  2 |  2 |   |   |    |    |
% | ui       | tab-bar              |  8 |  8 |  8 |   |   |    |    |
% | ui       | pull-down-refresh    |  2 |  2 |  3 |   |   |    |    |
% | ui       | scroll               |  1 |  1 |  1 |   |   |    |    |
% | ui       | animation            | 32 | 32 | 21 |   |   |    |    |
% | ui       | sticky               |  1 |  1 |  0 |   |   |    |    |
% | ui       | custom-component     |  1 |  1 |  1 |   |   |    |    |
% | ui       | menu                 |  1 |  1 |  1 |   |   |    |    |
% | ui       | window               |  2 |  2 |  4 |   |   |    |    |
% | ui       | keyboard             |  2 |  2 |  3 |   |   |    |    |
% | ui       | node-info            |  0 |  0 | 14 |   |   |    |    |
% | network  | request              |  5 |  5 |  2 |   |   |    |    |
% | network  | download             |  7 |  7 | 11 |   |   |    |    |
% | network  | upload               |  7 |  7 |  6 |   |   |    |    |
% | network  | websocket            | 14 | 14 | 13 |   |   |    |    |
% | network  | mdns                 | 10 | 10 |  0 |   |   |    |    |
% | network  | udp                  | 13 | 13 |  0 |   |   |    |    |
% | storage  | undefined            | 10 | 10 | 10 |   |   |    |    |
% | media    | map                  |  8 |  8 |  7 |   |   |    |    |
% | media    | image                |  6 |  6 |  6 |   |   |    |    |
% | media    | video                | 14 | 14 | 19 |   |   |    |    |
% | media    | audio                | 38 | 38 | 27 |   |   |    |    |
% | media    | background-audio     | 26 | 26 | 17 |   |   |    |    |
% | media    | live                 | 26 | 26 |  8 |   |   |    |    |
% | media    | recorder             | 16 | 16 | 12 |   |   |    |    |
% | media    | camera               |  9 |  9 |  9 |   |   |    |    |
% | media    | editor               | 11 | 11 |  4 |   |   |    |    |
% | media    | font                 |  1 |  1 |  0 |   |   |    |    |
% | media    | RTC                  |  0 |  0 | 13 |   |   |    |    |
% | media    | TTS                  |  0 |  0 |  1 |   |   |    |    |
% | location | undefined            |  3 |  3 |  7 |   |   |    |    |
% | share    | undefined            |  4 |  4 |  3 |   |   |    |    |
% | canvas   | undefined            | 60 | 60 | 46 |   |   |    |    |
% | file     | undefined            | 39 | 39 | 35 |   |   |    |    |
% | open-api | login                |  2 |  5 |  3 |   |   |    |    | 
% | open-api | miniprogram-navigate |  2 |  2 |  3 |   |   |    |    |
% | open-api | account-info         |  1 |  1 |  0 |   |   |    |    |
% | open-api | user-info            |  2 |  5 |  1 |   |   |    |    |
% | open-api | report               |  1 |  1 |  0 |   |   |    |    |
% | open-api | data-analysis        |  1 |  1 |  1 |   |   |    |    |
% | open-api | payment              |  1 |  1 |  1 |   |   |    |    |
% | open-api | authorize            |  1 |  1 |  1 |   |   |    |    |
% | open-api | setting              |  3 |  3 |  2 |   |   |    |    |
% | open-api | address              |  1 |  1 |  1 |   |   |    |    |
% | open-api | card                 |  2 |  2 |  0 |   |   |    |    |
% | open-api | invoice              |  2 |  2 |  1 |   |   |    |    |
% | open-api | subscribe            |  1 |  1 |  1 |   |   |    |    |
% | open-api | soter                |  3 |  3 |N/A |   |   |N/A |    |
% | open-api | werun                |  1 |  1 |N/A |   |   |N/A |    |
% | open-api | enterprise           |  0 |  5 |N/A |   |   |N/A |    |
% | open-api | package              |  0 |  0 |  3 |   |   |    |    |
% | open-api | system-risk          |  0 |  0 |  1 |   |   |    |    |
% | open-api | Bookshelf            |N/A |N/A |  5 |   |   |    |    |
% | device   | ibeacon              |  6 |  6 |  0 |   |   |    |    |
% | device   | wifi                 |  9 |  9 | 10 |   |   |    |    |
% | device   | bluetooth-ble        |  9 |  9 |  0 |   |   |    |    |
% | device   | contact              |  1 |  1 |  1 |   |   |    |    |
% | device   | bluetooth            |  9 |  9 |  0 |   |   |    |    |
% | device   | battery              |  2 |  2 |  2 |   |   |    |    |
% | device   | clipboard            |  2 |  2 |  2 |   |   |    |    |
% | device   | nfc                  |  5 |  9 |  0 |   |   |    |    |
% | device   | network              |  2 |  2 |  2 |   |   |    |    |
% | device   | screen               |  4 |  4 |  3 |   |   |    |    |
% | device   | phone                |  1 |  1 |  1 |   |   |    |    |
% | device   | accelerometer        |  3 |  3 |  3 |   |   |    |    |
% | device   | compass              |  3 |  3 |  3 |   |   |    |    |
% | device   | motion               |  3 |  3 |  3 |   |   |    |    |
% | device   | gyroscope            |  3 |  3 |  0 |   |   |    |    |
% | device   | performance          |  1 |  1 |  1 |   |   |    |    |
% | device   | scan                 |  1 |  1 |  1 |   |   |    |    |
% | device   | vibrate              |  2 |  2 |  2 |   |   |    |    |
% | device   | calendar             |  0 |  0 |  2 |   |   |    |    |
% | cloud    | storage              |N/A |N/A |  3 |   |   |    |    |
% | cloud    | function             |N/A |N/A |  1 |   |   |    |    |
% | cloud    | init                 |N/A |N/A |  1 |   |   |    |    |
% | cloud    | database             |N/A |N/A |  3 |   |   |    |    |
% | ai       | vision               | 16 | 16 |N/A |   |   |    |    |
% | ai       | OCR                  |  0 |  0 |  4 |   |   |    |    |
% | ai       | voice-recognition    |  0 |  0 |  8 |   |   |    |    |
% | ai       | text-to-audio        |  0 |  0 |  1 |   |   |    |    |
% | ai       | text-review          |  0 |  0 |  1 |   |   |    |    |
% | ai       | nlp-lexer            |  0 |  0 |  1 |   |   |    |    |
% | ai       | image-classify       |  0 |  0 |  7 |   |   |    |    |
% | ai       | image-audit          |  0 |  0 |  1 |   |   |    |    |
% | ai       | face-detection       |  3 |  3 |  6 |   |   |    |    |
% | worker   | undefined            |  5 |  5 |  0 |   |   |    |    |
% | ext      | undefined            |  2 |  2 |  2 |   |   |    |    |
% | wxml     | undefined            | 18 | 18 |  0 |   |   |N/A |    |
% | ad       | undefined            | 19 | 19 |  9 |   |   |  5 |    |
% | misc     | undefined            |N/A |N/A |N/A |   |   |    |    |    

% total baidu hidden API: 135
\ignore{
[x] /swanAPI/dataChannel',      other
[x] /swanAPI/cloudRequest',     cloud other
[x] /swanAPI/aiRequest',        ai other
[x] /swanAPI/im/pullMsg',       other
[x] /swanAPI/privateGetUserInfo',  open-api user-info
[x] /swanAPI/publishThread',       open-api other
[x] /swanAPI/camera/update',       media camera
[x] /swanAPI/camera/remove',       media camera
[x] /swanAPI/camera/insert',       media camera
[x] /swanAPI/setTplBdussSync',     open-api user-info
[x] /swanAPI/setSelectedAddressSync', open-api user-info
[x] /swanAPI/installApp4Ad',       ad
[x] /swanAPI/getChannelID',        other
[x] /swanAPI/getPushSettingStateSync', device other
[x] /swanAPI/guidePushSetting',        device other
[x] /swanAPI/coverimage',              ui interaction
[x] /swanAPI/coverview',               ui interaction
[x] /swanAPI/debuggerlaunch',          debug
[x] /swanAPI/remoteDebug',             debug
[x] /swanAPI/sConsole',                debug
[x] /swanAPI/joinActivity',            open-api other
[x] /swanAPI/activityRequest',         open-api other
[x] /swanAPI/addActivityFavor',        open-api other
[x] /swanAPI/wirelessdebuglaunch',     debug
[x] /swanAPI/launch',                  base app
[x] /swanAPI/perfCat',                 debug
[x] /swanAPI/ARCamera/detectContent',  media camera
[x] /swanAPI/ARCamera/insert',         media camera
[x] /swanAPI/ARCamera/remove',         media camera
[x] /swanAPI/ARCamera/changeARStatus', media camera
[x] /swanAPI/ARCamera/arMessage',      media camera
[x] /swanAPI/ARCamera/update',         media camera
[x] /swanAPI/adRequest',               ad
[x] /swanAPI/openAdWebPage',           ad
[x] /swanAPI/openAdLandingPage',       ad
[x] /swanAPI/debug/setWebDegradeDebugHost', debug
[x] /swanAPI/localdebuglaunch',             debug
[x] /swanAPI/openFullScreenView',           ui window
[x] /swanAPI/closeFullScreenView',          ui window
[x] /swanAPI/imageRecognition',             ai vision
[x] /swanAPI/debug/setReplaceSwanCoreConfig',  debug
[x] /swanAPI/debugSwanCore',                   debug
[x] /swanAPI/debug/setReplaceDynamicLibConfig', debug
[x] /swanAPI/debug/setExtensionConfig',         debug
[x] /swanAPI/debug/setCtsConfig',               debug
[x] /swanAPI/debug/setReplaceDependencyConfig', debug
[x] /swanAPI/debug/replaceSwanCore',            debug
[x] /swanAPI/debug/setDebugConfig',             debug
[x] /swanAPI/debug/replaceDependency',          debug
[x] /swanAPI/debug/replaceDynamicLib',          debug
[x] /swanAPI/debug/downloadExtension',          debug
[x] /swanAPI/debug/getDebugConfig',             debug
[x] /swanAPI/getLaunchAppInfo',                 base app
[x] /swanAPI/launchCloudGame',                  base app
[x] /swanAPI/menu',                             ui menu
[x] /swanAPI/getPhoneNumberByLogin',            open-api user-info
[x] /swanAPI/thirdPartyLogin',                  ext
[x] /swanAPI/getRealNameInfo',                  open-api user-info
[x] /swanAPI/getStoken',                        open-api user-info
[x] /swanAPI/getBDUSS',                         open-api user-info
[x] /swanAPI/faceResultVerify',                 ai vision
[x] /swanAPI/canvas/drawCanvas',                canvas
[x] /swanAPI/canvas/remove',                    canvas
[x] /swanAPI/canvas/insert',                    canvas
[x] /swanAPI/canvas/update',                    canvas
[x] /swanAPI/button',                           ui interaction
[x] /swanAPI/recommendProducts',                open-api other
[x] /swanAPI/recommendSimilarProducts',         open-api other
[x] /swanAPI/exit',                             base app
[x] /swanAPI/postPageInfo',                     ui interaction
[x] /swanAPI/cancelRequest',                    network request
[x] /swanAPI/prefetchAppData',                  base app
[x] /swanAPI/installApp',                       base app
[x] /swanAPI/addComponentToFullScreenSync',     ui window
[x] /swanAPI/setFullscreenOrientationSync',     ui window
[x] /swanAPI/removeComponentFromFullScreenSync', ui window
[x] /swanAPI/updateInput',                       ui keyboard
[x] /swanAPI/openInput',                         ui keyboard
[x] /swanAPI/closeInput',                        ui keyboard
[x] /swanAPI/debugGameCore',                    debug
[x] /swanAPI/openApp4Ad',                       ad
[x] /swanAPI/openApp',                          base app
[x] /swanAPI/getSlaveIdSync',                   other
[x] /swanAPI/openStatisticFlowJar',             report
[x] /swanAPI/openStatisticEvent',               report
[x] /swanAPI/postMessage',                      other
[x] /swanAPI/preloadSubPackage',                base app
[x] /swanAPI/pageTransition',                   ui interaction
[x] /swanAPI/performancePanel',                 debug
[x] /swanAPI/preloadSwanCore',                  debug
[x] /swanAPI/preventPullDownRefresh',           ui pulldown refresh
[x] /swanAPI/abTestConfig',                     debug
[x] /swanAPI/confirmSwanClose',                 debug
[x] /swanAPI/getLocalImgData',                  media image
[x] /swanAPI/getAppInfoSync',                   base app
[x] /swanAPI/getFormId',                        ui node-info
[x] /swanAPI/animView',                         ui animation
[x] /swanAPI/insertWebView',                    ui webview
[x] /swanAPI/updateWebView',                    ui webview
[x] /swanAPI/removeWebView',                    ui webview
[x] /swanAPI/webviewPostMessage',               ui webview
[x] /swanAPI/quickPay',                         open-api payment
[x] /swanAPI/updateTextarea',                   ui interaction
[x] /swanAPI/openTextarea',                     ui interaction
[x] /swanAPI/getScreenshot',                    base system
[x] /swanAPI/closeTextarea',                    ui interaction
[x] /swanAPI/community/openReplyEditor',        ui interaction
[x] /swanAPI/community/closeReplyEditor',       ui interaction
[x] /swanAPI/addFavor',                         open-api other
[x] /swanAPI/deleteFavor',                      open-api other
[x] /swanAPI/isFavor',                          open-api other
[x] /swanAPI/topFavor',                         open-api other
[x] /swanAPI/hideOpenAppGuide',                 base app
[x] /swanAPI/showOpenAppGuide',                 base app
[x] /swanAPI/getCommonSysInfo',                 base system
[x] /swanAPI/getUserInfo',                      open-api user-info
[x] /swanAPI/login',                            open-api login
[x] /swanAPI/multiAuthorize',                   open-api authorize
[x] /swanAPI/getPhoneNumber',                   open-api user-info
[x] /swanAPI/debugGameExtensionCore',           debug
[x] /swanAPI/debug/replaceGameCore',            debug
[x] /swanAPI/debug/setReplaceGameCoreConfig',   debug
[x] /swanAPI/debug/dashboardConnect',           debug
[x] /swanAPI/getRegionData',                    open-api other
[x] /swanAPI/getAutoRotationSync',              device other
[x] /swanAPI/debugGameSconsole',                debug
[x] /swanAPI/startMediaVolumeListen',           device other
[x] /swanAPI/stopMediaVolumeListen',           device other
[x] /swanAPI/vrvideo',                         media video
[x] /swanAPI/setPhoneContact',                 device contacts
[x] /swanAPI/getPhoneContacts',                device contacts
[x] /swanAPI/checkAppInstalled',               base system
[x] /swanAPI/ubcFlowJar',                      other
[x] /swanAPI/getHistory',                      other
[x] /swanAPI/deleteHistory',                   other
}
% baidu hidden category result:
\ignore{
  other: 8,
  'cloud other': 1,
  'ai other': 1,
  'open-api user-info': 9,
  'open-api other': 11,
  'media camera': 9,
  ad: 5,
  'device other': 5,
  'ui interaction': 10,
  debug: 29,
  'base app': 11,
  'ui window': 9,
  'ai vision': 2,
  'ui menu': 1,
  ext: 1,
  canvas: 4,
  'network request': 1,
  'ui keyboard': 3,
  report: 2,
  'ui pulldown refresh': 1,
  'media image': 1,
  'ui node-info': 1,
  'ui animation': 1,
  'open-api payment': 1,
  'base system': 3,
  'open-api login': 1,
  'open-api authorize': 1,
  'media video': 1,
  'device contacts': 2
}

% following is WeChat data
\ignore{
[x]  'addNativeDownloadTask',                     network download
[x]  'getABTestConfig',                           base app
[x]  'launchApplication',                         base app
[x]  'makeVoIPCall',                              device phone
[x]  'private_onWebPageUrlExposed',               ui other
[x]  'openADCanvas',                              canvas
[x]  'resumeDownloadTask',                        network download
[x]  'writeCommData',                             other
[x]  'addPhoneCalendar',                          open-api phone
[x]  'WEB_INVOKE_APPSERVICE',                     other
[x]  'onWebviewFinishLoad',                       ui webview
[x]  'onWebviewStartLoad',                        ui webview
[x]  'onWebviewError',                            ui webview
[x]  'insertHTMLWebView',                        ui webview
[x]  'updateHTMLWebView',  ui webview
[x]  'updateXWebCanvas', ui webview
[x]  'addDownloadTask',    network download
[x]  'addDownloadTaskForNative', network download
[x]  'addDownloadTaskStraight', network download
[x]  'cancelDownloadTask', network download
[x]  'cancelDownloadTaskForNative', network download
[x]  'getInstallState', base app
[x]  'getInstallStateForNative', base app
[x]  'installDownloadTask',  network download
[x]  'installDownloadTaskForNative', network download
[x]  'jumpDownloaderWidgetForNative', network download
[x]  'launchApplicationForNative', base app
[x]  'pauseDownloadTask', network download
[x]  'pauseDownloadTaskForNative', network download
[x]  'queryDownloadTask', network download
[x]  'queryDownloadTaskForNative', network download
[x]  'resumeDownloadTaskForNative', network download
[x]  'onDownloadAppStateChangeForNative', network download
[x]  'getDownloadWidgetTaskInfoForNative', network download
[x]  'bindGroup', open-api account-info
[x]  'joinGroup', open-api account-info 
[x]  'getMusicPlayerState', media audio
[x]  'openRealnameAuth', open-api authorize
[x]  'requestAuthUserAutoFillData',  open-api authorize
[x]  'canvasToTempFilePathSync', canvas
[x]  'chooseShareGroup', open-api share
[x]  'setBackgroundFetchToken', other
[x]  'triggerBackgroundFetch', other
[x]  'getBackgroundFetchToken', other
[x]  'getAppConfig',  base app
[x]  'getOAID', open-api account-info 
[x]  'checkIsSupportFacialRecognition', open-api soter
[x]  'faceVerifyForPay', open-api payment
[x]  'handleMPChannelAction', other
[x]  'openWebViewUseFastLoad', ui webview
[x]  'onUpdateChannelFeeds', other
[x]  'getRandomValues', other
[x]  'jumpRedPacketEnvelopeList', open-api payment
[x]  'jumpRedPacketEnvelopePreview', open-api payment
[x]  'requestQueryCashier', open-api payment
[x]  'requestOfflineUserBindQuery', other
[x]  'opNativeRedDot', other
[x]  'openAddress', open-api address
[x]  'openWCCardHomePage', open-api other
[x]  'openWCCertHomePage', open-api other
[x]  'openDeliveryList', open-api other
[x]  'openLink', base other
[x]  'openOfflinePayView', open-api payment
[x]  'openUrl', base other
[x]  'openWCExDeviceList', open-api other
[x]  'openWCPayLQTDepositPlan',  open-api payment
[x]  'openWCPayLQTDepositPlanAdd', open-api payment
[x]  'openWCPayLQTDetail', open-api payment
[x]  'openWCPayLQTSave', open-api payment
[x]  'phoneBindCardVerifySms', open-api authorize
[x]  'predownloadMiniProgramPackage', base app
[x]  'private_openUrl', base other
[x]  'chooseWeChatContact', device contacts
[x]  'searchContacts', device contacts
[x]  'reportSubmitForm', other
[x]  'restart', base basic
[x]  'saveWaid', other
[x]  'systemLog', base debug
[x]  'uploadToCommonCDN', network upload
[x]  'removeSplashScreenshot', device screen
[x]  'saveSplashScreenshot', device screen
[x]  'private_fileSystemConvert', storage
[x]  'declareOriginalFinished', other
[x]  'deleteFinderDataItem', other
[x]  'endorsementFinished', other
[x]  'postFinderDataItem', other
[x]  'resendProfileFeed', other
[x]  'kvReport', open-api data-analysis
[x]  'openFinderProfile', other
[x]  'onH5Data', other
[x]  'sendDataToH5', other
[x]  'openRedPacket', open-api payment
[x]  'sendRedPacket', open-api payment
[x]  'getLabInfo', open-api other
[x]  'setLabInfo', open-api other
[x]  'onReceiveMsgChannel', other
[x]  'previewMedia', media other
[x]  'isSupportNFC', device nfc
[x]  'onNFCDiscovered', device nfc
[x]  'isNFCTechConnected', device nfc
[x]  'NFCGetMaxTransceiveLength', device nfc
[x]  'NFCSetTimeout', device nfc
[x]  'NFCTransceive', device nfc
[x]  'startNFCDiscovery', device nfc
[x]  'stopNFCDiscovery', device nfc
[x]  'writeNdefMessage', device nfc
[x]  'secureTunnel', other
[x]  'loadPaySpeechDialectConfig', open-api payment
[x]  'setCurrentPaySpeech', open-api payment
[x]  'onStartReportPageData',  open-api data-analysis
[x]  'exitVoIPChat', device phone
[x]  'setStatusBarStyle', ui other
[x]  'setMenuStyle', ui menu
[x]  'bindPaymentCard', open-api payment
[x]  'getWCPayOverseaPrepayRequest', open-api payment
[x]  'handleWCPayOverseaWalletBuffer', open-api payment
[x]  'openSelectPayment', open-api payment
[x]  'openWCPayOverseaPaymentReceive', open-api payment
[x]  'requestBizSplitBillPayment', open-api payment
[x]  'requestEntrustAuthorization', open-api authorize
[x]  'requestH5Transaction', open-api payment
[x]  'requestPaymentToBank', open-api payment
[x]  'requestVerifyUserIdentity', open-api authorize
[x]  'requestVirtualPayment', open-api payment
[x]  'sendBizRedPacket', open-api payment
[x]  'verifyPaymentPassword', open-api payment
[x]  'openQRCode', device scan
[x]  'showUpdatableMessageSubscribeButton', open-api subscribe
[x]  'showVirtualBottomNavigationBar', ui other
[x]  'openWeAppHistoryList', open-api other
[x]  'openWeAppStarList', open-api other
[x]  'reportAction', open-api data-analysis
[x]  'reportIDKey', open-api data-analysis
[x]  'checkIsOpenAccessibility', device other
[x]  'getVolume', device other
[x]  'setVolume', device other
[x]  'launchApplicationDirectly', base app
[x]  'onDownloadAppStateChange', network download
[x]  'startCustomFacialRecognitionVerify',  open-api soter
[x]  'startCustomFacialRecognitionVerifyAndUploadVideo', open-api soter
[x]  'startFacialRecognitionVerify', open-api soter
[x]  'startFacialRecognitionVerifyAndUploadVideo', open-api soter
[x]  'openAddressWithLightMode', open-api address
[x]  'openMapApp', base app
[x]  'NFCClose', device nfc
[x]  'NFCConnect', device nfc
[x]  'NFCGetAtqa', device nfc
[x]  'NFCGetHistoricalBytes', device nfc
[x]  'NFCGetSak', device nfc
[x]  'requestJointPayment', open-api payment
[x]  'requestMallPayment', open-api payment
[x]  'uploadWeRunData', open-api werun
[x]  'onXWebCastingInterrupt',  ui webview
[x]  'onXWebCastingUserSelect', ui webview
[x]  'onXWebVideoEnded', ui webview
[x]  'onXWebVideoPause', ui webview
[x]  'onXWebVideoPlay', ui webview
[x]  'onXWebVideoProgress', ui webview
[x]  'onXWebVideoTimeUpdate', ui webview
[x]  'onXWebVideoWaiting', ui webview
[x]  'onXWebDLNACastingStateChange', ui webview
[x]  'removeXWebWebGLCanvas', canvas
[x]  'updateXWebWebGLCanvas', canvas
[x]  'editTextWithPopForm', other
[x]  'onBLEPeripheralConnectionStateChanged', device bluetooth-ble
[x]  'onCharacteristicReadRequest', other
[x]  'onCharacteristicWriteRequest', other
[x]  'openChannelsActivity', open-api other
[x]  'openChannelsLive', open-api other
[x]  'openChannelsUserProfile', open-api other
[x]  'fetchSendingAndFailProfileFeed', open-api other
[x]  'getFinderAccount', open-api other
[x]  'onFeedPostCallback', open-api other
[x]  'fetchFinderProfileFeed', open-api other
[x]  'modifyFinderAccountAvatar', open-api other
[x]  'modifyFinderAccountNickname', open-api other
[x]  'openFinderPostPicker', open-api other
[x]  'shareFinderEndorsementToFriend', open-api other
[x]  'setPageOrientation', ui other
[x]  'private_setNavigationBarRightButton', ui navigation-bar
[x]  'getRecentUsageList', other
[x]  'onGetRecentUsageListResult', other
[x]  'onRealtimeDataResponse', other
[x]  'onXWebLivePlayerOrientationChanged', ui webview
[x]  'onXWebVideoOrientationChanged', ui webview
[x]  'addWeRunData', open-api werun
[x]  'insertXWebWebGLCanvas', canvas
[x]  'getAppContact', open-api account-info
[x]  'getPublicLibVersion', base app
[x]  'loadWAFile', base app
[x]  'loadWAFileSync', base app
[x]  'onLocalServiceEvent', other
[x]  'operateLocalServicesScan', other
[x]  'getRegionData', open-api other
[x]  'getBackgroundFetchData', open-api other
[x]  'operateRealtimeData', open-api other
[x]  'reportKeyValue', open-api data-analysis
[x]  'xwebCanvasToTempFilePath', canvas
[x]  'enableLocationUpdate', location
[x]  'openVideoEditor', media video
[x]  'operateMediaContainer', media other
[x]  'operateMediaTrack', media other
[x]  'onLongPress', device other
[x]  'onTouchCancel', device screen
[x]  'onTouchStart', device screen
[x]  'onTouchMove', device screen
[x]  'onTouchEnd', device screen
[x]  'updateXWebVoIPView', device phone
[x]  'insertXWebVoIPView', device phone
[x]  'removeXWebVoIPView', device phone
[x]  'insertXWebCamera', device phone
[x]  'removeXWebCamera', device phone
[x]  'updateXWebCamera', device phone
[x]  'onSkiaCanvasLongPress', canvas
[x]  'onSkiaCanvasTouchEnd', canvas
[x]  'insertXWebCanvas', canvas
[x]  'onXWebCanvasSurfaceChange', canvas
[x]  'removeXWebCanvas', canvas
[x]  'insertXWebLivePlayer', media live
[x]  'operateXWebLivePlayer', media live
[x]  'removeXWebLivePlayer', media live
[x]  'updateXWebLivePlayer', media live
[x]  'onXWebLivePlayerAudioVolume', media live
[x]  'onXWebLivePlayerBackgroundPlaybackChange', media live
[x]  'onXWebLivePlayerEvent', media live
[x]  'onXWebLivePlayerNetStatus', media live
[x]  'insertXWebLivePusher', media live 
[x]  'operateXWebLivePusher', media live
[x]  'removeXWebLivePusher', media live
[x]  'updateXWebLivePusher', media live
[x]  'onXWebLivePusherAudioVolume', media live
[x]  'onXWebLivePusherBGMComplete',  media live
[x]  'onXWebLivePusherBGMProgress', media live
[x]  'onXWebLivePusherBGMStart', media live
[x]  'onXWebLivePusherError', media live
[x]  'onXWebLivePusherEvent', media live
[x]  'onXWebLivePusherNetStatus', media live
[x]  'insertXWebMap', media map
[x]  'removeXWebMap', media map
[x]  'updateXWebMap', media map
[x]  'insertXWebVideo', media video
[x]  'operateXWebVideo', media video
[x]  'removeXWebVideo', media video
[x]  'updateXWebVideo', media video
[x]  'onXWebVideoBackgroundPlaybackChange', media video
[x]  'onXWebVideoError', media video
[x]  'onXWebVideoLoadedMetaData', media video 
[x]  'onXWebVideoPreloadedMetaData', media video
[x]  'onXWebVideoSeekComplete', media video
[x]  'onContactUpdate', device contacts
[x]  'onAudioStateChange', media audio
[x]  'onTextViewLinkClick', ui interaction
[x]  'onUpdateWXConfig', base app
[x]  'onCameraInitDone', media camera
[x]  'onCameraNeedAuthCancel', media camera
[x]  'onCameraScanCode', media camera
[x]  'onCameraStop', media camera
[x]  'onCameraVideoTaken', media camera
[x]  'onImagePreviewerLoadFail', media image
[x]  'onImageViewLoad', media image
[x]  'onImageViewClick', media image
[x]  'onTextViewClick', ui interaction 
[x]  'onTextViewDrag', ui interaction
[x]  'onScrollViewScroll', ui interaction
[x]  'onBeaconServiceChanged', device iBeacon
[x]  'onBeaconUpdated', device iBeacon
[x]  'onLocationChangeError', location
[x]  'enableLocationUpdateBackground', location
[x]  'onMapControlClick', media map
[x]  'onMapMarkerClusterClick', media map
[x]  'onMapMarkerClusterCreate', media map
[x]  'onMapAnchorPointClick', media map
[x]  'onMapCalloutClick', media map
[x]  'onMapClick', media map
[x]  'onMapIndoorChange', media map
[x]  'onMapLabelClick', media map
[x]  'onMapMarkerClick', media map
[x]  'onMapPoiClick', media map
[x]  'onMapRegionChange', media map
[x]  'onLivePlayerAudioVolume', media live
[x]  'onLivePlayerFullScreenChange', media live
[x]  'onLivePlayerNetStatus', media live
[x]  'onLivePlayerEvent', media live
[x]  'onLivePusherAudioVolume', media live
[x]  'onLivePusherBGMComplete', media live
[x]  'onLivePusherBGMProgress', media live
[x]  'onLivePusherBGMStart', media live
[x]  'onLivePusherError', media live
[x]  'onLivePusherNetStatus', media live
[x]  'onLivePusherEvent', media live
[x]  'onDownloadTaskStateChange', network download
[x]  'onRequestTaskStateChange', network request
[x]  'onUploadTaskStateChange', network upload
[x]  'onSocketTaskStateChange', network websocket
[x]  'onMultiPickerViewChange', ui other
[x]  'onVideoCanPlay', media video
[x]  'onVideoClickDanmuBtn', media video
[x]  'onVideoEnded', media video
[x]  'onVideoError', media video
[x]  'onVideoFullScreenChange', media video
[x]  'onVideoLoadedMetaData',  media video
[x]  'onVideoPause', media video
[x]  'onVideoPlay', media video
[x]  'onVideoProgress', media video
[x]  'onVideoResourceError', media video
[x]  'onVideoResourceLoad', media video
[x]  'onVideoTimeUpdate', media video
[x]  'onVideoWaiting', media video 
[x]  'onDeviceOrientationChange', device other
[x]  'addToFavorites', open-api other
[x]  'navigateBackApplication', open-api miniprogram-navigate
[x]  'openWeRunSetting', open-api werun
[x]  'private_addContact', device contact
[x]  'refreshSession', other
[x]  'showImageOperateSheet', media image
[x]  'onViewDidResize', ui other
[x]  'updateApp', base update
[x]  'onUpdateStatusChange', base update
[x]  'operateXWebLivePlayerBackground', ui webview
[x]  'operateXWebVideoBackground', ui webview
[x]  'adDataReport', open-api data-analysis
[x]  'addFileToFavorites', open-api 
[x]  'addImageToFavorites', open-api other
[x]  'addVideoToFavorites', open-api other
[x]  'batchGetContact', device contact
[x]  'getBackgroundAudioState', media audio
[x]  'onMusicEnd', media audio
[x]  'onMusicPause', media audio
[x]  'onMusicPlay', media audio
[x]  'operateMusicPlayer', media audio
[x]  'createAudioInstance', media audio
[x]  'createAudioInstanceAsync', media audio
[x]  'destroyAudioInstance', media audio
[x]  'getAudioState', media audio
[x]  'operateAudio', media audio
[x]  'onRecorderStateChange', media recorder
[x]  'operateRecorder', media recorder
[x]  'setAudioState', media recorder
[x]  'createVestUser', open-api user-info
[x]  'deleteUserAutoFillData', open-api user-info
[x]  'getPhoneNumber', open-api user-info
[x]  'getUserAutoFillData', open-api user-info
[x]  'setUserAutoFillData', open-api user-info
[x]  'batchPreloadMiniProgram', base app
[x]  'captureScreen', device screen
[x]  'functionalPageStartGame', other
[x]  'getPermissionBytes', base other
[x]  'getPluginPermissionBytes', base other
[x]  'getBLEDeviceRSSI', device bluetooth-ble
[x]  'makeBluetoothPair', device bluetooth
[x]  'notifyBLECharacteristicValueChanged', device bluetooth-ble
[x]  'setBLEMTU', device bluetooth-ble
[x]  'addBLEPeripheralService', device bluetooth-ble
[x]  'closeBLEPeripheralServer', device bluetooth-ble
[x]  'createBLEPeripheralServer', device bluetooth-ble
[x]  'removeBLEPeripheralService', device bluetooth-ble
[x]  'startBLEPeripheralAdvertising', device bluetooth-ble
[x]  'stopBLEPeripheralAdvertising', device bluetooth-ble
[x]  'writeBLEPeripheralCharacteristicValue', device bluetooth-ble
[x]  'markScene', other
[x]  'operateCamera', media camera
[x]  'openChannelsCreateContact', other
[x]  'openChannelsPostPage', other
[x]  'pageNotFoundCallback', ui other
[x]  'chooseContact', device contact
[x]  'enterContact', device contact
[x]  'privateEnterContact', device contact
[x]  'measureTextString', other
[x]  'returnCopyUrl', other
[x]  'sendRedCoverAppMsg', open-api other
[x]  'traceEvent', base debug
[x]  'updatePerfData', open-api performance
[x]  'verifyPlugin', base app
[x]  'preloadMiniProgramEnv', base app
[x]  'faceDetect', open-api soter
[x]  'faceProcessInit', open-api soter
[x]  'faceProcessStop', open-api soter
[x]  'checkHandoffEnabled', other
[x]  'startHandoff', other
[x]  'hideSplashScreenshot', ui other
[x]  'navigateBackH5', open-api miniprogram-navigate
[x]  'loadJsFiles', file
[x]  'createFinderAccount', open-api other
[x]  'hideKeyboard', ui keyboard
[x]  'onTextAreaHeightChange', ui other
[x]  'removeTextArea', ui other
[x]  'restoreWebviewFocus', ui webview
[x]  'setKeyboardValue', ui keyboard
[x]  'onKeyboardValueChange', ui keyboard
[x]  'disableLocationUpdate', location
[x]  'onLoadSubPackageTaskStateChange', base app
[x]  'chooseMultiMedia', media other
[x]  'onUploadEncryptedFileToCDNProgress', network upload
[x]  'uploadEncryptedFileToCDN', network upload
[x]  'compressVideo', media video
[x]  'getVideoInfo', media video
[x]  'launchMiniProgram', base app
[x]  'requestSubscribeMessage', open-api subscribe
[x]  'navigateBackNative', open-api miniprogram-navigate
[x]  'operateDownloadTask', network download
[x]  'operateRequestTask', network request
[x]  'operateUploadTask', network  upload
[x]  'checkNetworkAPIURL', network other
[x]  'operateSocketTask', network socket
[x]  'reportPageData', open-api data-analysis
[x]  'onVoIPChatInterrupted', device phone
[x]  'onVoIPChatMembersChanged', device phone
[x]  'onVoIPChatSpeakersChanged', device phone
[x]  'onVoIPVideoMembersChanged',  device phone
[x]  'onNavigateBackIntercept', ui interaction
[x]  'setNavigationBarRightButton', navigation-bar
[x]  'showNavigationBar', ui navigation-bar
[x]  'hideHomeButton', ui other
[x]  'hideNavigationBar', ui navigation-bar
[x]  'initReady', other
[x]  'initReadyAfterRenderingCache', other
[x]  'initReadyForPrerender', other
[x]  'preloadWebview', ui webview
[x]  'rewriteRoute', route
[x]  'scrollWebviewTo', ui scroll
[x]  'setNavigateBackConfirmDialog', ui interaction
[x]  'setNavigateBackInterception', ui interaction
[x]  'requestFacetoFacePayment', open-api payment
[x]  'requestPersonalPay', open-api payment
[x]  'openBizProfile', open-api enterprise
[x]  'openUserProfile', open-api user-info
[x]  'profile', other
[x]  'noticePerformanceMetrics', device performance
[x]  'operateRecentUsageList', other
[x]  'scanItem', device scan
[x]  'hideShareTimelineMenu', open-api share
[x]  'shareTimeline', open-api share
[x]  'showShareMenuWithShareTicket', ui other
[x]  'showShareTimelineMenu', ui other
[x]  'updateShareMenuDynamic', ui other
[x]  'updateShareMenuShareTicket', ui other
[x]  'updateShareMenuToDo', ui other
[x]  'updateShareMenuUpdatable', ui other
[x]  'onCopyUrl', other
[x]  'hideVirtualBottomNavigationBar', ui navigation-bar
[x]  'openWeAppSearch', open-api other
[x]  'openWeAppProfile', open-api other
[x]  'onInitialRenderingCacheReady', other
[x]  'saveInitialRenderingCache', other
[x]  'onMemoryWarningReceive', device performance
[x]  'loadVideoResource', media video
[x]  'reportRealtimeAction', open-api data-analysis
[x]  'enableAccelerometer', device accelerometer
[x]  'enableCompass', device compass
[x]  'enableDeviceMotionChangeListening', device motion
[x]  'enableDeviceOrientationChangeListening', device other
[x]  'enableGyroscope', device gyroscope
[x]  'getSystemInfoAsync', base system
[x]  'onEnterLivePlayerPictureInPicture', ui other
[x]  'onLeaveLivePlayerPictureInPicture', ui other
[x]  'onEnterVideoPictureInPicture', ui other
[x]  'onLeaveVideoPictureInPicture', ui other
[x]  'operateWXData', open-api other
[x]  'adOperateWXData', ad
[x]  'private_quicklyAddBrandContact', device contact
[x]  'openBusinessView', ui other
[x]  'showKeyboard', ui keyboard
[x]  'updateInput', ui keyboard
[x]  'removeMapMarkers', media map
[x]  'setMapCenterOffset', media map
[x]  'setMapIndoorFloor', media map
[x]  'setMapIndoorMaskColor', media map
[x]  'setMapLocMarkerIcon', media map 
[x]  'toScreenLocation', media map
[x]  'translateMapMarker', media map
[x]  'updateMapGroundOverlay', media map
[x]  'updateMapMarkers', media map
[x]  'addMapCircles', media map
[x]  'addMapControls', media map
[x]  'addMapCustomLayer', media map
[x]  'addMapGroundOverlay', media map
[x]  'addMapLines', media map
[x]  'addMapMarkers', media map
[x]  'addMapPolygons', media map
[x]  'eraseMapLines', media map
[x]  'fromScreenLocation', media map
[x]  'getMapCenterLocation', media map
[x]  'getMapIndoorFloor', media map
[x]  'getMapRegion', media map
[x]  'getMapRotate', media map
[x]  'getMapScale', media map
[x]  'getMapSkew', media map
[x]  'includeMapPoints', media map
[x]  'initMapMarkerCluster', media map
[x]  'moveMapMarkerAlong', media map
[x]  'moveToMapLocation', media map
[x]  'removeMapGroundOverlay', media map
[x]  'removeMapCustomLayer', media map
[x]  'removeMapLines', media map
[x]  'createLoadSubPackageTask', base app
[x]  'navigateToDevMiniProgram', open-api miniprogram-navigate
[x]  'launchDevMiniProgram', base app
[x]  'createDownloadTask', network download
[x]  'createDownloadTaskAsync', network download 
[x]  'createRequestTask', network request
[x]  'createRequestTaskAsync', network request
[x]  'createUploadTask', network upload
[x]  'createUploadTaskAsync', network upload
[x]  'createSocketTask', network socket
[x]  'joinVoIPChat', device phone
[x]  'updateVoIPChatMuteConfig', device phone
[x]  'hasJoinVoIPChat', device phone
[x]  'operateCallTone', device phone
[x]  'subscribeVoIPMembers', device phone
[x]  'setDisplayOrientation', ui other
[x]  'private_setPageOrientation', ui other
[x]  'disableScrollBounce', ui scroll
[x]  'showDatePickerView', ui other
[x]  'showMultiPickerView', ui other
[x]  'showPickerView', ui other
[x]  'updateMultiPickerView', ui other
[x]  'shareAppMessage', open-api share
[x]  'shareAppMessageDirectly', open-api share
[x]  'shareAppMessageForFakeNative', open-api share
[x]  'getGlobalStorage', storage
[x]  'getGlobalStorageInfo', storage
[x]  'removeGlobalStorage', storage
[x]  'setGlobalStorage', storage
[x]  'removeHTMLWebView', ui webview
[x]  'drawCanvas', canvas
[x]  'insertCanvas', canvas
[x]  'insertWebGLCanvas', canvas
[x]  'removeCanvas', canvas
[x]  'removeWebGLCanvas', canvas
[x]  'updateCanvas', canvas
[x]  'updateWebGLCanvas', canvas
[x]  'insertCamera', canvas
[x]  'removeCamera', canvas
[x]  'updateCamera', canvas
[x]  'insertPositioningContainer', ui other
[x]  'removePositioningContainer', ui other
[x]  'updatePositioningContainer', ui other
[x]  'animateCoverView', ui other
[x]  'insertImagePreviewer', ui other
[x]  'insertImageView', ui other
[x]  'insertScrollView', ui other
[x]  'insertTextView', ui other
[x]  'removeImagePreviewer', ui other
[x]  'removeImageView', ui other
[x]  'removeScrollView', ui other
[x]  'removeTextView', ui other
[x]  'updateImagePreviewer', ui other
[x]  'updateImageView', ui other
[x]  'updateScrollView', ui other
[x]  'updateTextView', ui other
[x]  'insertTextArea', ui other
[x]  'updateTextArea', ui other
[x]  'updateMap', media map
[x]  'insertMap', media map
[x]  'removeMap', media map
[x]  'insertVoIPView', device phone
[x]  'removeVoIPView', device phone
[x]  'updateVoIPView', device phone
[x]  'join1v1VoIPChat', device phone
[x]  'shareAppMessageToSpecificContactDirectly', open-api share
[x]  'shareAppMessageToSpecificContactForFakeNativeDirectly', open-api share
[x]  'checkTrafficCardConditions', open-api other
[x]  'deleteTrafficCard', open-api other
[x]  'issueTrafficCard', open-api other
[x]  'queryTrafficCardInfo', open-api other
[x]  'rechargeTrafficCard', open-api other
[x]  'setDefaultTrafficCard', open-api other
}

% result of WeChat, total: 567
\ignore{
'network download': 22,
'base app': 20,
'device phone': 21,
'ui other': 46,
canvas: 21,
other: 47,
'open-api phone': 1,
'ui webview': 23,
'open-api account-info': 4,
'media audio': 12,
'open-api authorize': 5,
'open-api share': 8,
'open-api soter': 8,
'open-api payment': 28,
'open-api address': 2,
'open-api other': 36,
'base other': 5,
'device contacts': 3,
'base basic': 1,
'base debug': 2,
'network upload': 6,
'device screen': 7,
storage: 5,
'open-api data-analysis': 8,
'media other': 4,
'device nfc': 14,
'ui menu': 1,
'device scan': 2,
'open-api subscribe': 2,
'device other': 6,
'open-api werun': 3,
'device bluetooth-ble': 11,
'ui navigation-bar': 4,
location: 4,
'media video': 26,
'media live': 30,
'media map': 48,
'ui interaction': 7,
'media camera': 6,
'media image': 4,
'device iBeacon': 2,
'network request': 4,
'network websocket': 1,
'open-api miniprogram-navigate': 4,
'device contact': 6,
'base update': 2,
'open-api': 1,
'media recorder': 3,
'open-api user-info': 6,
'device bluetooth': 1,
'open-api performance': 1,
file: 1,
'ui keyboard': 5,
'network  upload': 1,
'network other': 1,
'network socket': 2,
'navigation-bar': 1,
route: 1,
'ui scroll': 2,
'open-api enterprise': 1,
'device performance': 2,
'device accelerometer': 1,
'device compass': 1,
'device motion': 1,
'device gyroscope': 1,
'base system': 1,
ad: 1
}

% following is wecom data
\ignore{
[x] sdk_navigateToMiniProgram, open-api miniprogram-navigation
[x] onAddToFavorites, open-api other
[x] onBackgroundAudioNext, media audio
[x] onBackgroundAudioPrev, media audio
[x] onBackgroundAudioStateChange, media audio
[x] onBLEConnectionStateChanged, device bluetooth-ble
[x] onCameraOutput, media camera
[x] operateBackgroundAudio, media audio
[x] setBackgroundAudioState, media audio
[x] qy__navigateBackNative, open-api miniprogram-navigation
[x] onCheckAppShareMessageEnable, open-api share
[x] onForwardAppMessage, open-api other
[x] loadLibFiles, base app
[x] onKeyboardComplete, ui keyboard
[x] onKeyboardConfirm, ui keyboard
[x] onKeyboardShow, ui keyboard
[x] exitMiniProgram, base app
[x] onUserOpStatistic, open-api data-analysis
[x] getCurrentRoute, route
[x] onNetworkWeakChange, network other
[x] onTapNavigationBarRightButton, ui navigation-bar
[x] qy__applyCodeForRestrictedChat, open-api enterprise
[x] qy__bioassayAuthentication, open-api soter
[x] qy__checkAppShareMessageEnable, open-api share
[x] qy__chooseAttach, file
[x] qy__chooseFile, file
[x] qy__chooseInvoice, open-api invoice
[x] qy__chooseWxworkContact, open-api enterprise
[x] qy__selectConvAndAction, open-api enterprise
[x] qy__chooseWxworkVisibleRange, open-api enterprise
[x] qy__getContext, base other
[x] qy__getMacAddress, device other
[x] qy__idcardVerify, open-api other 
[x] qy__bioassayFaceCompare, open-api soter
[x] qy__openChatWithMsg, open-api enterprise
[x] qy__openWechatWebviewUrl, ui webview
[x] qy__openWebview, ui webview
[x] qy__postNotification, base system
[x] qy__requestPayment, open-api payment
[x] qy__openWechatMiniProgram, open-api miniprogram-navigate
[x] qy__sendMessageToConv, open-api enterprise
[x] qy__sendMessageToWX, open-api other
[x] qy__shareAppMessageEx, open-api share
[x] qy__shareToExternalChat, open-api share
[x] qy__shareToExternalContact, open-api share
[x] qy__shareToTrainee, open-api share
[x] qy__shareToTraineeChat, open-api share
[x] qy__startWecast, open-api other
[x] qy__translateVoice, voice-recognition
[x] qy__wwLog, other
[x] qy__wwlogicInternal, other
[x] qy__wwOpenUrlScheme, other
[x] qy__showUserProfile, open-api user-info
[x] qy__enableShareToWxMenuGlobal, open-api share
[x] qy__openDeviceProfile, device other
[x] qy__enterHWOpenTalk, open-api other
[x] qy__queryCurrHWOpenTalk, open-api other
[x] qy__canIUsePrivate, open-api login
[x] qy__operatePrivate, open-api other
[x] qy__updateEnterpriseChat, open-api enterprise
[x] qy__chooseMessageFile, open-api enterprise
[x] qy__claimClassAdmin, open-api other
[x] qy__createCorpGroupChat, open-api enterprise
[x] qy__createSchoolPayment, open-api payment
[x] qy__getAvatar, open-api user-info
[x] qy__getCurExternalContact, open-api enterprise
[x] qy__getEmail, open-api user-info
[x] qy__getEnterpriseUserInfo, open-api enterprise
[x] qy__getMobile, open-api user-info
[x] qy__getQrCode, open-api enterprise
[x] qy__getShareInfo, open-api share
[x] qy__hideChatAttachmentMenu, ui menu
[x] qy__navigateToAddCustomer, open-api enterprise
[x] qy__navigateToKfChat, open-api enterprise
[x] qy__openEnterpriseContact, open-api enterprise
[x] qy__openExistChat, open-api enterprise
[x] qy__openThirdAppServiceChat, open-api enterprise
[x] qy__openUrl, open-api other
[x] qy__openUserProfile, open-api user-info
[x] qy__replayLiving, media live
[x] qy__selectPrivilegedContact, device contact
[x] qy__sendChatMessage, open-api enterprise
[x] qy__setShareAttr, open-api share
[x] qy__shareAppMessageToAdmin, open-api share
[x] qy__shareToExternalMoments, open-api share
[x] qy__startLiving, media live
[x] qy__startMeeting, open-api enterprise
[x] qy__updateCorpGroupChat, open-api enterprise
[x] qy__updateMomentsSetting,  open-api enterprise
[x] qy__downloadMedia, network download
[x] qy__uploadMedia, network upload
[x] qy__selectCorpGroupContact, open-api enterprise
[x] qy__discoverDevice, device other
[x] insertLivePlayer, media live
[x] insertLivePusher,  media live
[x] operateLivePlayer, media live
[x] operateLivePusher, media live
[x] removeLivePlayer, media live
[x] removeLivePusher, media live
[x] updateLivePlayer, media live
[x] updateLivePusher, media live
[x] insertVideoPlayer, media video
[x] operateVideoPlayer, media video
[x] removeVideoPlayer, media video
[x] updateVideoPlayer, media video
[x] qy__getUserInfo, open-api user-info
}

% final result:
\ignore{
  'open-api miniprogram-navigation': 2,
  'open-api other': 10,
  'media audio': 5,
  'device bluetooth-ble': 1,
  'media camera': 1,
  'open-api share': 12,
  'base app': 2,
  'ui keyboard': 3,
  'open-api data-analysis': 1,
  route: 1,
  'network other': 1,
  'ui navigation-bar': 1,
  'open-api enterprise': 22,
  'open-api soter': 2,
  file: 2,
  'open-api invoice': 1,
  'base other': 1,
  'device other': 3,
  'ui webview': 2,
  'base system': 1,
  'open-api payment': 2,
  'open-api miniprogram-navigate': 1,
  'voice-recognition': 1,
  other: 3,
  'open-api user-info': 6,
  'open-api login': 1,
  'ui menu': 1,
  'media live': 10,
  'device contact': 1,
  'network download': 1,
  'network upload': 1,
  'media video': 4
}

% following is tiktok
\ignore{
operateModalWebviewState, ui webview
hostLogin, open-api misc
startMock, device misc
stopMock, device misc
showActivityAd, ad
prefetchImages, media image
getUseDuration, open-api user-info
base64ToTempFilePath, base basic
base64ToTempFilePathSync, base basic
getCloudStorageByLocation, open-api misc
operateRecorder, media recorder
createAudioInstance, media audio
operateAudio, media audio
checkFollowAwemeState, open-api misc
destroyAudioInstance, media audio
setAudioState, media audio
getAudioState, media audio
getAudioStateSync, media audio
showEncourageCard, open-api misc
getBackgroundAudioContext, media audio
startFacialRecognitionVerify, open-api bio-auth
operateBgAudio, media audio
requestPayment, open-api payment
setBgAudioState, media audio
requestWXH5Payment, open-api payment
getBgAudioState, media audio
createPreloadVideoTask, media video
operatePreloadVideoTask, media video
createRequestTask, network request
operateRequestTask, network request
createInnerRequestTask, network request
operateInnerRequestTask, network request
createDownloadTask, network download
operateDownloadTask, network download
createInnerDownloadTask, network download
operateInnerDownloadTask, network download
createUploadTask, network upload
operateUploadTask, network upload
createInnerUploadTask, network upload
operateInnerUploadTask, network upload
createSocketTask, network websocket
operateSocketTask, network websocket
openUserProfile, open-api user-info
dealUserRelation, open-api user-info
createBannerAd, ad
openCustomerService, open-api misc
updateBannerAd, ad
operateBannerAd, ad
createVideoAd, ad
joinChatGroup, open-api misc
getAwemeChatGroupInfo, open-api misc
operateVideoAd, ad
operateInterstitialAd, ad
joinAwemeConversation, open-api misc
showECommerceAd, ad
launchApp, base app
setAnalyticsConfigSync, open-api misc
checkShortcut, uncatgorized
systemLog, base system
reportTimelinePoints, open-api misc
addShortcut, uncatgorized
_webviewGetPhoneNumber, open-api user-info
reportJsRuntimeError, open-api misc
sentryReport, open-api misc
_serviceGetPhoneNumber, open-api user-info
getLocalPhoneNumber, open-api user-info
reportMetrics, open-api misc
reportAppLog, open-api misc
getLocalPhoneNumberToken, open-api user-info
onBeforeCloseReturnSync, uncatgorized
getHostLaunchQuery, uncatgorized
createFollowButton, ui interaction
getHostLaunchQuerySync, uncatgorized
operateFollowButton, ui interaction
getCloudStorageByRelation, open-api misc
getUserCloudStorage, open-api misc
setSystemVolume, device misc
setUserCloudStorage, open-api misc
removeUserCloudStorage, open-api misc
getSystemVolume, device misc
getBatteryInfoSync, device misc
getBatteryInfo, device misc
isInUserFavoritesSync, open-api user-info
addToFavorites, open-api user-info
addToUserFavorites, open-api user-info
createDxppTask, uncatgorized
getFavoritesList, open-api user-info
operateDxppTask, uncatgorized
removeFromFavorites, open-api user-info
sortFavorites, open-api user-info
getDxppTaskStatusSync, uncatgorized
getSavedFileInfo, file
shareAppMessageDirectly, share
shareVideo, share
operateInternalStorageSync, storage
setMenuButtonVisibility, ui misc
showMorePanel, ui misc
protocolPathToAbsPath, base basic
getAppInfoSync, base app
setInputValue, ui misc
getRenderEnvSync, ui misc
getGeneralInfo, base basic
hideKeyboard, ui keyboard
getPerformanceTimingSync, open-api misc
getAppbrandSettingsSync, base app
callHostMethodSync, base system
callHostMethod, base system
addHostEventListener, base system
removeHostEventListener, base system
checkAppInstall, base system
launchAppDirectly, base app
canLaunchAppSync, base app
getRecentAppList, base system
sendUmengEventV1, open-api misc
removeFromRecentAppList, base system
showErrorPage, base misc
createCanvasEnvSync, canvas
preloadMiniProgram, base app
createHeliumCameraEnvSync, device camera
enableAccelerometer, device misc
openModalWebview, ui webview
closeModalWebview, ui webview
}

\ignore{
  'ui webview': 3,
  'open-api misc': 20,
  'device misc': 7,
  ad: 8,
  'media image': 1,
  'open-api user-info': 13,
  'base basic': 4,
  'media recorder': 1,
  'media audio': 10,
  'open-api bio-auth': 1,
  'open-api payment': 2,
  'media video': 2,
  'network request': 4,
  'network download': 4,
  'network upload': 4,
  'network websocket': 2,
  'base app': 6,
  uncatgorized: 8,
  'base system': 8,
  'ui interaction': 2,
  file: 1,
  share: 2,
  storage: 1,
  'ui misc': 4,
  'ui keyboard': 1,
  'base misc': 1,
  canvas: 1,
  'device camera': 1
}

% following is qq raw data
\ignore{
addMapCircles, media map
addMapControls, media map
addMapLines, media map
addMapMarkers, media map
addMapPolygons, media map
getMapCenterLocation, media map
getMapRegion, media map
getMapRotate, media map
getMapScale, media map
getMapSkew, media map
includeMapPoints, media map
insertMap, media map
moveToMapLocation, media map
removeMapMarkers, media map
translateMapMarker, media map
updateMap, media map
createAudioInstance, media audio
destroyAudioInstance, media audio
getAudioState, media audio
getBackgroundAudioState, media audio
getMusicPlayerState, media audio
operateAudio, media audio
operateBackgroundAudio, media audio
operateMusicPlayer, media audio
operateRecorder, media recorder
setAudioState, media audio
setBackgroundAudioState, media audio
drawCanvas, canvas
insertCanvas, canvas
updateCanvas, canvas
removeCanvas, canvas
hideVirtualBottomNavigationBar, ui navigation
hideVirtualBottomNavigationBar, ui navigation
insertXWebLivePlayer, media live
operateXWebLivePlayer, media live
removeXWebLivePlayer, media live
setDisplayOrientation, ui misc
showVirtualBottomNavigationBar, ui navigation
showVirtualBottomNavigationBar, ui navigation
updateXWebLivePlayer, media live
hideVirtualBottomNavigationBar, ui navigation
insertXWebLivePusher, media live
operateXWebLivePusher, media live
removeXWebLivePusher, media live
setDisplayOrientation, ui misc
showVirtualBottomNavigationBar, ui navigation
updateXWebLivePusher, media live
getVolume, device misc
hideVirtualBottomNavigationBar, ui navigation
insertXWebVideo, ui webview
operateXWebVideo, ui webview
removeXWebVideo, ui webview
setDisplayOrientation, ui misc
setVolume, device misc
showVirtualBottomNavigationBar, ui navigation
updateXWebVideo, ui webview
insertXWebExternalElement, ui webview
operateXWebExternalElement, ui webview
removeXWebExternalElement, ui webview
updateXWebExternalElement, ui webview
insertImageView, media image
removeImageView, media image
updateImageView, media image
customWebviewPostMessage, ui webview
insertCustomHTMLWebView, ui webview
insertHTMLWebView, ui webview
scrollWebviewTo, ui webview
removeHTMLWebView, ui webview
scrollWebviewTo, ui webview
updateCustomHTMLWebView, ui webview
updateHTMLWebView, ui webview
insertLivePlayer, media live
operateLivePlayer, media live
removeLivePlayer, media live
updateLivePlayer, media live
insertLivePusher, media live
operateLivePusher, media live
removeLivePusher, media live
updateLivePusher, media live
insertCamera, media camera
insertVideoPlayer, media video
operateCamera, media camera
operateVideoPlayer, media video
removeCamera, media camera
removeVideoPlayer, media video
updateCamera, media camera
updateVideoPlayer, media video
getRegionData, open-api misc
showDatePickerView, ui interaction
showMultiPickerView, ui interaction
showPickerView, ui interaction
updateMultiPickerView, ui interaction
disableScrollBounce, ui interaction
insertScrollView, ui interaction
removeScrollView, ui interaction
updateScrollView, ui interaction
toggleSecureWindow, ui interaction
createLoadSubPackageTask, base app
detectAbnormalLog, open-api misc
insertTextView, ui misc
removeTextView, ui misc
updateTextView, ui misc
operateRecorder, media recorder
createBlockAd, ad
operateBlockAd, ad
updateBlockAdSize, ad
operateCustomButton, ui misc
getOpenDataUserInfo, open-api user-info
navigateToMiniProgramConfig, open-api navigation
recordOffLineResourceState, open-api misc
downloadWithCache, network download
setMenuStyle, ui menu
setStatusBarStyle, ui misc
onAppEnterBackground, base app
onAppEnterForeground, base app
onAppStop, base app
registerProfile, open-api misc
timePerformanceResult, open-api misc
onRaffleShareSucNotice, share
minigameRaffle, uncategorized
onUpdateCheckResult, base app
onUpdateDownloadResult, base app
updateApp, base app
insertVideoPlayer, media video
operateVideoPlayer, media video
removeVideoPlayer, media video
updateVideoPlayer, media video
operateAppBox, uncategorized
cancelDownloadAppTask, base app
installApp, base app
isMicroAppInstalled, base app
queryAppInfo, base app
queryDownloadAppTask, base app
startApp, base app
startDownloadAppTask, base app
refreshSession, open-api misc
createBannerAd, ad
operateBannerAd, ad
updateBannerAdSize, ad
insertBookshelf, open-api misc
enterContact, device contact
openCustomerServiceConversation, open-api misc
getTextLineHeight, ui misc
private_addContact, device contact
batchGetContact, device contact
getCloudTicket, open-api misc
getGroupInfo, open-api misc
getGroupInfoExtra, open-api misc
getNativeUserInfo, open-api user-info
getNativeWeRunData, open-api misc
openWeRunSetting, open-api misc
getPerformance, open-api misc
getUserInfoExtra, open-api user-info
invokeGroupJSApi, open-api misc
operateAppAdData, ad
operateWXData, open-api misc
profile, uncategorized
reportSubmitForm, open-api misc
verifyPlugin, base app
addFavorites, open-api misc
addToFavorites, open-api misc
createDownloadTask, network download
createFileSystemInstance, file
createUploadTask, network upload
operateDownloadTask, network download
operateUploadTask, network upload
compressImage, media image
hideKeyboard, ui misc
setKeyboardValue, ui misc
showKeyboard, ui misc
updateInput, ui misc
updateKeyboard, ui misc
getQua, uncategorized
getStoreAppList, open-api misc
launchApplication, base app
notifyNative, open-api misc
openUrl, network misc
private_openUrl, network misc
operateInterstitialAd, ad
saveAppToDesktop, open-api misc
invokeNativePlugin, open-api misc
openNativePage, open-api misc
canUseComponent, uncategorized
getFriendCloudStorage, open-api misc
getGroupCloudStorage, open-api misc
getPotentialFriendList, open-api misc
getReactiveFriendList, open-api misc
getUserCloudStorage, open-api misc
getUserInteractiveStorage, open-api misc
modifyFriendInteractiveStorage, open-api misc
removeUserCloudStorage, open-api misc
setMessageToFriendQuery, open-api misc
setUserCloudStorage, open-api misc
shareMessageToFriend, share
checkH5PayStatus, open-api payment
consumeStarCurrency, open-api misc
queryStarCurrency, open-api misc
rechargeAndConsumeStarCurrency, open-api misc
rechargeStarCurrency, open-api misc
requestFriendPayment, open-api payment
requestMidasCoinPaymentByH5, open-api payment
requestMidasGoodsPay, open-api payment
requestMidasMonthCardPay, open-api payment
requestMidasPayment, open-api payment
requestMidasPaymentByH5, open-api payment
Personalize, open-api misc
preloadPackage, base app
addFriend, open-api misc
api_report, open-api misc
realtimeLog, open-api misc
reportDC, open-api misc
reportDataToDC, open-api misc
reportKeyValue, open-api misc
reportRealtimeAction, open-api misc
addGroupApp, open-api misc
createRequestTask, network request
createSocketTask, network websocket
getGroupAppStatus, open-api misc
operateRequestTask, network request
operateSocketTask, network websocket
wnsCgiRequest, network misc
wnsGroupRequest, network misc
wnsGuildRequest, network misc
wnsRequest, network misc
operateRewardedAd, ad
openScheme, open-api misc
enableAccelerometer, device misc
enableCompass, device misc
enableDeviceMotionChangeListening, device misc
enableGyroscope, device misc
openAddress, open-api misc
openQzonePublish, open-api misc
shareAppMessage, share
shareAppMessageDirectlyToFriendList, share
shareAppMessageDirectly, share
shareAppPictureMessage, share
shareAppPictureMessageDirectly, share
showShareMenuWithShareTicket, share
updateShareMenuShareTicket, share
getGlobalStorage, storage
setGlobalStorage, storage
getPhoneNumber, device phone
createUDPTask, network misc
operateUDPTask, network misc
insertTextArea, ui misc
updateTextArea, ui misc
removeTextArea, ui misc
hideHomeButton, ui misc
updateQQApp, open-api misc
hideMiniAIOEntrance, open-api misc
showMiniAIOEntrance, open-api misc
addColorSign, ui misc
addColorSignDirectly, ui misc
addRecentColorSign, ui misc
isColorSignExistSync, ui misc
exitMiniProgram, open-api misc
navigateToWeMiniProgram, open-api navigation
tav_createObject, uncategorized
tav_sendMsgToObject, uncategorized
tav_releaseObject, uncategorized
tav_util, uncategorized
tav_createObject, uncategorized
tav_sendMsgToObject, uncategorized
tav_releaseObject, uncategorized
tav_checkInit, uncategorized
getCMShowInfo, uncategorized
setCMShowPetStatus, uncategorized
getChannelUserInfo, open-api user-info
openExpandChat, open-api misc
getExpandUserInfo, open-api user-info
checkin_uploadRes, open-api misc
getMultiMemList, open-api misc
play_invokeGYCamera, media camera
checkin_invokeGYCamera, media camera
miniApp_invokeGYCamera, media camera
launchApp, open-api misc
nowlive, media live
openConnectAuthorize, open-api misc
qsubscribe_getdeviceinfo, open-api misc
qsubscribe_opendetail, open-api misc
qsubscribe_opendiscover, open-api misc
qsubscribe_openhomepage, open-api misc
checkin_qzoneUploadAndPublish, open-api misc
refreshQzoneFeed, open-api misc
uploadAvatar, open-api misc
tdoc_channel, uncategorized
openTenpayView, ui misc
qWalletBridge, open-api misc
tim_space, open-api misc
freeTrafficCardModel, open-api misc
groupAlbum_downloadGroupAlbumPhoto, open-api misc
groupAlbum_groupUploadPhoto, open-api misc
groupAlbum_importGroupAIO, open-api misc
groupAlbum_jumpCategoryAlbum, open-api misc
groupAlbum_jumpGroupAlbumSendBox, open-api misc
groupAlbum_openUserQzoneHome, open-api misc
groupAlbum_pickQzoneAlbum, open-api misc
groupAlbum_showGroupPhotoBrowser, open-api misc
groupAlbum_start, open-api misc
requestWebSSO, open-api misc
weiyunDownload, network download
}

\ignore{
'media map': 16,
  'media audio': 10,
  'media recorder': 2,
  canvas: 4,
  'ui navigation': 8,
  'media live': 17,
  'ui misc': 23,
  'device misc': 6,
  'ui webview': 16,
  'media image': 4,
  'media camera': 7,
  'media video': 8,
  'open-api misc': 80,
  'ui interaction': 9,
  'base app': 17,
  ad: 9,
  'open-api': 1,
  'open-api navigation': 2,
  'network download': 4,
  'ui menu': 1,
  share: 9,
  uncategorized: 16,
  'device contact': 3,
  'open-api user-info': 4,
  file: 1,
  'network upload': 2,
  'network misc': 8,
  'open-api payment': 7,
  'network request': 2,
  'network websocket': 2,
  storage: 2,
  'device phone': 1
}

% following is wechat privileged raw data
\ignore{
uploadToCommonCDN, network upload
navigateToMiniProgramDirectly, open-api navigate
batchGetContactDirectly, device contact
preloadMiniProgramEnvDirectly, base app
predownloadMiniProgramPackageDirectly, base app
getABTestConfig, base app
setCookies, open-api misc
getCookies, open-api misc
enterContact, device contact
playBackgroundAudio, media audio
pauseBackgroundAudio, media audio
stopBackgroundAudio, media audio
sendBizRedPacket, open-api payment
requestVirtualPayment, open-api payment
chooseMultiMedia, media other
chooseWeChatContact, device contacts
uploadEncryptedFileToCDN, network upload
checkIsSupportFacialRecognition, open-api bio-auth
startFacialRecognitionVerify, open-api bio-auth
startFacialRecognitionVerifyAndUploadVideo, open-api bio-auth
startCustomFacialRecognitionVerify, open-api bio-auth
startCustomFacialRecognitionVerifyAndUploadVideo, open-api bio-auth
launchMiniProgram, base app
launchApplicationDirectly, base app
launchApplicationForNative, base app
captureScreen, device screen
quicklyAddBrandContact, device contact
preloadWebview, ui webview
openDeliveryList, open-api misc
navigateBackNative, open-api navigate
stopHCE, device bluetooth
addNativeDownloadTask, network download
secureTunnel, uncategorized
verifyPaymentPassword, open-api payment
bindPaymentCard, open-api payment
requestPaymentToBank, open-api payment
openOfflinePayView, open-api payment
requestMallPayment, open-api payment
setCurrentPaySpeech, open-api payment
loadPaySpeechDialectConfig, open-api payment
requestJointPayment, open-api payment
openWCPayOverseaPaymentReceive, open-api payment
handleWCPayOverseaWalletBuffer, open-api payment
requestVerifyUserIdentity, open-api misc
faceVerifyForPay, open-api payment
openOfficialAccountProfile, open-api misc
openUserProfile, open-api user-info
openSelectPayment, open-api payment
requestEntrustAuthorization, open-api misc
requestFacetoFacePayment, open-api payment
openWeAppProfile, open-api misc
openWeAppSearch, open-api misc
openWeAppHistoryList, open-api misc
openWeAppStarList, open-api misc
checkTrafficCardConditions, open-api misc
queryTrafficCardInfo, open-api misc
issueTrafficCard, open-api misc
rechargeTrafficCard, open-api misc
setDefaultTrafficCard, open-api misc
openQRCode, device scan
makeVoIPCall, device phone
showShareActionSheet, share
bindGroup, open-api account-info
joinGroup, open-api account-info
chooseShareGroup, open-api misc

  'network upload': 2,
  'open-api navigate': 2,
  'device contact': 3,
  'base app': 6,
  'open-api misc': 16,
  'media audio': 3,
  'open-api payment': 15,
  'media other': 1,
  'device contacts': 1,
  'open-api bio-auth': 5,
  'device screen': 1,
  'ui webview': 1,
  'device bluetooth': 1,
  'network download': 1,
  uncategorized: 1,
  'open-api user-info': 1,
  'device scan': 1,
  'device phone': 1,
  share: 1,
  'open-api account-info': 2
}

% following is wecom priviledged data
\ignore{
qy__showUserProfile
qy__postNotification
qy__canIUsePrivate
qy__chooseAttach
qy__wwOpenUrlScheme
qy__sendMessageToWX
qy__chooseWxworkContact
qy__selectConvAndAction
qy__chooseWxworkVisibleRange
qy__openEnterpriseContact
qy__startWecast
qy__operatePrivate
qy__shareAppMessageToAdmin
qy__shareToExternalContact
qy__shareToExternalChat
qy__shareToTraineeChat
qy__shareToTrainee
}

% following is baidu priviledged data
\ignore{
quickLogin, open-api login
faceVerify, open-api bio-auth
getRealNameInfo, open-api user-info
queryQuickLoginInfo, open-api login
getFaceVerifyImage, open-api bio-auth
getChannelID, open-api misc
thirdPartyLogin, open-api misc
getExtensionJSVersion, base basic
getSeid, uncategorized
getPayStatus, open-api payment
getZidInfo, uncategorized
getAbSwitches, uncategorized
callGC, base system
getSystemStatus, base system
getBDUSS, open-api user-info
getCommonSysInfo, base system
getAdDeviceInfo, ad
login, open-api login
getDeviceInfo, open-api misc
getFavor, open-api misc
checkPhoneContactsAuthorization, device contact
getDebugConfig, base debug
confirmAppClose, base app
getHistory, open-api misc
getPhoneContacts, device contact
openBdboxWebview, ui webview
getUnionBDUSS, open-api user-info

'open-api login': 3,
  'open-api bio-auth': 2,
  'open-api user-info': 3,
  'open-api misc': 5,
  'base basic': 1,
  uncategorized: 3,
  'open-api payment': 1,
  'base system': 3,
  ad: 1,
  'device contact': 2,
  'base debug': 1,
  'base app': 1,
  'ui webview': 1
}

% following is tiktok
\ignore{
  downloadFile: '{"errMsg":"downloadFile:fail param.url should pass String, not Undefined"}',
  createMapContext: 'parameter mapId should be a string.',
  requestPayment: '{"errMsg":"requestPayment:fail param.data should pass Object, not Undefined"}',
  requestWXH5Payment: '{"errMsg":"requestWXH5Payment:fail permission denied"}',
  ucRequestPayment: '{"errMsg":"requestPayment:fail param.data should pass Object, not Undefined"}',
  performance: 'globalThis.tt[l] is not a function',
  cloud: 'globalThis.tt[l] is not a function',
  requestSubscribeMessage: '{"errMsg":"requestSubscribeMessage:fail params.tmplIds should be array, but got undefined","errNo":20000}',
  checkAppInstall: '{"errMsg":"checkAppInstall:fail param.packageName should pass String, not Undefined"}',
  requestSafari: '{"errMsg":"requestSafari:fail android does not support"}',
  launchAppDirectly: '{"errMsg":"launchAppDirectly:fail param.scheme should pass String, not Undefined"}',
  showActionSheet: '{"errMsg":"showActionSheet:fail params.itemList should be array, but got undefined","errNo":20000}',
  canIPutStuffOverComponent: 'canIPutStuffOverComponent:fail inputs[0] should be string, but got a(n) object',
  canIUse: 'canIUse: schema should be string',
  connectSocket: '{"errMsg":"connectSocket:fail params.url should be string, but got undefined","errNo":20000}',
  compressImage: '{"errMsg":"compressImage:fail params.src should be string, but got undefined","errNo":20000}',
  previewImage: '{"errMsg":"previewImage:fail params.urls should be array, but got undefined","errNo":20000}',
  interactionAnalysis: '{"errMsg":"interactionAnalysis:fail expect params.type to be one of "like", "favorite", "post_comment", but got undefined","errNo":20000}',
  showLoading: '{"errMsg":"showLoading:fail params.title should be string, but got undefined","errNo":20000}',
  makePhoneCall: '{"errMsg":"makePhoneCall:fail params.phoneNumber should be string, but got undefined","errNo":20000}',
  navigateTo: '{"errMsg":"navigateTo:fail params.url should be string, but got undefined","errNo":20000}',
  redirectTo: '{"errMsg":"redirectTo:fail params.url should be string, but got undefined","errNo":20000}',
  reLaunch: '{"errMsg":"reLaunch:fail params.url should be string, but got undefined","errNo":20000}',
  switchTab: '{"errMsg":"switchTab:fail params.url should be string, but got undefined","errNo":20000}',
  openSchema: '{"errMsg":"openSchema:fail params.schema should be string, but got undefined","errNo":20000}',
  request: '{"errMsg":"request:fail params.url should be string, but got undefined","errNo":20000}',
  showECommerceAd: '{"errMsg":"showECommerceAd:fail params.ad_unit_id should be string, but got undefined","errNo":20000}',
  saveVideoToPhotosAlbum: '{"errMsg":"saveVideoToPhotosAlbum:fail params.filePath should be string, but got undefined","errNo":20000}',
  authorize: '{"errMsg":"authorize:fail params.scope should be string, but got undefined","errNo":20000}',
  onBeforeExitMiniProgram: 'onBeforeExitMiniProgram:fail inputs[0] should be function, but got a(n) object',
  navigateToMiniProgram: '{"errMsg":"navigateToMiniProgram:fail params.appId should be string, but got undefined","errNo":20000}',
  getMoreGamesInfo: '{"errMsg":"getMoreGamesInfo:fail params.appId should be string, but got undefined\n' +
    'params.ticket should be string, but got undefined","errNo":20000}',
  openLocation: '{"errMsg":"openLocation:fail params.latitude should be number, but got undefined\n' +
    'params.longitude should be number, but got undefined","errNo":20000}',
  showDouyinOpenAuth: '{"errMsg":"showDouyinOpenAuth:fail params.scopes should be object, but got undefined","errNo":20000}',
  onAccelerometerChange: 'onAccelerometerChange:fail inputs[0] should be function, but got a(n) object',
  offAccelerometerChange: 'offAccelerometerChange:fail inputs[0] should be function or undefined, but got a(n) object',
  openDocument: '{"errMsg":"openDocument:fail params.filePath should be string, but got undefined","errNo":20000}',
  onCompassChange: 'onCompassChange:fail inputs[0] should be function, but got a(n) object',
  offCompassChange: 'offCompassChange:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppShow: 'onAppShow:fail inputs[0] should be function, but got a(n) object',
  offAppShow: 'offAppShow:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppHide: 'onAppHide:fail inputs[0] should be function, but got a(n) object',
  offAppHide: 'offAppHide:fail inputs[0] should be function or undefined, but got a(n) object',
  onAppLaunch: 'onAppLaunch:fail inputs[0] should be function, but got a(n) object',
  offAppLaunch: 'offAppLaunch:fail inputs[0] should be function or undefined, but got a(n) object',
  openEcGood: '{"errMsg":"openEcGood:fail params.promotionId should be string, but got undefined","errNo":20000}',
  openDouyinProfile: '{"errMsg":"openDouyinProfile:fail params.userId should be string, but got undefined\n' +
    'params.shopId should be string, but got undefined","errNo":20000}',
  openEcCart: '{"errMsg":"openEcCart:fail params.shopId should be string, but got undefined","errNo":20000}',
  openEcCoupon: '{"errMsg":"openEcCoupon:fail params.shopId should be string, but got undefined\n' +
    'params.couponId should be string, but got undefined","errNo":20000}',
  openEcIm: '{"errMsg":"openEcIm:fail params.shopId should be string, but got undefined","errNo":20000}',
  openEcOrderDetail: '{"errMsg":"openEcOrderDetail:fail params.orderId should be string, but got undefined\n' +
    'params.shopId should be string, but got undefined","errNo":20000}',
  setTabBarBadge: '{"errMsg":"setTabBarBadge:fail params.index should be number, but got undefined\n' +
    'params.text should be string, but got undefined","errNo":20000}',
  removeTabBarBadge: '{"errMsg":"removeTabBarBadge:fail params.index should be number, but got undefined","errNo":20000}',
  showTabBarRedDot: '{"errMsg":"showTabBarRedDot:fail params.index should be number, but got undefined","errNo":20000}',
  hideTabBarRedDot: '{"errMsg":"hideTabBarRedDot:fail params.index should be number, but got undefined","errNo":20000}',
  setTabBarItem: '{"errMsg":"setTabBarItem:fail params.index should be number, but got undefined","errNo":20000}',
  setNavigationBarTitle: '{"errMsg":"setNavigationBarTitle:fail params.title should be string, but got undefined","errNo":20000}',
  setNavigationBarColor: '{"errMsg":"setNavigationBarColor:fail params.frontColor should be string, but got undefined\n' +
    'params.backgroundColor should be string, but got undefined","errNo":20000}',
  saveFile: '{"errMsg":"saveFile:fail params.tempFilePath should be string, but got undefined","errNo":20000}',
  getFileInfo: '{"errMsg":"getFileInfo:fail params.filePath should be string, but got undefined","errNo":20000}',
  removeSavedFile: '{"errMsg":"removeSavedFile:fail params.filePath should be string, but got undefined","errNo":20000}',
  reportAnalytics: 'reportAnalytics:fail the length of inputs should be greater than or equal to 2',
  getImageInfo: '{"errMsg":"getImageInfo:fail params.src should be string, but got undefined","errNo":20000}',
  getStorage: '{"errMsg":"getStorage:fail params.key should be string, but got undefined","errNo":20000}',
  setStorage: '{"errMsg":"setStorage:fail params.key should be string, but got undefined","errNo":20000}',
  removeStorage: '{"errMsg":"removeStorage:fail params.key should be string, but got undefined","errNo":20000}',
  setClipboardData: '{"errMsg":"setClipboardData:fail params.data should be string, but got undefined","errNo":20000}',
  preloadMiniProgram: '{"errMsg":"preloadMiniProgram:fail params.appList should be array, but got undefined","errNo":20000}',
  env: 'globalThis.tt[l] is not a function',
  createRewardedVideoAd: 'createRewardedVideoAd:fail inputs[0].adUnitId should be string, but got undefined',
  createEffectCameraStream: 'createEffectCameraStream:fail inputs[0].__webviewId__ should be number, but got undefined',
  uploadFile: '{"errMsg":"uploadFile:fail params.url should be string, but got undefined\n' +
    'params.filePath should be string, but got undefined\n' +
    'params.name should be string, but got undefined","errNo":20000}',
  getDownloadAppTaskStatusSync: 'getDownloadAppTaskStatusSync:fail inputs[0].app_name should be string, but got undefined\n' +
    'inputs[0].pkg_name should be string, but got undefined\n' +
    'inputs[0].download_url should be string, but got undefined',
  setSwipeBackMode: 'setSwipeBackMode:fail expect inputs[0] to be one of 0, 1, 2, but got a(n) object',
  offUserScreenRecord: 'offUserScreenRecord:fail inputs[0] should be function or undefined, but got a(n) object',
  createDownloadAppTask: 'createDownloadAppTask:fail inputs[0].apple_id should be string, but got undefined\n' +
    'inputs[0].download_url should be string, but got undefined\n' +
    'inputs[0].app_name should be string, but got undefined\n' +
    'inputs[0].pkg_name should be string, but got undefined',
  preloadVideo: '{"errMsg":"preloadVideo:fail the resource of video cannot be empty","errNo":21500}',
  getAmaz: 'getAmaz:fail platform auth deny',
  getAlgorithmManager: '{"errMsg":"getAlgorithmManager:fail params.width should be number, but got undefined\n' +
    'params.height should be number, but got undefined\n' +
    'params.useSyncMode should be boolean, but got undefined","errNo":20000}',
  createInterstitialAd: 'createInterstitialAd:fail inputs[0].adUnitId should be string, but got undefined',
  reportPOI: 'reportPOI:fail the length of inputs should be greater than or equal to 2',
  prefetchImages: '{"errMsg":"prefetchImages:fail params.images should be array, but got undefined","errNo":20000}',
  createTradeOrder: '{"errMsg":"createTradeOrder:fail params.goodsInfo should be array, but got undefined\n' +
    'params.totalAmount should be number, but got undefined","errNo":20000}',
  getTradeOrder: '{"errMsg":"getTradeOrder:fail params.orderId should be string, but got undefined","errNo":20000}',
  createTradeRefundOrder: '{"errMsg":"createTradeRefundOrder:fail params.orderId should be string, but got undefined\n' +
    'params.reason should be string, but got undefined\n' +
    'params.type should be string, but got undefined\n' +
    'params.description should be string, but got undefined","errNo":20000}',
  getTradeRefundOrder: '{"errMsg":"getTradeRefundOrder:fail params.refundOrderId should be string, but got undefined","errNo":20000}',
  completeRefundSync: 'completeRefundSync:fail the length of inputs should be greater than or equal to 2',
  onError: 'onError:fail inputs[0] should be function, but got a(n) object',
  offError: 'offError:fail inputs[0] should be function or undefined, but got a(n) object',
  callHostMethod: '{"errMsg":"callHostMethod:fail params.method should be string, but got undefined","errNo":20000}',
  callHostMethodSync: 'callHostMethodSync:fail inputs[0].method should be string, but got undefined',
  addHostEventListener: 'addHostEventListener:fail the length of inputs should be greater than or equal to 2',
  rateAwemeOrder: '{"errMsg":"rateAwemeOrder:fail params.orderId should be string, but got undefined","errNo":20000}',
  canRateAwemeOrders: '{"errMsg":"canRateAwemeOrders:fail params.orderIds should be array, but got undefined","errNo":20000}'
}

% following is qq raw data
\ignore{
  enterContact: '{"errMsg":"enterContact:fail no permission"}',
  getQimei36: '{"errMsg":"getQimei36:fail no permission"}',
  openScheme: '{"errMsg":"openScheme:fail no permission"}',
  invokeNativePlugin: '{"errMsg":"invokeNativePlugin:fail no permission"}',
  navigateToBookshelf: '{"errMsg":"navigateToBookshelf:fail no permission"}',
  getUserInfo: '{"errMsg":"getUserInfo:fail auth deny"}'
}


==> tables/official-api.tex <==

% official APIs table
% should it in categories?

% count down 700 with 500 -> 200 -> 50


==> tables/superapp-versions.tex <==



% raw data of WeChat

% | version | all | official |
% 6.3.27-880  &  77  &   76 \\
% 6.3.28-900  &  77  &   76 \\
% 6.3.30-920  & 107  &   96 \\
% 6.3.31-940  & 107  &   96 \\
% 6.3.32-941  & 121  &  101 \\
% 6.5.3-980   & 128  &  101 \\
% 6.5.4-1000  & 133  &  103 \\
% 6.5.7-1041  & 167  &  104 \\
% 6.5.8-1060  & 207  &  117 \\
% 6.5.10-1080 & 255  &  175 \\
% 6.5.13-1100 & 253  &  154 \\
% 6.5.14-1100 & 257  &  160 \\
% 6.5.16-1120 & 285  &  160 \\
% 6.5.19-1140 & 306  &  167 \\
% 6.5.22-1140 & 336  &  167 \\
% 6.5.23-1180 & 336  &  167 \\
% 6.6.0-1200  & 352  &  176 \\
% 6.6.1-1220  & 354  &  176 \\
% 6.6.2-1240  & 369  &  176 \\
% 6.6.3-1260  & 374  &  194 \\
% 6.6.6-1300  & 374  &  197 \\
% 6.6.7-1321  & 389  &  197 \\
% 6.7.2-1340  & 412  &  206 \\
% 6.7.3-1341  & 444  &  210 \\
% 6.7.3-1360  & 444  &  210 \\
% 6.7.4-1360  & 471  &  211 \\
% 7.0.0-1360  & 471  &  211 \\
% 7.0.0-1362  & 470  &  211 \\
% 7.0.0-1363  & 470  &  211 \\
% 7.0.0-1380  & 470  &  211 \\
% 7.0.3-1381  & 486  &  224 \\
% 7.0.3-1400  & 486  &  224 \\
% 7.0.4-1402  & 494  &  224 \\
% 7.0.4-1420  & 494  &  224 \\
% 7.0.5-1421  & 554  &  226 \\
% 7.0.6-1480  & 561  &  226 \\
% 7.0.6-1500  & 561  &  226 \\
% 7.0.7-1505  & 578  &  246 \\
% 7.0.7-1522  & 578  &  246 \\
% 7.0.7-1523  & 578  &  246 \\
% 7.0.8-1540  & 592  &  246 \\
% 7.0.9-1542  & 605  &  253 \\
% 7.0.9-1543  & 605  &  253 \\
% 7.0.9-1544  & 605  &  253 \\
% 7.0.9-1545  & 605  &  253 \\
% 7.0.9-1560  & 605  &  253 \\
% 7.0.10-1560 & 628  &  253 \\
% 7.0.10-1561 & 628  &  253 \\
% 7.0.10-1580 & 613  &  253 \\
% 7.0.12-1600 & 643  &  271 \\
% 7.0.12-1601 & 643  &  271 \\
% 7.0.12-1620 & 643  &  271 \\
% 7.0.13-1620 & 667  &  271 \\
% 7.0.13-1621 & 667  &  273 \\
% 7.0.13-1640 & 667  &  273 \\
% 7.0.14-1640 & 681  &  273 \\
% 7.0.14-1660 & 681  &  273 \\
% 7.0.15-1660 & 699  &  273 \\
% 7.0.15-1680 & 699  &  283 \\
% 7.0.15-1681 & 699  &  283 \\
% 7.0.16-1680 & 712  &  283 \\
% 7.0.16-1690 & 712  &  283 \\
% 7.0.16-1691 & 712  &  283 \\
% 7.0.16-1700 & 712  &  283 \\
% 7.0.17-1700 & 722  &  283 \\
% 7.0.17-1701 & 722  &  284 \\
% 7.0.17-1720 & 722  &  284 \\
% 7.0.18-1720 & 734  &  284 \\
% 7.0.18-1723 & 739  &  284 \\
% 7.0.18-1740 & 739  &  284 \\
% 7.0.19-1740 & 744  &  284 \\
% 7.0.19-1760 & 744  &  284 \\
% 7.0.20-1760 & 755  &  306 \\
% 7.0.20-1781 & 755  &  306 \\
% 7.0.21-1781 & 756  &  306 \\
% 7.0.21-1782 & 756  &  306 \\
% 7.0.21-1783 & 756  &  306 \\
% 7.0.21-1800 & 756  &  306 \\
% 7.0.21-1821 & 756  &  306 \\
% 7.0.22-1800 & 763  &  306 \\
% 7.0.22-1820 & 766  &  306 \\
% 8.0.0-1840  & 771  &  306 \\
% 8.0.1-1841  & 776  &  306 \\
% 8.0.2-1841  & 781  &  306 \\
% 8.0.2-1852  & 784  &  306 \\
% 8.0.2-1860  & 781  &  306 \\
% 8.0.3-1880  & 784  &  446 \\
% 8.0.6-1900  & 792  &  451 \\
% 8.0.7-1900  & 798  &  451 \\
% 8.0.7-1920  & 798  &  451 \\
% 8.0.9-1920  & 769  &  451 \\
% 8.0.9-1940  & 767  &  451 \\
% 8.0.11-1960 & 774  &  454 \\

% raw data of WeCom
% version | all | official 
% 2.7.2  | 488 | 206 + 44
% 2.8.2  | 561 | 211 + 51
% 2.8.5  | 563 | 211 + 52
% 2.8.6  | 563 | 211 + 52
% 2.8.7  | 566 | 211 + 53
% 2.8.8  | 566 | 211 + 53
% 2.8.9  | 566 | 211 + 53
% 2.8.10 | 566 | 211 + 53
% 2.8.17 | 566 | 211 + 53
% 3.0.1  | 567 | 211 + 54
% 3.0.12 | 711 | 271 + 56
% 3.0.20 | 719 | 271 + 61
% 3.0.24 | 720 | 271 + 62
% 3.0.28 | 720 | 271 + 62
% 3.1.18 | 655 | 271 + 86



% raw data of Baidu
% version | all | official 
% 11.18.0.8-96994304   | 239 | 336
% 11.19.0.8-97256448   | 238 | 337
% 11.21.0.9-97780864   | 238 | 341
% 11.22.0.8-98042880   | 238 | 341
% 11.25.0.8-98829312   | 239 | 366
% 12.0.0.8-100664320   | 239 | 372
% 12.0.0.9-100664448   | 239 | 372
% 12.0.0.10-100664576  | 239 | 372
% 12.0.0.12-100664832  | 239 | 372
% 12.3.0.8-101450752   | 239 | 379
% 12.3.0.9-101450880   | 239 | 379
% 12.16.1.10-104862976 | 242 | 296
% 12.17.5.10-105141504 | 242 | 298
% 12.21.0.12-106169856 | 245 | 317


% raw data of QQ
% version | all | official 
% 8.4.1-1442  | 389 | 270
% 8.4.18-1558 | 376 | 278
% 8.5.0-1596  | 418 | 282
% 8.5.5-1630  | 419 | 282
% 8.6.0-1672  | 420 | 282
% 8.6.5-1696  | 420 | 282
% 8.7.0-1718  | 420 | 282
% 8.8.3-1818  | 421 | 283
% 8.8.33-2150 | 431 | 287




==> tables/tbl-cmp.tex <==
\begin{table}[]
\centering
\scalebox{0.95}{
\scriptsize
\begin{tabular}{@{}clcc@{}}
\toprule[1.5pt]
 
\multicolumn{2}{c}{}                                                                                            & \textbf{\begin{tabular}[c]{@{}c@{}}Mobile Web\\ Browsers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Mobile Super \\ Apps\end{tabular}} \\ \midrule[0.7pt]
\multirow{5}{*}{\begin{tabular}[c]{c} Apps\\ Provided\end{tabular}}                 & Remote Backend             & Accessed via URLs                                                & Optional                                                       \\
                                                                                      & 1st-party Apps       & \cmark                                                 & \cmark                                        \\
                                                                                    &   3rd-party Apps       & \cmark                                                 & \cmark                                        \\
                                                                                          & Centralized Vetting     & \xmark                                                 & \cmark   \\
                                                                                                      & Openness     & \cmark                                                 & \xmark  \\
                                                                                         \midrule
\multirow{3}{*}{\begin{tabular}[c]{ c }Resources \\ Consumed \end{tabular}} & OS Resources        & \cmark                                                & \cmark                                        \\
                                                                                          & Super App Resources & \xmark                                                 & \cmark                                        \\
                                                                                          & Authentication  & OAuth, or Individually                                                                  & One-click Login                                                \\\midrule
                                                                                          \multirow{3}{*}{\begin{tabular}[c]{c}Examples\end{tabular}}  & 1st-party apps & Google.com, Firefox.com     &  WeChat Pay\\
                                                                           & 3rd-party apps & Facebook.com  & Starbucks Miniapp \\
                                                                           & Host apps & Chrome, Firefox  & Wechat, Snapchat \\
%                                                 & Environment         & Standard  engine                                                   & Customized engine                                             \\                                           
\bottomrule[1.5pt]
\end{tabular}
}
\caption{Comparison between mobile web browsers and mobile super apps}
\label{tab:cmp}
\end{table}
